The Fluted Fragment with Transitive Relations

We study the satisfiability problem for the fluted fragment extended with transitive relations. The logic enjoys the finite model property when only one transitive relation is available and the finite model property is lost when additionally either equality or a second transitive relation is allowed. We show that the satisfiability problem for the fluted fragment with one transitive relation and equality remains decidable. On the other hand we show that the satisfiability problem is undecidable already for the two-variable fragment of the logic in the presence of three transitive relations (or two transitive relations and equality).

==> 2-Undecidable.tex <==
%\newcommand{\border}{\ensuremath{\mathsf{border}}}
%\newcommand{\blt}{\ensuremath{\mathsf{border_l}}}
%\newcommand{\brt}{\ensuremath{\mathsf{border_r}}}
%\newcommand{\btp}{\ensuremath{\mathsf{border_t}}}
%\newcommand{\bbm}{\ensuremath{\mathsf{border_b}}}
%
%
%\newcommand{\corner}{\ensuremath{\mathsf{corner}}}
%\newcommand{\clt}{\ensuremath{\mathsf{corner_{lt}}}}
%\newcommand{\crt}{\ensuremath{\mathsf{corner_{rt}}}}
%\newcommand{\clb}{\ensuremath{\mathsf{corner_{lb}}}}
%\newcommand{\crb}{\ensuremath{\mathsf{corner_{rb}}}}


%\begin{center}
%	\begin{table}
%		
%		\begin{center}
%			{
%				{%\setlength{\extrarowheight}{5pt}
%					\begin{tabular}{|c|c|}
%						\hline
%						%			&\\
%						{\bf Special symbols} & {\large{\color{white}I}} {\bf Decidability and Complexity}\\
%						%			&\\
%						\hline\hline
%						no transitive r.  & { FMP, \NExpTime{}-complete}$(*)$ \cite{???,GKV97}\\
%					%	\hline 
%				%		0 transitive r. with = & {\bf no FMP, in \TwoNExpTime{}} \cite{???}\\
%				
%						\hline
%						1 transitive r.   & FMP, in \TwoNExpTime \cite{P-HT19}\\
%						\hline
%						1 transitive r. + = & \Sat: in \TwoNExpTime,  Theorem~\ref{th:one}\\
%											& \FinSat: in \ThreeNExpTime$(*)$ \cite{PH18}\\
%						\hline
%						2 transitive r.  &  no FMP: Example~\ref{ex:two}, Sat: ? \FinSat{}: ? \\
%						\hline
%						2 transitive r. + = & undecidable  (Fin)Sat: {Theorem~\ref{th:two}} \\
%						\hline
%						1 trans. + 1 equiv. + = & undecidable (Fin)Sat: Corollary~\ref{cor:two}\\
%						\hline
%						3 transitive r. & undecidable \Sat: Theorem~\ref{th:three} \FinSat{}: Theorem~\ref{th:threeFinsat}\\
%						\hline
%						3 equivalence r. & undecidable (Fin)Sat{}: Corollary~\ref{cor:three}\\
%						\hline
%						
%%						1 linear order $(*)$& \NExpTime-complete \cite{Otto01}\\
%%						\hline			
%%						2 linear orders $(*)$  & Sat: ? \FinSat{} in \TwoNExpTime{}   \cite{ZeumeH2016} \\
%%						\hline			
%%						3 linear orders & undecidable \cite{Kie2011}\\
%%						\hline			
%%						
%					\end{tabular} 
%			}}
%			\label{tabela}%\caption{Overview}
%			
%			\caption{Overview of $\FLt$ over restricted classes of structures. The upper bounds in the results marked with $(*)$ are actually obtained for full \FOt{}.}% The corresponding lower bounds, if present, hold for \GFt{}.}
%		\end{center}
%	\end{table}
%\end{center}
%


\section{Fluted Logic with more Transitive Relations}\label{sec:undecidable}
In the previous section, we considered $\FLt$ extended with a single transitive relation and equality.
In this section we consider $\FLt$ extended with more transitive relations.
Specifically, we show that the satisfiability and finite satisfiability problems for
$\FLt_=2T$
(two-variable fluted logic with two transitive relations and equality) or for $\FLt{}3T$
(two-variable fluted logic with three transitive relations but without equality), are all undecidable.
We also show that $\FLt2T$ (two-variable fluted logic with two transitive relations but without equality)
lacks the finite model property; however, the decidability of its satisfiability and finite satisfiability problems is left open.

A \emph{tiling system} is a tuple $\boldsymbol{\mathcal{C}}=({\mathcal C}, {\mathcal C}_H, {\mathcal C}_V)$,\nb{I don't like this notation} where
$\mathcal C$ is a finite set of {\em tiles},
and
${\mathcal C}_H$, ${\mathcal C}_V \subseteq {\mathcal C} \times {\mathcal C}$ are the  {\em horizontal} and {\em vertical} constraints.
A \textit{tiling} of $\N^2$ for $\boldsymbol{\mathcal{C}}$ is a function $f: \N^2 \rightarrow C$, such that 
for all $i,j \in \N$, 
$(f(i,j), f(i+1,j)) \in {\cal C}_H$ and $(f(i,j), f(i,j+1)) \in {\cal C}_V$. Intuitively, we think of $f$ as assigning 
(a copy of) some tile in $\cC$ to each point with integer coordinates in the upper-right quadrant of the plane: this assignment
must respect the horizontal and vertical constraints, understood as a list
of which tiles may be placed immediately to the right of (respectively: immediately above) which others. A tiling
is {\em periodic} if there exist $m$, $n$ such that, for all $i$ and  $j$, $f(i+m,j) = f(i,j+n) = f(i,j)$. 
Denote by 
$\N^2_{m,n}$ the finite initial segment
$[0,m-1] \times [0,n-1]$ of $\N^2$. A \textit{tiling} of $\N^2_{m,n}$ is a function
$f: \N^2_{m,n} \rightarrow C$, such that 
for all $i$, $j$ ($0 \leq i < m-1$, $0 \leq j \leq n-1$),
$(f(i,j), f(i+1,j)) \in {\cal C}_H$ and 
for all $i$, $j$ ($0 \leq i \leq  m-1$, $0 \leq j < n-1$), $(f(i,j), f(i,j+1)) \in {\cal C}_V$. If $f$ is a tiling (of either $\N^2_{m,n}$ or $\N^2$), we
call the value $f(0,0)$ the {\em initial condition}, and, if $f$ is a tiling of $\N^2_{m,n}$,
we call the value $f(m-1,n-1)$ the {\em final condition}.

There are many undecidability results concerning tiling systems: some are straightforward, others anything but.
The {\em infinite tiling problem with initial condition} is the following: given a tiling system $\boldsymbol{\mathcal{C}}$ and
a tile $c_0 \in \cC$, does there exist a tiling of $\N^2$ for $\boldsymbol{\mathcal{C}}$ with intial condition $c_0$?
The {\em finite tiling problem with initial and final conditions} is the following: given a tiling system $\boldsymbol{\mathcal{C}}$ and
tiles $c_0, c_1 \in \cC$, do there exist positive $m$, $n$ and a tiling of $\N^2_{m,n}$ for $\boldsymbol{\mathcal{C}}$ with intial condition $c_0$ and final condition $c_1$? It is straightforward to show:
\begin{proposition}
The infinite tiling problem with initial condition and the finite tiling problem with initial and final conditions are both undecidable.
\label{prop:noddyTiling}
\end{proposition}
The following result, by contrast, is deep (see~e.g.~\cite{purdyTrans:BGG97}). Recall that sets $A$ and $B$ are \textit{recursively inseparable} if there exists no recursive (=decidable) set $C$ such that $A \subseteq C$ and $B \cap C = \emptyset$.
\begin{proposition}
The set of tiling systems for which there exists a periodic tiling of $\N^2$ is recursively inseparable from the set 
of tiling systems for which there exists no tiling of $\N^2$.
\label{prop:insep}
\end{proposition}

%Let $S$ be any of the spaces $\N \times \N$, $\Z\times \Z$  or $\Z_t \times \Z_t$. 
%A tiling system $\boldsymbol{\mathcal{C}}$ \emph{tiles} $S$, if there exists a function $\rho: S \rightarrow {\cal C}$ such that for all $(p,q)\in S$: 
%$	(\rho(p,q), \rho(p+1,q)) \in {\cal C}_H$ and $(\rho(p,q), \rho(p,q+1)) \in {\cal C}_V$. 
%
%\begin{align*}
%&	(\rho(p,q), \rho(p+1,q)) \in {\cal C}_H\\
%&	(\rho(p,q), \rho(p,q+1)) \in {\cal C}_V
%%		\mbox{ and, } & \\
%%&	\rho(0,0)=c_0 \mbox{\quad (if origin constrained) }
%\end{align*}
%		$$(\rho(p,q), \rho(p+1,q)) \in C_H,$$  $$(\rho(p,q), \rho(p,q+1)) \in C_V.$$
%\end{definition}
%
%It is known that the problem whether a given tiling system tiles any of the spaces $\N \times \N$, $\Z\times \Z$, $\Z_t\times \Z_t$ is undecidable. 

%The following problems are undecidable \cite{purdyTrans:BGG97}:
%\begin{itemize}
%		\item
%	Plane tiling:	given a tiling system $\boldsymbol{\mathcal{C}}$ determine if $\boldsymbol{\mathcal{C}}$ tiles $\Z\times\Z$. 
%		\item
%Quadrant tiling:	given a tiling system $\boldsymbol{\mathcal{C}}$ determine if $\boldsymbol{\mathcal{C}}$ tiles $\N\times\N$. 
%	\item
%Torus tiling:	given a tiling system $\boldsymbol{\mathcal{C}}$ determine if $\boldsymbol{\mathcal{C}}$ tiles $\Z_t\times\Z_t$, for some $t\geq 1$. 
%	\item
%Rectangle tiling:	given a tiling system $\boldsymbol{\mathcal{C}}$ and two single tiles $C_0,C_0'$ determine if there exists $t,t'\geq 1$ and a tiling $\sigma$ of %a finite rectangle
% $\{0,\ldots, t\}\times\{0,\ldots t'\}$ such that $\sigma(0,0)=C_0$ and $\sigma(t,t')=C_0'$.  
%\end{itemize}

%We show how to reduce one of the above problems to the (finite) satisfiability problem for $\FLt$ with transitive relations. 

%Let $\boldsymbol{\mathcal{C}}=({\cal C}, {\cal C}_H, {\cal C}_V)$ be a tiling system. 
%
%%
%We write an $\cal L$-formula $\eta_{\boldsymbol{\cal{C}}} $ such that the following reduction properties hold
%\begin{enumerate}
%	\item[(i)]	$\eta_{\boldsymbol{\cal C}}$ is satisfiable  iff  $\boldsymbol{\cal C}$ tiles  $\N \times \N$ or $\Z \times \Z$, and 
%	\item[(ii)]	$\eta_{\boldsymbol{\cal C}}$ is finitely satisfiable  iff  $\boldsymbol{\cal C}$ tiles  $\Z_t \times \Z_t$, for some $t\geq 1$.
%\end{enumerate}
%Properties (i) and (ii) above yield undecidability of the satisfiability, respectively, finite satisfiability, problem for $\cal L$. 
%


%When $\cal L$ is a two-variable logic it is convenient to define $\eta_{\boldsymbol{\cal C}}$ as a conjunction $\eta_{\boldsymbol{\cal C}}:= \phi_{grid}\wedge \phi_{\boldsymbol{\cal{C}}}$, where the role of $\phi_{grid}$ is to define {\em grid-like} structures and $\phi_{\boldsymbol{\cal{C}}}$ assigns to nodes of a model {\em tiles} from $\cal C$ treating each $C \in {\cal C}$ as a unary predicate. 
% The latter task in \fod{} is easy. Assume $\phi_{grid}$ contains the conjunct $\forall x (\exists y h(x,y) \wedge \exists y v(x,y)$, with $h$ and $v$ binary predicates representing the horizontal and vertical successors 
% One can take $\phi_{\boldsymbol{\mathcal{C}}}$ as a conjunction of the following \fod{}-formulas:
%
\subsection{The case with two transitive relations}\label{sec:twotrans}

In this section we show that both the satisfiability and the finite satisfiability problems for $\FLtwotranstEq$ are undecidable. 
(Recall from Example~\ref{ex:two} that $\FLtwotrans$ admits infinity axioms.)
%
	%
	\begin{figure}[thb]
		\begin{center}
			\begin{minipage}{13cm}
				\begin{minipage}{12.5cm}
					\begin{center}
						\begin{tikzpicture}[xscale=1,yscale=1]
						%
						% 					\def{\z}{0.1}
						\clip (-0.15,-0.15) rectangle (7.3,4.3);
						\foreach \x in {-1,1,3,5,7}
						\foreach \y in {-1,1,3,5,7} \foreach \z in {0.1} 
						{
							\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
							(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
							\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) --
							(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
							
						}	
						
						\foreach \x in {0,2,4,6}
						\foreach \y in {0,2,4,6} \foreach \z in {0.1} 
						{
							\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
							(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
							\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) --
							(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
						}	
						
						\foreach \x in {1,5}
						\foreach \y in {1,5} \foreach \z in {0.15} 
						{
							\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
							\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
							\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
							\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
						}	
						
						\foreach \x in {3,7}
						\foreach \y in {3,7} \foreach \z in {0.15} 
						{
							\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
							\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
							\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
							\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
						}	
						
						
						\foreach \x in {1,5}
						\foreach \y in {3,7} \foreach \z in {0.15} 
						{
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x, \y) ;
							\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y);
							\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y);
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x, \y-1);						
						}	
						
						\foreach \x in {3,7}
						\foreach \y in {1,5} \foreach \z in {0.15} 
						{
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
							\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
							\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
						}	
						
						\foreach \x in {1,5}
						\foreach \y in {3,7} \foreach \z in {0.15} 
						{
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
							\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
							\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
							\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
						}	
						
						
						
						% 						\draw[color=red,thick,->, >=latex] (\x-0.05, \y+0.1) -- (\x-0.05, \y+0.8);
						% 						
						% 						%	\draw[color=blue,thick,->, >=latex] (\x+0.1, \y) -- ($(\x,\y) + (0.9,0)$); 
						% 						\draw[color=black,thick,->, >=latex] (\x+0.1, \y-0.05) -- ($(\x,\y) + (0.8,0-0.05)$); 
						% 						\draw[color=blue,thick,->, >=latex] (\x+0.1, \y+0.05) -- ($(\x,\y) + (0.8,0+0.05)$); 
						% 						
						% 						%		\draw[color=blue,thick,->, >=latex] (\x+1.9, \y) -- ($(\x,\y) + (1.1,0)$); 
						% 						\draw[color=green,thick,->, >=latex] ($(\x,\y) + (1.1,-0.05)$) -- (\x+1.8, \y-0.05); 
						% 						\draw[color=red,thick,->, >=latex] ($(\x,\y) + (1.1,+0.05)$) -- (\x+1.8, \y+0.05); 
						% 						
						% 						%\draw[color=blue,thick,->, >=latex] (\x+1, \y+0.1) -- (\x+1, \y+0.9);
						% 						\draw[color=blue,thick,->, >=latex] (\x+0.95, \y+0.1) -- (\x+0.95, \y+0.8);
						% 						\draw[color=red,thick,dashed,->, >=latex] (\x+1.05, \y+0.1) -- (\x+1.05, \y+0.8);
						% 						
						%					}
						
						
						% 					\foreach \x in {1,3,5}
						% 					\foreach \y in {3,5}{
						% 						\draw[color=green,thick,dashed,->, >=latex]  (\x-0.05, \y+0.1) -- (\x-0.05, \y+0.8);
						% 						\draw[color=black,thick,->, >=latex]  (\x+0.05, \y+0.1) -- (\x+0.05, \y+0.8);
						% 						
						% 						\draw[color=blue,thick,->, >=latex] ($(\x,\y) + (0.9,-0.05)$) -- (\x+0.2, \y-0.05) ; 
						% 						\draw[color=black,thick,->, >=latex] ($(\x,\y) + (0.9,0.05)$) -- (\x+0.2, \y+0.05) ; 
						% 						
						% 						\draw[color=red,thick,->, >=latex] ($(\x,\y) + (1.8,-0.05)$) -- (\x+1.2, \y-0.05) ; 
						% 						\draw[color=green,thick,->, >=latex] ($(\x,\y) + (1.8,0.05)$) -- (\x+1.2, \y+0.05) ; 
						% 						
						% 						\draw[color=black,thick,dashed,->, >=latex]  (\x+0.95, \y+0.1) -- (\x+0.95, \y+0.8);
						% 						\draw[color=green,thick,->, >=latex]  (\x+1.05, \y+0.1) -- (\x+1.05, \y+0.8);
						% 						
						% 					}
						
						
						% 					\foreach \x in {1,2,3,4,5,6}
						% 					\foreach \y in {2}
						% 					{
						% 					\filldraw[fill=white] (\x, \y) circle (0.2); 
						% 					\pgfmathtruncatemacro{\abc}{mod(\y-1,2)} 
						% 					\pgfmathtruncatemacro{\bcd}{mod(\x-1,2)} 
						% 					\coordinate [label=center:$b_{\bcd \abc}$] (A) at (\x,\y);
						% 				}
						
						\foreach \x in {0,1,2,3,4,5,6,7}
						\foreach \y in {0,1,2,3,4,5,6,7}
						{
							\filldraw[fill=white] (\x, \y) circle (0.2); 
							\pgfmathtruncatemacro{\abc}{mod(\y,4)} 
							\pgfmathtruncatemacro{\bcd}{mod(\x,4)} 
							\coordinate [label=center:$_{\bcd\abc}$] (A) at (\x,\y);
						}
						
						
						%	\foreach \x in {1,2,3,4,5,6} \pgfmathtruncatemacro{\abc}{\x-1} \coordinate [label=center:$_{\abc}$] (A) at (\x, 1.5);
						%	\foreach \y in {1,2,3,4,5} \pgfmathtruncatemacro{\abc}{\y-1} \coordinate [label=center:$_{\abc}$] (A) at (0.5,\y+1);
						
						\draw[ ->, dotted, very thick] (7.5,0) -- (8,0);
						\draw[ ->, dotted, very thick] (0,7.5) -- (0,8);
						\draw[ ->, dotted, very thick] (7.5,7.5) -- (8,8);
						
						% 					\coordinate [label=center:$b$] (A) at (1.5,1.8);
						% 					\coordinate [label=center:$\color{cyan}c$] (A) at (1.5,2.2);
						% 					\coordinate [label=center:$\color{green}g$] (A) at (2.5,1.8);
						% 					\coordinate [label=center:$\color{red}r$] (A) at (2.5,2.2);
						% 					
						\end{tikzpicture}\end{center}
				\end{minipage}
				
			\end{minipage}		
		\end{center}
		
		\caption{Intended expansion of the $\N\times\N$ grid with two transitive relations {\color{blue}$b$}   and  {\color{red}$r$}. Edges without arrows represent connections in both direction. Nodes are marked by the indices of  the $c_{ij}$s they satisfy.  % (left picture)
			% and with three transitive relations $r_1, r_2, r_3$ (right picture).}\label{fig:und-equivalences}
			\label{fig:grid-two-transitive}}
	\end{figure}
	
	\begin{enumerate}[(1)]
		%	[label=(\arabic*]}
		\item There\nb{I: Tidied up these conjunct groups} is an initial element: $\exists  c_{00} $.
		%	\begin{equation*}
		%	\exists x (c_{00}(x) \wedge l(x)).
		%	\end{equation*}
		
		
		\item The predicates $c_{i,j}$ enforce a partition of the universe: $	\forall  (\dot{\bigvee}_{0\leq i \leq 3} \dot{\bigvee}_{0\leq j \leq 3} c_{i,j}) 
		$.	\label{tiling:partition}
		%	\begin{eqnarray*}
		%	\forall x \dot{\bigvee}_{0\leq i \leq 3} \dot{\bigvee}_{0\leq j \leq 3} c_{i,j}(x) 
		%	%	\forall x (c_{00}(x) \dot{\vee} c_{01}(x) \dot{\vee} c_{10}(x) \dot{\vee} c_{11}(x))
		%	\label{tiling:partition}
		%	\end{eqnarray*}
		\item Transitive paths do not connect distinct elements of the same colour:
		\begin{eqnarray*}
			\bigwedge_{0\leq i,j\leq 3} \forall  (c_{ij}\rightarrow \forall  ((b\vee r)\wedge c_{ij} \rightarrow =)).
			%	\bigwedge_{0\leq i,j\leq 3} \forall x (c_{ij}(x)\rightarrow \forall y (b(x,y)\wedge c_{ij}(y) \rightarrow x=y))
		\end{eqnarray*}\label{Clique}
		
\item   
Each element belongs to a 4-element blue clique: \label{CliqueBlue}
		%\end{enumerate}
%		\begin{align*}
%		%
%		%\bigwedge_{i,j=0,2} 
%		\forall x (c_{ij} &\rightarrow \exists  (b\wedge c_{i+1,j}))\\ %\wedge 	
%		\forall x (c_{i+1,j} &\rightarrow \exists  (b\wedge c_{i+1,j+1})) 	\nonumber\\
%		\forall x (c_{i+1,j+1} &\rightarrow \exists  (b\wedge c_{i,j+1})) \nonumber\\
%		\forall x (c_{i,j+1} &\rightarrow \exists  (b\wedge c_{ij})) 
%		%
%		\end{align*}
		%
		\begin{align}
	%
\bigwedge_{i,j \in \set{0,2}}
	\forall \quad \big( (c_{ij} &\rightarrow \exists  (b\wedge c_{i+1,j}))\wedge 	
	%\forall 
	(c_{i+1,j} \rightarrow \exists  (b\wedge c_{i+1,j+1})) \wedge\tag{4a}\\ %	\nonumber\\
	%\forall  
	(c_{i+1,j+1}& \rightarrow \exists  (b\wedge c_{i,j+1})) \wedge  
	%\forall  
\bigwedge_{i,j \in \set{0,2}}
	(c_{i,j+1} \rightarrow \exists  (b\wedge c_{ij})) \big);\nonumber
	%
	\end{align}
	%	
		%\begin{enumerate}[(5)]
		%\item[(4'')]  
moreover, each element belongs to a 4-element red clique:\label{CliqueRed}
		%\end{enumerate}
		%
%		\begin{align*}
%		%
%		%\bigwedge_{i,j=1,3} \big( 
%		\forall x (c_{ij} &\rightarrow \exists  (r\wedge c_{i+1,j}))\\ %\wedge 	
%	\forall x (c_{i+1,j} &\rightarrow \exists  (r\wedge c_{i+1,j+1})) 	\nonumber\\
%	\forall x (c_{i+1,j+1} &\rightarrow \exists  (r\wedge c_{i,j+1})) \nonumber\\
%	\forall x (c_{i,j+1} &\rightarrow \exists  (r\wedge c_{ij})) 
%		%
%		\end{align*}
				\begin{align}
		%
		%	\bigwedge_{i,j=0,2}  
\bigwedge_{i,j \in \set{1,3}}\forall \quad \big( (c_{ij} &\rightarrow \exists  (r\wedge c_{i+1,j}))\wedge 	
		%\forall 
		(c_{i+1,j} \rightarrow \exists  (r\wedge c_{i+1,j+1})) \wedge \tag{4b}\\ %	\nonumber\\
		%\forall  
\bigwedge_{i,j \in \set{1,3}} 
	(c_{i+1,j+1}& \rightarrow \exists  (r\wedge c_{i,j+1})) \wedge  
		%\forall  
		(c_{i,j+1} \rightarrow \exists  (r\wedge c_{ij})) \big).\nonumber
		%
		\end{align}
		%
		%\end{enumerate}
		%	Note that a conjunction of the formulas (2)-(5) %\eqref{Clique} and \eqref{tiling:partition} 
		%	implies that each element of a model of these formulas is a member of a four-element blue clique and a member of a four-element red clique; moreover, distinct elements of these cliques have distinct colours.   	
		
		%\begin{enumerate}
		%	\resume*
		\item Certain pairs of elements connected by one transitive relation are also connected by the other one, specifically: 
		\begin{align}
		%
		\bigwedge_{i=0,2} \forall  (c_{ii} \rightarrow &\forall  ((b\vee r)\wedge (c_{i,i-1}\vee c_{i-1,i})\rightarrow (b\wedge r))\tag{5a}
		% \wedge \nonumber\\
		%\forall x (c_{ii}(x) \rightarrow &\forall y (r(x,y)\wedge c_{i-1,i}(y))\rightarrow b(x,y)))
		\label{IfRed00}\\
		%
		\bigwedge_{i=1,3} \forall  (c_{ii} \rightarrow &\forall  ((b \vee r)\wedge (c_{i,i+1}\vee c_{i+1,i})\rightarrow (b\wedge r))\tag{5b}
		\label{IfRed11}\\	
		%
		\bigwedge_{i=0,2} \forall  (c_{i,i+1} \rightarrow &\forall  ((b \vee r)\wedge (c_{i,i+2}\vee c_{i-1,i+1})\rightarrow (b\wedge r))\tag{5c}
		\label{IfRed01}\\		%
		\bigwedge_{i=1,3} \forall  (c_{i,i-1} \rightarrow &\forall  ((b \vee r)\wedge (c_{ii}\vee c_{i,i-2} )\rightarrow (b\wedge r))\tag{5d}
		\label{IfRed10}
		%		
		%
		\end{align}
		
%		%\item[(5'')] 
%		- a group of formulas saying that some pairs of elements connected by $b$ are also connected by $r$: 
%		\begin{align}
%		%
%		\bigwedge_{i=0,2} \forall x (c_{ii}  \rightarrow &\forall y (b \wedge (c_{i,i-1} \vee c_{i-1,i}  )\rightarrow r )) \tag{7a}
%		\label{IfBlue00}\\
%		%
%		\bigwedge_{i=1,3} \forall x (c_{ii}  \rightarrow &\forall y (b \wedge (c_{i,i+1}  \vee  c_{i+1,i}  )\rightarrow r ))\tag{7b}
%		\label{IfBlue11}\\
%		%
%		\bigwedge_{i=0,2} \forall x (c_{i,i+1}  \rightarrow &\forall y (b \wedge (c_{i,i+2} \vee c_{i-1,i+1} )\rightarrow r )) \tag{7c}
%		\label{IfBlue01}\\
%		%
%		\bigwedge_{i=1,3} \forall x (c_{i,i-1}  \rightarrow &\forall y (b \wedge (c_{ii} \vee c_{i,i-2} )\rightarrow r ))\tag{7d}
%		\label{IfBlue10}
%		%		
%		%
%		\end{align}
%	
\end{enumerate}		
	A model of $\phi_{grid}$ is shown in Fig~\ref{fig:grid-two-transitive}. 
	One can also obtain finite models over a toroidal grid structure $\Z_{4m}\times \Z_{4m}$  ($m>0$) by identifying elements from columns 0 and $4m$ and from rows 0 and $4m$. 
	
	
	
%	In\nb{I: Still under construction.} order to encode tilings using two-variable logics it actually suffices to define structures that are grid-like. 
%	A structure $\fG=(G,h,v)$ with two binary relation $h$ and $v$ is {\em grid-like}, if one of the standard grids $\N\times \N$, $\Z\times\Z$ or $\Z_t\times\Z_t$ can be homomorphically embedded into $\fG$. Note that $\fG$ is grid-like if
%	it makes true the formulas $\forall x (\exists y . h(x,y) \wedge \exists y . v(x,y))$ and
%	\begin{equation*}
%	\forall xx'yy' ((h(x,y)\wedge v(x,x')\wedge v(y,y') \rightarrow h(x',y')).\tag{*}
%	\end{equation*}\label{tiling}
%	The first of these is an $\FLt$-formula, and we may write it, in variable-free notation, as $\forall (\exists h \wedge \exists v)$. The second, which we refer to as the {\em confluence} property is not fluted; however, we can reproduce its effect it in $\FLt{}$ using the transitive relations. 

We show that any model of $\phi_{grid}$ embeds the standard grid $\N^2$ in a natural way. To see this,
for all $i$, $j$ in the range $0 \leq i, j <4$, define the formulas $h_{i,j}$ and $v_{i,j}$ as follows:
\begin{align*}
h_{i,j} := & 
\begin{cases}
		b \wedge  c_{i+1,j} & \text{if $i$ is even}\\
		r \wedge  c_{i+1,j} & \text{otherwise}
\end{cases} & &
v_{i,j} := & 
\begin{cases}
b \wedge  c_{i,j+1} & \text{if $j$ is even}\\
r \wedge  c_{i,j+1} & \text{otherwise.}
\end{cases}
\end{align*}
The intuition is that, for any element $a$ satisfying $c_{i,j}$, $h_{i,j}$, will be satisfied by the pair $ab$ just in case
$b$ is immediately to the right of $a$, and $v_{i,j}$, will be satisfied by the pair $ab$ just in case
$b$ is immediately above $a$. (See Fig.~\ref{fig:grid-two-transitive}.) 

\begin{lemma}
In any model $\fA$, of $\phi_{grid}$, the following hold
\begin{align}
& \fA \models c_{i,j}[a] \Rightarrow \text{ there exists $b$ s.t.~$\fA \models h_{i,j}[a,b]$ and
	                                      $a'$ s.t.~$\fA \models v_{i,j}[a,a']$;}
\label{eq:propagate}\\
\begin{split}
& \fA \models c_{i,j}[a], \fA \models h_{i,j}[a,b],
\fA \models v_{i,j}[a,a'] \text{ and } 
\fA \models v_{i+1,j}[b,b'] \Rightarrow\\ 
& \hspace{8cm} \fA \models h_{i,j+1}[b,b'].
\end{split}
\label{eq:confluence}
\end{align}
\label{lma:grid}
\end{lemma}
\begin{proof}
We\nb{The details in this proof need updating} establish~\eqref{eq:propagate} separately for the possible indices $i$ and $j$.
Consider first the case $i = j= 0$, and suppose $\fA\models c_{00}(a)$. By \eqref{CliqueBlue}, $a$ belongs to a 4-element blue clique, i.e.~there are $a_1,a_2,a_3,a_4\in A$ such that $\fA \models b(a,a_1)\wedge c_{10}(a_1) \wedge b(a_1,a_2)\wedge c_{11}(a_2)\wedge b(a_2,a_3)\wedge c_{01}(a_3) \wedge b(a_3,a_4)\wedge c_{00}(a_4)$. 
By \eqref{Clique} $a=a_4$ and by transitivity of $b$ the elements $a,a_1,a_2,a_3$ form a blue clique in $\fA$. Hence, $\fA\models h(a,a_1)$ and $\fA\models v(a,a_3)$. 
Now consider the case  $i =1$, $j= 0$, and suppose $\fA\models c_{10}(a)$.
By \eqref{CliqueBlue} there is $a'\in A$ such that $\fA\models b(a,a')\wedge c_{11}(a')$, hence $\fA\models v(a,a')$. Moreover, by \eqref{CliqueRed} there are $a_1,a_2,a_3,a_4\in A$ such that $\fA \models r(a,a_1)\wedge c_{13}(a_1) \wedge r(a_1,a_2)\wedge c_{23}(a_2)\wedge r(a_2,a_3)\wedge c_{20}(a_3)\wedge  r(a_3,a_4)\wedge c_{10}(a_4)$. 
By \eqref{Clique} $a=a_4$ and by transitivity of $r$ the elements $a,a_1,a_2,a_3$ form a red clique in $\fA$. By \eqref{IfRed10} $\fA\models b(a,a_1)$, hence $\fA\models h(a,a_1)$. The remaining cases are dealt with similarly. We should regard the witnesses for the formulas $\exists h_{i,j}$ and $\exists v_{i,j}$ with respect to any element $a$ are the 
horizonal and vertical neighbours, respectively, of $a$.

We next establish~\eqref{eq:confluence}, again proceeding separately for the possible indices $i$ and $j$.
Consider first the case $i = j= 0$, and suppose $\fA\models c_{00}(a)$. Applying the formulas $\forall (c_{i,j} \rightarrow \exists h_{i,j} \wedge \exists v_{i,j})$, we have $a'$, $b$ and $b'$ such that $\fA \models c_{01}(a')\wedge b(a,a')\wedge b(a,b) \wedge c_{10}(b)\wedge b(b,b') \wedge c_{11}(b')$. By \eqref{CliqueBlue} $b'$ is a member of a blue clique containing elements of colours $c_{11}, c_{01}, c_{00}, c_{10}$. Since by \eqref{Clique} the relation $b$ does not connect distinct elements of the same colour, $a'$ belongs to the blue clique of $b'$ and $\fA \models b(a',a)$. Now, by transitivity of $b$, $\fA \models h(a',b')$. 

Consider now the case $i = 3$, $j= 0$, and suppose
$\fA \models c_{30}(a)$. Then we have $a'$, $b$ and $b'$  such that
$\fA \models c_{31}(a')\wedge b(a,a')\wedge r(a,b) \wedge c_{00}(b)\wedge b(b,b') \wedge c_{01}(b') $. 
Thus, $b$ belongs to the red clique of $a$, whence $\fA\models r(b,a)$. 
By \eqref{IfRed00}, $\fA \models b(b,a)$. Moreover, $b'$ is in a blue clique of $b$, and so $\fA \models b(b',b)$. 
By transitivity of $b$,  $\fA \models b(b',a')$.  Now, by \eqref{IfBlue01}, $\fA\models r(b',a')$. 
By \eqref{CliqueBlue}, $a'$ is a member of a red clique that, by \eqref{Clique}, must contain $b'$. Hence $h(a',b')$ holds.
		
		%\item 
		%$\fA \models c_{21}(a)$. Then by \eqref{right} and \eqref{up} $\fA \models c_{22}(a')\wedge b(a',a)\wedge b(a,b) \wedge c_{31}(b)\wedge b(b',b) \wedge c_{32}(b') $.
		%By \eqref{CliqueBlue} $a'$ is a member of a blue clique containing (in particular) an element $d$ such that  $\fA\models b(d,a')\wedge c_{32}(d)$. By transitivity of $b$, $\fA\models b(d,b)$. By \eqref{IfBlue10} $\fA\models r(d,b) \wedge r(b',b)$. By \eqref{CliqueRed} $b$ is a member of a red clique containing an element $d'$ of colour $c_{32}$. By \eqref{Clique} $d=d'$, and hence $\fA \models \htw(a',b')$.  
		
		%\item
		%$\fA \models c_{01}(a)$.  Then %by \eqref{right} and \eqref{up} 
		%$\fA \models c_{02}(a')\wedge b(a,a')\wedge b(b,a) \wedge c_{11}(b)\wedge b(b,b') \wedge c_{12}(b') $.
		%By \eqref{CliqueBlue} $a'$ is a member of a blue clique containing (in particular) an element $d$ such that  $\fA\models b(a,d)\wedge c_{12}(d)$. By transitivity of $b$, $\fA\models b(b,d)$. By \eqref{IfBlue10} $\fA\models r(b,d) \wedge r(b',b)$. By \eqref{CliqueRed} $b'$ is a member of a red clique containing an element $d'$ of colour $c_{11}$. By \eqref{Clique} $b=d'$, and employing transitivity of $r$ also $d=b'$, hence  $\fA \models \htw(a',b')$.  
	%
The remaining cases are dealt with similarly.
\end{proof}

Lemma~\ref{lma:grid} shows that any model $\fA$ of $\phi_{grid}$ contains, in effect, a homomorphic embedding of the infinite 
grid $\N^2$. Secifically, we define a function $\iota: \N^2 \rightarrow A$ as follows.
Set $\iota(0,0)$ to be some witness for (1). By~\eqref{eq:propagate},
we may choose $\iota(1,0), \iota(2,0), \dots$ such that, for all $i \geq 0$, $\fA \models h_{i,0}[\iota(i,0), \iota(i+1,0)]$; and
then, for every $i \geq 0$, we may choose $\iota(i,1), \iota(i,2), \dots$ such that for every $j \geq 0$,
$\fA \models v_{i,j}[\iota(i,j), \iota(i,j)]$.  A simple induction on $j$ using~\eqref{eq:confluence} then shows that, for all $i$ and $j$,
$\fA \models h_{i,j}[\iota(i,j), \iota(i+1,j)]$. 

We can now map any tiling system $\boldsymbol{\mathcal{C}}$ to an $\mathcal{FL}^2_=2\mbox{\rm T}$-formula $\eta_\cC$ in such 
a way that  $\cC$ is has a tiling if any only if $\eta_\cC$ is satisfiable. We simply let $\eta_\cC$ be the conjunction of
$\phi_{grid}$ with the following formulas. 
\begin{enumerate}
\item[(6)] Each node encodes precisely one tile: $$\forall \big(\bigvee_{C \in {\cal C}} C  \wedge \bigwedge_{C \neq D} (\neg C   \vee \neg D )\big).$$
	%	
		%		\begin{eqnarray}
		%		\forall x (\dot{\bigvee}_{C \in {\cal C}} C x)\label{tiling:C1}
		%		\end{eqnarray}
\item[(7)] Adjacent tiles respect ${\cal C}_H$ and ${\cal C}_V$:
	\begin{eqnarray*}
		%
		\bigwedge_{0 \leq i,j < 4} \forall (C \wedge c_{ij}  \rightarrow  \forall y (h_{i,j}  \rightarrow \bigvee_{C': (C,C') \in {\cal C}_H}  C'))\wedge\\
		\bigwedge_{0 \leq i,j < 4} \forall (C \wedge c_{ij}  \rightarrow  \forall y (v_{i,j}  \rightarrow \bigvee_{C': (C,C') \in {\cal C}_V}  C')).
		%
	\end{eqnarray*}
\end{enumerate}
	%	
	%	\htw(x,y) := & b(x,y) \wedge b(y,x) \wedge  
	%	\bigvee_{i=0,2, j=0,1,2,3 } (c_{ij}  \wedge c_{i+1,j}  )\vee 
	%	\nonumber\\
	%	& r(x,y) \wedge r(y,x) \wedge  
	%	\bigvee_{i=1,3, j=0,1,2,3 } (c_{ij}  \wedge c_{i+1,j}  )\\
	%
If $f$ is a tiling of $\N^2$ for $\boldsymbol{\cal C}$ tiles, we expand the standard grid model of $\phi_{grid}$ by taking 
any predicate $c \in \cC$ to be satisfied by $(i,j) \in \N^2$ just in case $f(i,j) = c$. It is a simple matter to check that 
$\eta_{\boldsymbol{\cal C}}$ is true in the resulting structure. Conversely, 
if $\fA \models \eta_{\boldsymbol{\cal C}}$, then $\fA \models \phi_{grid}$, and so 
there exists a grid embedding $\iota: \N^2 \rightarrow A$. We then define a function
$f: \N^2 \rightarrow {\cal C}$ by setting $f(i,j)$ to be the unique tile $c \in \cC$ such that $\fA \models c[\iota(i,j)]$,
which is well-defined by (6). By (7), $f$ is a tiling for $\boldsymbol{\cal C}$.

Indeed, the same argument shows that, $\eta_{\boldsymbol{\cal C}}$ has a {\em finite} model if and only if there is a {\em periodic} tiling 
of $\N^2$ for $\boldsymbol{\cal C}$. Since, remarked above, the set of tiling systems for which there exists no tiling of the plane is 
recursively inseparable from the set of tiling systems for which there exists a periodic tiling of the plane, we obtain:
\begin{theorem}
	The satisfiability problem and the finite satisfiability problems for $\mathcal{FL}^2_=2\mbox{\rm T}$ are both undecidable.
	\label{theo:twoEqUndecidable}
\end{theorem}
A quick check reveals that the formula $\eta_{\boldsymbol{\cal C}}$ lies in the guarded fragment of first-order logic. Moreover,
the proof of Lemma~\ref{lma:grid} would remain valid even if $r$ is required to be an equivalence relation. Thus we have:
\begin{corollary}
	The satisfiability problem and the finite satisfiability problems for the intersection of $\mathcal{FL}^2_=2\mbox{\rm T}$  with the two-variable guarded fragment are both undecidable. This result continues to hold if, in place of $\mathcal{FL}^2_=2\mbox{\rm T}$,
	we have $\mathcal{FL}^2_=1\mbox{\rm T}1\mbox{\rm E}$, the two-variable fluted fragment together with identity, one transitive relation and
	one equivalence relation. 
\label{cor:twoEqUndecidable}
\end{corollary}
%
%
%
%
%
\subsection{Undecidability of fluted logic with three transitive relations}\label{sec:twotrans}

In this section we assume that equality is not available in signatures and we show that the (finite) satisfiability problem for $\FLthreetrans$ are undecidable. 
We first prove the following theorem.
\begin{theorem}
	The satisfiability problem for $\FLthreetrans$, the two-variable fluted fragment with three transitive relations, is undecidable. 
	\label{th:three}
\end{theorem}

\begin{proof}
	%Now we want to show that without equality three transitive relations suffice to obtain undecidability of $\FLt{}$. 
	Suppose the signature contains transitive relations $b$ (black), $g$ (green)  and $r$ (red), and additional unary predicates $e$, $e'$, $bottom$, $\mathit{left}$, $c_{i,j}$ ($0\leq i\leq 5$, $0\leq j\leq 2$) and $d_{i,j}$ ($0\leq i \leq 2$, $0\leq j \leq 5$); we refer to the  $c_{i,j}$'s and to the $d_{i,j}$'s as {\em colours}. 
	%In the sequel, addition in subscripts of the $c_{i,j}$'s is
	%always understood modulo 6 in the first position, and modulo 3 in the second position, i.e. $c_{i+a,j+b}$ denotes $c_{(i+a)mod\; 6,(j+b)mod\; 3}$.
	%Similarly, addition in subscripts of the $d_{i,j}$'s is understood modulo 3 in the first position, and modulo 6 in the second position.
	% figure INTENDED MODEL
	

	
	We reduce from the $\N\times\N$ tiling problem. We first write a formula $\phi_{grid}$ that is an infinity axiom and  captures several properties of the intended expansion of the $\N\times\N$ grid  as shown 
	in Fig.~\ref{fig:grid-three-transitive:Left}. There the predicates $c_{i,j}$  and $d_{i,j}$ together define a partition of the universe as follows: 
	an element $(k,k')$ with $k'>k$ (i.e.~in the yellow region, above the diagonal) satisfies $c_{i,j}$ with $i=k\mod 6$, $j=k'\mod 3$, and an  element $(k,k')$ with $k\geq k'$ (i.e.~in the pink region, on or below the diagonal) satisfies $d_{i,j}$ with $i=k\mod 3, j=k'\mod 6$. 
	% Transitive relations connect elements that are `close' in the grid; more precisely,
	Paths of the same transitive relation have length at most 7 and follow one of designated patterns shown in Figure~\ref{fig:patterns}.
	 Remaining unary predicates mark the following elements: $\mathit{left}$---left column, $bottom$---bottom row, $e$---main diagonal, and  $e'$---elements with coordinates $(k,k+1)$. % (cf.~Figure~\ref{fig:grid-three-transitive}). 

	\begin{figure}[thb]
	\begin{center}
		%	\begin{minipage}{6.2cm}
		\begin{subfigure}[t]{0.54\textwidth}
			\begin{center}
				\resizebox{!}{4cm}
				{
					\begin{tikzpicture}[scale=0.95]
					
					\clip (-0.8,-0.8) rectangle (11.3,9.3);
					
					
					%%%% COLOURED REGIONS in Figure 2.
					\path [fill=myYellow] (0,0.5) to (9,9.5) to (0,9.5) to (0,0.5);
					\path [fill=myMelon] (0,0.5) to  (9,9.5) to (14.4,9.5) to (14.4,0) to (0,0) to (0,0.5);
					
					\draw [help lines] (0,0) grid (18,18);
					%		\draw (0,0) -- (18,18);
					
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=white] (\x, \y) circle (0.1); 
					}
					
					
					
					% pattern B
					\foreach \x in {1,7,13} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					\foreach \x in {3,9,15} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1); 
						\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					\foreach \x in {5,11} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					
					%			\foreach \x in {1,3,5,7,9,11,13,15} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					%				{
					%					\draw [|->, rounded corners, ultra thick, blue]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					%					\draw [->, ultra thick, dashed, blue] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					%				}
					
					
					% pattern C
					\foreach \y in {2,8,14} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					\foreach \y in {4,10,16} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					\foreach \y in {6,12,18} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					%									\foreach \y in {2,4,6,8,10,12,14,16} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					%									{
					%										\draw [|->, rounded corners, ultra thick, orange]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
					%										\draw [->, ultra thick, dashed, orange] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					%									}	
					
					%pattern A	
					
					\foreach \y in {3,9,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  red]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					\foreach \y in {5,11,17} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					\foreach \y in {1,7,13,20} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14,\y+17} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					%			\foreach \y in {1,3,5,7,9,11,13,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					%			{
					%				\draw [|->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
					%				\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					%			}
					%			
					
					%pattern D
					\foreach \x in {2,8,14} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
					\foreach \x in {4,10,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
					\foreach \x in {6,12} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  red]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, red] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
					
					%			\foreach \x in {2,4,6,8,10,12,14,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					%			{
					%				\draw [|->, rounded corners, ultra thick,  yellow]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
					%				\draw [->, ultra thick, dashed, yellow] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					%			}
					%			
					
					%bottom row
					
					\foreach \x in {0,3,6,9,12,15,18} \foreach \y in {0} \foreach \s in {0.1}
					{\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x+\s,\y) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					%left column
					
					\foreach \y in {1,4,7,10,13,16,19} \foreach \x in {0} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					
					\foreach \x in {0,3,6,9,12,15}
					\foreach \y in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=black] (\x, \y) circle (0.1); 
					}
					
					
					
					%labels
					%			\coordinate [label=center:$r_1$] (A) at ($(1.5,1.5)$);
					%			\coordinate [label=center:$r_2$] (A) at ($(2.5,2.5)$);
					%			\coordinate [label=center:$r_3$] (A) at ($(3.5,3.5)$);
					%			
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
					\end{tikzpicture}
				}
				%\vspace{0cm}
			\end{center} 
			\caption{the infinite grid}
			\label{fig:grid-three-transitive:Left}
		\end{subfigure}	
		%	\end{minipage}	
		%\hspace{0.6cm} 
	%	\vspace{-0.5cm}
		%				\begin{minipage}{6.5cm}
		\begin{subfigure}[t]{0.44\textwidth}					
			\begin{center}
				%	\vspace{-1cm}
				\resizebox{!}{4cm}
				{
					\begin{tikzpicture}[scale=0.95]
					
					\clip (-0.8,-0.8) rectangle (9.5,9.5);
					
					
					%%%% COLOURED REGIONS in Figure 2.
					\path [fill=myYellow] (0,0.5) to (8.5,9.0) to (0,9.0) to (0,0.5);
					\path [fill=myMelon] (0,0.5) to  (8.5,9.0) to (9.0,9.0) to (9.0,0) to (0,0) to (0,0.5);
					
					\draw [help lines] (0,0) grid (18,18);
					%		\draw (0,0) -- (18,18);
					
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=white] (\x, \y) circle (0.1); 
					}
					
					
					
					% pattern B
					\foreach \x in {1} \foreach \y in {\x,\x+3,\x+6}%,\x+9,\x+12,\x+15} 
					\foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
						\foreach \x in {7} \foreach \y in {\x}%,\x+9,\x+12,\x+15} 
					\foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					\foreach \x in {3}%,9,15} 
					\foreach \y in {\x,\x+3}%,\x+6,\x+9,\x+12,\x+15} 
					\foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1); 
						\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
				
					\foreach \x in {3} \foreach \y in {\x+6} \foreach \s in {0.1}
				{	\filldraw[fill=black] (\x, \y) circle (0.1); 
					\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s);% -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					\draw [->, ultra thick, dashed, black] (\x+\s,\y) -- (\x+1-\s,\y);
				}
				
					\foreach \x in {5,11} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					
					%			\foreach \x in {1,3,5,7,9,11,13,15} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
					%				{
					%					\draw [|->, rounded corners, ultra thick, blue]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					%					\draw [->, ultra thick, dashed, blue] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					%				}
					
					
					% pattern C
					\foreach \y in {2,8,14} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					\foreach \y in {4,10,16} \foreach \x in {\y+2}%,\y+5,\y+8,\y+11,\y+14} 
					\foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					\foreach \y in {6,12,18} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- %(\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- 
						(\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					}	
					
					%									\foreach \y in {2,4,6,8,10,12,14,16} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					%									{
					%										\draw [|->, rounded corners, ultra thick, orange]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
					%										\draw [->, ultra thick, dashed, orange] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
					%									}	
					
					%pattern A	
					
					\foreach \y in {3,9,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  red]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					\foreach \y in {5,11,17} \foreach \x in {\y+2}%,\y+5,\y+8,\y+11,\y+14} 
					\foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					\foreach \y in {1}%,7,13,20} 
					\foreach \x in {\y+2,\y+5}%,\y+8,\y+11,\y+14,\y+17} 
					\foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					\foreach \y in {1,7} \foreach \x in {9}%,\y+5,\y+8,\y+11,\y+14,\y+17} 
					\foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s); %-- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, green] (\x,\y+\s) -- (\x,\y+1-\s);
					}
					
					
					%			\foreach \y in {1,3,5,7,9,11,13,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
					%			{
					%				\draw [|->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
					%				\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					%			}
					%			
					
					%pattern D
					\foreach \x in {2}%,8,14} 
					\foreach \y in {\x,\x+3}%,\x+6,\x+9,\x+12} 
					\foreach \s in {0.1}
					{	\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
				
					\foreach \x in {2,8} \foreach \y in {8} \foreach \s in {0.1}
				{	\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) %-- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) 
					-- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
					\draw [->, ultra thick, dashed, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
				}
				
					\foreach \x in {4,10,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
					\foreach \x in {6,12} \foreach \y in {\x}%,\x+3,\x+6,\x+9,\x+12} 
					\foreach \s in {0.1}
					{	\filldraw[fill=red] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  red]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						\draw [->, ultra thick, dashed, red] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					}
					
					%			\foreach \x in {2,4,6,8,10,12,14,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
					%			{
					%				\draw [|->, rounded corners, ultra thick,  yellow]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
					%				\draw [->, ultra thick, dashed, yellow] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
					%			}
					%			
					
					%bottom row
					
					\foreach \x in {0,3,6}%,9,12,15,18} 
					\foreach \y in {0} \foreach \s in {0.1}
					{\filldraw[fill=black] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  black]  (\x+\s,\y) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
					}
					
					%left column
					
					\foreach \y in {1,4,7,10,13,16,19} \foreach \x in {0} \foreach \s in {0.1}
					{	\filldraw[fill=green] (\x, \y) circle (0.1);
						\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
					}
					
					
					\foreach \x in {0,3,6}%,9,12,15}
					\foreach \y in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=black] (\x, \y) circle (0.1); 
					}
					
					
					
					%labels
					%			\coordinate [label=center:$r_1$] (A) at ($(1.5,1.5)$);
					%			\coordinate [label=center:$r_2$] (A) at ($(2.5,2.5)$);
					%			\coordinate [label=center:$r_3$] (A) at ($(3.5,3.5)$);
					%			
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
					\end{tikzpicture}	
					
				}
			\end{center}
			\caption{the $\{0,\ldots 9\}\times \{0,\ldots,9\}$ grid.
			}
			\label{fig:grid-three-transitive:Finsat}
		\end{subfigure}
		%	\end{minipage}
		
	\end{center}
	
	\caption{Expansions of the grids in the proofs of, respectively, Theorem~\ref{th:three} (a) and Theorem~\ref{th:threeFinsat} (b).  Three transitive relations:  $b$,  {\color{green} $g$} and  {\color{red} $r$}. Filled nodes depict the beginning of a transitive path of the same colour; dotted lines connect the first element with the last element on such  path. 
	Paths of length 7 have four distinct patterns (cf.~Figure~\ref{fig:patterns}). For instance the same pattern A is followed by: the red path starting at node (5,3), the green path starting at node (3,1) and the black path starting at node (7,5). Paths starting at nodes (4,2), (8,6) and (6,4) follow  pattern B; paths starting at nodes (1,1), (5,5) and (3,3) follow pattern C; and paths starting at nodes (6,6), (4,4) and (2,2) follow pattern D. 
		Two shorter path patterns E and F appear on the left and bottom border; two additional shorter patterns appear on the right and top border in (b).
		%	\\
		%		Right picture:  two transitive relations {\color{blue}$b$}   and  {\color{red}$r$}. 
	}\label{fig:grid-three-transitive}
\end{figure}
	
	
	%	These patters will be enforced for each of the transitive relations at nodes satisfying certain colours.
	
	
	\begin{figure}[hbt] % PATH PATTERNS
		\begin{center}
			
			\resizebox{10.2cm}{!}{
				\begin{tikzpicture}[scale=1]
				
				\draw [help lines] (0,13) grid (15,15);
				
				% pattern B
				\foreach \x in {6} \foreach \y in {14} \foreach \s in {0.1}
				{	\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s)  -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
				}
				
				% pattern C
				\foreach \x in {3} \foreach \y in {15} \foreach \s in {0.1}
				{ \filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
					\draw [->, ultra thick, dashed] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
				}	
				
				
				%pattern A	
				\foreach \x in {1} \foreach \y in {13} \foreach \s in {0.1}
				{	\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
					\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
				}
				
				
				%pattern D
				\foreach \x in {11} \foreach \y in {13} \foreach \s in {0.1}
				{	\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
					\draw [->, ultra thick, dashed] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
				}
				
				%pattern E
				\foreach \x in {12} \foreach \y in {13} \foreach \s in {0.1}
				{	%\filldraw[myLavender]  (\x+\s,\y) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
					\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [->, rounded corners, ultra thick]  (\x+\s,\y) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
					\draw [->, ultra thick, dashed] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
				}
				
				
				% pattern F
				\foreach \x in {14} \foreach \y in {13} \foreach \s in {0.1}
				{	%\filldraw[myFuchsia] (\x,\y+\s) -- (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					\filldraw[fill=black] (\x, \y) circle (0.1);
					\draw [|->, rounded corners, ultra thick]  (\x,\y+\s) -- (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
					\draw [->, ultra thick, dashed] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
				}		
				
				
				%labels
				\coordinate [label=center:pattern A] (A) at ($(1.1,12.5)$);
				\coordinate [label=center:pattern B] (A) at ($(4.1,12.5)$);
				\coordinate [label=center:pattern C] (A) at ($(7.1,12.5)$);
				\coordinate [label=center:pattern D] (A) at ($(10.1,12.5)$);
				\coordinate [label=center:pattern E] (A) at ($(12.5,12.5)$);
				\coordinate [label=center:pattern F] (A) at ($(14.5,12.5)$);
				
				%			\foreach \x in {1,2,3,4,5,6,7,8,9} \pgfmathtruncatemacro{\abc}{mod(\x-1,3)} \coordinate [label=center:$_{\abc}$] (A) at (\x, 0.5);
				%			\foreach \y in {1,2,3,4,5,6,7} \pgfmathtruncatemacro{\abc}{mod(\y-1,3)} \coordinate [label=center:$_{\abc}$] (A) at (0.5,\y);
				%			
				\end{tikzpicture}
			}
			\vspace{0cm}		
		\end{center}
		
		\caption{Path patterns in the infinite grid. Solid lines show a path joining several adjacent nodes in a grid; filled nodes depict the first element of a path; dotted lines join the first element with the last element of a path. }\label{fig:patterns}
	\end{figure}
	
	
%	JESZCZE JEDEN OBRAZEK
%	
%		\begin{figure}[t]%{0.45\textwidth}					
%		\begin{center}
%			%	\vspace{-1cm}
%			\resizebox{5.5cm}{3.5cm}
%			{
%				\begin{tikzpicture}[xscale=0.8,yscale=0.8]
%				%
%				% 					\def{\z}{0.1}
%				\clip (-0.8,-0.8) rectangle (7.3,4.3);
%				\foreach \x in {1,3,5,7}
%				\foreach \y in {1,3,5,7} \foreach \z in {0.1} 
%				{
%					\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
%					(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
%					\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) --
%					(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
%					
%				}	
%				
%				\foreach \x in {0,2,4,6}
%				\foreach \y in {0,2,4,6} \foreach \z in {0.1} 
%				{
%					\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
%					(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
%					\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) --
%					(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
%				}	
%				
%				\foreach \x in {1,5}
%				\foreach \y in {1,5} \foreach \z in {0.15} 
%				{
%					\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
%					\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
%					\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
%					\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
%				}	
%				
%				\foreach \x in {3,7}
%				\foreach \y in {3,7} \foreach \z in {0.15} 
%				{
%					\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
%					\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
%					\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
%					\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
%				}	
%				
%				
%				\foreach \x in {1,5}
%				\foreach \y in {3,7} \foreach \z in {0.15} 
%				{
%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x, \y) ;
%					\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y);
%					\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y);
%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x, \y-1);						
%				}	
%				
%				\foreach \x in {3,7}
%				\foreach \y in {1,5} \foreach \z in {0.15} 
%				{
%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
%					\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
%					\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
%				}	
%				
%%				\foreach \x in {1,5}
%%				\foreach \y in {3,7} \foreach \z in {0.15} 
%%				{
%%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
%%					\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
%%					\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
%%					\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
%%				}	
%%				
%%				
%				
%				
%				\foreach \x in {0,1,2,3,4,5,6,7}
%				\foreach \y in {0,1,2,3,4,5,6,7}
%				{
%					\filldraw[fill=white] (\x, \y) circle (0.1); 
%					\pgfmathtruncatemacro{\abc}{mod(\y,4)} 
%					\pgfmathtruncatemacro{\bcd}{mod(\x,4)} 
%	%				\coordinate [label=center:$_{\bcd\abc}$] (A) at (\x,\y);
%				}
%				
%				
%				%	\foreach \x in {1,2,3,4,5,6} \pgfmathtruncatemacro{\abc}{\x-1} \coordinate [label=center:$_{\abc}$] (A) at (\x, 1.5);
%				%	\foreach \y in {1,2,3,4,5} \pgfmathtruncatemacro{\abc}{\y-1} \coordinate [label=center:$_{\abc}$] (A) at (0.5,\y+1);
%				
%				\draw[ ->, dotted, very thick] (7.5,0) -- (8,0);
%				\draw[ ->, dotted, very thick] (0,7.5) -- (0,8);
%				\draw[ ->, dotted, very thick] (7.5,7.5) -- (8,8);
%				
%				% 					\coordinate [label=center:$b$] (A) at (1.5,1.8);
%				% 					\coordinate [label=center:$\color{cyan}c$] (A) at (1.5,2.2);
%				% 					\coordinate [label=center:$\color{green}g$] (A) at (2.5,1.8);
%				% 					\coordinate [label=center:$\color{red}r$] (A) at (2.5,2.2);
%				
%				 	\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
%				 	\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
%				 					
%				\end{tikzpicture}
%				
%			}
%		\end{center}
%		\caption{two transitive relations: {\color{blue}$b$}   and  {\color{red}$r$}. Edges without arrows depict connections in both direction. Nodes are marked by the indices of  the $c_{ij}$s they satisfy. }
%	\end{figure}
%	%	\end{minipage}
%	
%	
%	
%	KONIEC OBRAZKA
	
	\begin{figure}[hbt]
	\begin{subfigure}[t]{0.45\textwidth}	
		\begin{center}
			\begin{minipage}{5.5cm}
				\begin{center}
					%\resizebox{11.2cm}{!}
					{

						
						
						\begin{tikzpicture}[scale=0.7]
						
						\clip (-0.8,-0.8) rectangle (7.3,7.3);
						
						\draw [help lines] (0,0) grid (18,18);
						\draw [gray, dotted] (0,0) -- (18,18);
						
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=white] (\x, \y) circle (0.1); 
						}
						
						%first edge 		
						\draw[ultra thick, ->, black] (0,0) -- (0,1);
						
						% diagonal		
						%	\foreach \x in {1,7,13} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
						\foreach \x in {1} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
						\foreach \x in {2,8,14} \draw[ultra thick, ->, red] (\x,\x) -- (\x-1,\x);
						\foreach \x in {3,9,15} \draw[ultra thick, <-, green] (\x,\x) -- (\x-1,\x);
						\foreach \x in {4,10,16} \draw[ultra thick, ->, black] (\x,\x) -- (\x-1,\x);
						\foreach \x in {5,11,17} \draw[ultra thick, <-, red] (\x,\x) -- (\x-1,\x);
						%	\foreach \x in {6,12,18} \draw[ultra thick, ->, green] (\x,\x) -- (\x-1,\x);
						
						% below the diagonal i.e. x=y+3k, k>0
						
						\foreach \y in {5,11,17} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						\foreach \y in {2,8,14} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						\foreach \y in {4,10,16} \foreach \x in {\y} %,\y+3,\y+6,\y+9,\y+12,\y+15} 
						\draw[ultra thick, <-, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						%	\foreach \y in {7,13} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						\foreach \y in {1} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1);
						
						\foreach \y in {3,9,15} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						%	\foreach \y in {6,12,18} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						% above the diagonal i.e. x=y+3k, k>0
						
						\foreach \x in {3,9,15} \foreach \y in {\x+1}%,\x+4,\x+7,\x+10,\x+13,\x+16} 
						\draw[ultra thick, ->, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						%					\foreach \x in {6,12,18} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						
						\foreach \x in {4,10,16} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {7,13} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {1} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y);
						
						%	\foreach \x in {5,11,17} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {2,8,14} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						
						% left edges	
						\foreach \x in {0} \foreach \y in {2,5,8,11,14,17} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y+2);
						
						%bottom edges
						\foreach \y in {0} \foreach \x in {1,4,7,10,13,16} \draw[ultra thick, ->, red] (\x,\y) -- (\x+2,\y);
						
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
						
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=white] (\x, \y) circle (0.1); 
						}
						
						
						\foreach \x in {0,1} %,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=YellowOrange] (\x, \x) circle (0.1); 
						}
						\foreach \x in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=yellow] (\x, \x+1) circle (0.1); 
						}
						
						
						%			
						\end{tikzpicture}
					}
				\end{center}
			\end{minipage}
		\end{center}
	\caption{Path starting with an initial element and generated by witnesses for conjuncts of group (3). 
		%Arrows indicate nodes where the zig-zag path crosses the diagonal or where its definition switches from one transitive relation to another.
	}
		\label{fig:embeddingLeft}
	\end{subfigure}
	\hspace{0.05\textwidth}
	\begin{subfigure}[t]{0.45\textwidth}	
		\begin{center}
			\begin{minipage}{5.5cm}
				\begin{center}
					%	\resizebox{11.2cm}{!}
					{
						\begin{tikzpicture}[scale=0.7]
						
						\clip (-0.8,-0.8) rectangle (7.3,7.3);
						
						\draw [help lines] (0,0) grid (18,18);
						%		\draw (0,0) -- (18,18);
						
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=white] (\x, \y) circle (0.1); 
						}
						
						
						
						% pattern B
						
						\foreach \s in {0.15}
						{			\draw [->, ultra thick, dashed, red] (1+\s,1+\s) -- (1+\s,1+1-\s-\s);
							\draw [->, ultra thick, red] (1+\s,1-\s) -- (1+\s,0+\s);
						}
						
						%	\foreach \x in {1,7,13} \foreach \y in {\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
						\foreach \x in {1} \foreach \y in {\x+3} \foreach \s in {0.15}
						{	%\filldraw[fill=red] (\x, \y) circle (0.1);
							\draw [->,  ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s);
							\draw [->,  ultra thick, red] (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s);
							\draw [->,  ultra thick, red] (\x+1+\s,\y-1+\s) -- (\x+2-\s,\y-1+\s);
							\draw [->,  ultra thick, red] (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s);
							% -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
							\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
							%
						}
						
						%	\foreach \x in {3,9,15} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
						\foreach \x in {3} \foreach \y in {\x} \foreach \s in {0.15}
						{	%\filldraw[fill=black] (\x, \y) circle (0.1); 
							\draw [->,  ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s);
							\draw [->,  ultra thick, black] (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s);
							\draw [->,  ultra thick, black] (\x+1+\s,\y-1+\s) -- (\x+2-\s,\y-1+\s);
						% one more edges erased	
						 %	\draw [->,  ultra thick, black] (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s);
							% -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
							\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
							
							%\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
							%\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
						}
						%			\foreach \x in {5,11} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
						%			{	%\filldraw[fill=green] (\x, \y) circle (0.1);
						%				\draw [->,  ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s);
						%				\draw [->,  ultra thick, green] (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s);
						%				\draw [->,  ultra thick, green] (\x+1+\s,\y-1+\s) -- (\x+2-\s,\y-1+\s);
						%				\draw [->,  ultra thick, green] (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s);
						%				% -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						%				\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
						%				%
						%				%\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						%				%\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
						%			}
						%			
						
						%			\foreach \x in {1,3,5,7,9,11,13,15} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12,\x+15} \foreach \s in {0.1}
						%				{
						%					\draw [|->, rounded corners, ultra thick, blue]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s) -- (\x+2-\s,\y-1+\s) -- (\x+2-\s,\y-\s) -- (\x+1-\s,\y-\s) -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
						%					\draw [->, ultra thick, dashed, blue] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
						%				}
						
						
						% pattern C
						
						%			\foreach \y in {2} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						\foreach \y in {2} \foreach \x in {\y+2} \foreach \s in {0.15}
						{	%\filldraw[fill=red] (\x, \y) circle (0.1);
							\draw [->, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s);
							\draw [->, ultra thick, red] (\x+\s,\y-1-\s) -- (\x+\s,\y-2+\s);
							% -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
							\draw [->, ultra thick, dashed, red] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
						}	
						
						%			\foreach \y in {8,14} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%			{	\filldraw[fill=red] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						%				\draw [->, ultra thick, dashed, red] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
						%			}	
						
						%			\foreach \y in {4,10,16} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%			{	\filldraw[fill=black] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						%				\draw [->, ultra thick, dashed, black] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
						%			}	
						
						%			\foreach \y in {6,12,18} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%			{	\filldraw[fill=green] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						%				\draw [->, ultra thick, dashed, green] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
						%			}	
						
						%									\foreach \y in {2,4,6,8,10,12,14,16} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%									{
						%										\draw [|->, rounded corners, ultra thick, orange]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s) -- (\x+2-\s,\y-2+\s) -- (\x+2-\s,\y-1-\s) -- (\x+1-\s,\y-1-\s) -- (\x+1-\s,\y-\s);
						%										\draw [->, ultra thick, dashed, orange] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
						%									}	
						
						%pattern A	
						
						%			\foreach \y in {3,9,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						\foreach \y in {3,9,15} \foreach \x in {\y+2} \foreach \s in {0.15}
						{	%\filldraw[fill=red] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  red]  (\x-\s,\y+\s) -- (\x-1+\s,\y+\s);
							\draw [->, ultra thick,  red] (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s);
							\draw [->, ultra thick,  red] (\x-1+\s,\y+1+\s) -- (\x-1+\s,\y+2-\s);
							% -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick, dashed, red] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						}
						
						%			\foreach \y in {5,11,17} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%			{	\filldraw[fill=black] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						%				\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						%			}
						\foreach \y in {1} \foreach \x in {\y+2} \foreach \s in {0.15}
						{%	\filldraw[fill=green] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  green]  (\x-\s,\y+\s) -- (\x-1+\s,\y+\s);
							\draw [->, ultra thick,  green] (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s);
							\draw [->, ultra thick,  green] (\x-1+\s,\y+1+\s) -- (\x-1+\s,\y+2-\s);
							%\draw [->, ultra thick,  green] (\x-1+\s,\y+2-\s)  -- (\x-\s,\y+2-\s);
							% -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
							
							%\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							%\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						}
						
						\foreach \y in {1,7,13,20} \foreach \x in {\y+5,\y+8,\y+11,\y+14,\y+17} \foreach \s in {0.15}
						{%	\filldraw[fill=green] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  green]  (\x-\s,\y+\s) -- (\x-1+\s,\y+\s);
							\draw [->, ultra thick,  green] (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s);
							\draw [->, ultra thick,  green] (\x-1+\s,\y+1+\s) -- (\x-1+\s,\y+2-\s);
							\draw [->, ultra thick,  green] (\x-1+\s,\y+2-\s)  -- (\x-\s,\y+2-\s);
							% -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
							
							%\draw [->, rounded corners, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							%\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						}
						
						
						%			\foreach \y in {1,3,5,7,9,11,13,15} \foreach \x in {\y+2,\y+5,\y+8,\y+11,\y+14} \foreach \s in {0.1}
						%			{
						%				\draw [|->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-1+\s,\y+1-\s) -- (\x-1+\s,\y+2-\s) -- (\x-\s,\y+2-\s) -- (\x-\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
						%				\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						%			}
						%			
						
						%pattern D
						\foreach \x in {2} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.15}
						{	%\filldraw[fill=black] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  black]  (\x-\s,\y+\s) -- (\x-1+\s,\y+\s);
							\draw [->, ultra thick,  black]  (\x-1-\s,\y+\s) -- (\x-2+\s,\y+\s);
							% -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
							\draw [->, ultra thick, dashed, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
						}
						
						%			\foreach \x in {8,14} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
						%			{	\filldraw[fill=black] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick,  black]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						%				\draw [->, ultra thick, dashed, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
						%			}
						%			\foreach \x in {4,10,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
						\foreach \x in {4,10,16} \foreach \y in {\x} \foreach \s in {0.15}
						{	%\filldraw[fill=green] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  green]  (\x,\y+\s) -- (\x-1+\s,\y+\s); 
							\draw [->, ultra thick,  green] (\x-1-\s,\y+\s) -- (\x-2+\s,\y+\s);
							\draw [->, ultra thick,  green] (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s); 
							\draw [->, ultra thick,  green] (\x-2+\s,\y+1+\s) -- (\x-2+\s,\y+2-\s);
							% -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
							\draw [->, ultra thick, dashed, green] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
						}
						%			\foreach \x in {6,12} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
						%			{	\filldraw[fill=red] (\x, \y) circle (0.1);
						%				\draw [->, rounded corners, ultra thick,  red]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						%				\draw [->, ultra thick, dashed, red] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
						%			}
						%			
						%			\foreach \x in {2,4,6,8,10,12,14,16} \foreach \y in {\x,\x+3,\x+6,\x+9,\x+12} \foreach \s in {0.1}
						%			{
						%				\draw [|->, rounded corners, ultra thick,  yellow]  (\x,\y+\s) -- (\x-1+\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s) -- (\x-2+\s,\y+2-\s) -- (\x-1-\s,\y+2-\s) -- (\x-1-\s,\y+1-\s) -- (\x-\s,\y+1-\s);
						%				\draw [->, ultra thick, dashed, yellow] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
						%			}
						%			
						
						%bottom row
						
						\foreach \x in {0} \foreach \y in {0} \foreach \s in {0.15}
						{%\filldraw[fill=black] (\x, \y) circle (0.1);
							%\draw [->, rounded corners, ultra thick,  black]  (\x+\s,\y) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s) -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						}
						
						
						\foreach \x in {3,6,9,12,15,18} \foreach \y in {0} \foreach \s in {0.15}
						{%\filldraw[fill=black] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  black]  (\x+\s,\y) -- (\x+\s,\y+1-\s);
							\draw [->, ultra thick,  black]  (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s);
							% -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick, dashed, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
						}
						
						%left column
						
						\foreach \y in {1,4} \foreach \x in {0} \foreach \s in {0.15}
						{	%\filldraw[fill=green] (\x, \y) circle (0.1);
							\draw [->, ultra thick,  green]  (\x,\y+\s) -- (\x+1-\s,\y+\s);
							\draw [->, ultra thick,  green] (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s);
							% -- (\x+\s,\y+1-\s);
							\draw [->, ultra thick, dashed, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
						}
						
						
						\foreach \x in {0,3,6,9,12,15}
						\foreach \y in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=black] (\x, \y) circle (0.1); 
						}
						
						
						%first edge 		
						\draw[ultra thick, ->, black] (0,0) -- (0,1);
						
						% diagonal		
						\foreach \x in {1} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
						\foreach \x in {2,8,14} \draw[ultra thick, ->, red] (\x,\x) -- (\x-1,\x);
						\foreach \x in {3,9,15} \draw[ultra thick, <-, green] (\x,\x) -- (\x-1,\x);
						\foreach \x in {4,10,16} \draw[ultra thick, ->, black] (\x,\x) -- (\x-1,\x);
						\foreach \x in {5,11,17} \draw[ultra thick, <-, red] (\x,\x) -- (\x-1,\x);
						%		\foreach \x in {6,12,18} \draw[ultra thick, ->, green] (\x,\x) -- (\x-1,\x);
						
						% below the diagonal i.e. x=y+3k, k>0
						
						\foreach \y in {5,11,17} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						\foreach \y in {2,8,14} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						\foreach \y in {4} \foreach \x in {\y} \draw[ultra thick, <-, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						%		\foreach \y in {7,13} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						\foreach \y in {1} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1);
						
						\foreach \y in {3,9,15} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						%		\foreach \y in {6,12,18} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
						
						% above the diagonal i.e. x=y+3k, k>0
						
						%	\foreach \x in {3,9,15} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {3,9,15} \foreach \y in {\x+1} \draw[ultra thick, ->, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						
						%	\foreach \x in {6,12,18} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						
						\foreach \x in {4,10,16} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {7,13} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {1} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y);
						
						%		\foreach \x in {5,11,17} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						\foreach \x in {2,8,14} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
						
						% left edges	
						\foreach \x in {0} \foreach \y in {2,5,8,11,14,17} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y+2);
						
						%bottom edges
						\foreach \y in {0} \foreach \x in {1,4,7,10,13,16} \draw[ultra thick, ->, red] (\x,\y) -- (\x+2,\y);
						
						
						%labels
						%			\coordinate [label=center:$r_1$] (A) at ($(1.5,1.5)$);
						%			\coordinate [label=center:$r_2$] (A) at ($(2.5,2.5)$);
						%			\coordinate [label=center:$r_3$] (A) at ($(3.5,3.5)$);
						%			
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
						
						\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=white] (\x, \y) circle (0.1); 
						}
						
						\foreach \x in {0,1,2,3,4,5} %,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=YellowOrange] (\x, \x) circle (0.1); 
						}
						\foreach \x in {0,1,2,3,4} %,6,7,8,9,10,11,12,13,14,15,16,17}
						{
							\filldraw[fill=yellow] (\x, \x+1) circle (0.1); 
						}
						
						
						\end{tikzpicture}
					}	
				\end{center}
			\end{minipage}
		\end{center}
	\caption{Additional edges arising from conjuncts of group (4) (solid lines drawn inside grid cells) and transitivity (dashed lines). Nodes on the diagonals  are marked orange ($e$) and  yellow ($e'$).}
	\label{fig:embeddingRight}
\end{subfigure}
		\caption{Construction of the intended model of $\phi_{grid}$ % with universe $\N\times \N$ 
			in the proof of Theorem~\ref{th:three}.}
		\label{fig:embedding}
	\end{figure}
	
	
	The formula $\phi_{grid}$ comprises a large number of conjuncts. To help give an overview of the construction, we have organized these conjuncts into groups, each of which secures a particular property (or collection of properties) exhibited by its models.
	The first two properties are very simple:
	\begin{enumerate}
		\item[(1)] There is an `initial' element satisfying $d_{00}  \wedge e  \wedge \mathit{left} \wedge bottom $.\label{rgb:initial}
		%		
		\item[(2)] The predicates $c_{i,j}$ and $d_{i,j}$ together partition the universe.
	\end{enumerate}	
	%
	The third property generates the path shown in Fig.~\ref{fig:embeddingLeft}:%\nb{L to be fixed: correct reference, wrong number}
	\begin{enumerate}
		\item[(3)] Each element has a $b$- $r$- or $g$- successor as shown in the path shown in Fig.~\ref{fig:embeddingLeft}, and satisfying the appropriate predicates $c_{i,j}$ or $d_{i,j}$. Specifically, if a node in this path has coordinates $(x,y)$ with $y > x$,  	
		then it satisfies $c_{i,j}$ where $i = x \mod 3$ and $j = y \mod 6$; %if a node in this path has coordinates $(x,y)$ with 
		and when $y \leq x$, then the node satisfies $d_{i,j}$ where $i = x \mod 3$ and $j = y \mod 6$.
	\end{enumerate}
	The conjuncts enforcing this property have the form
	% Conjuncts from this group have the following form:
	\begin{equation}
	\forall  \big( colour \wedge diag \wedge border  \rightarrow \exists  (t \wedge colour' )\big),\tag{3a}\label{tiling:rgb:witnesses}
	\end{equation}
	where $colour$ and $colour'$ stand for one of the predicate letters $c_{i,j}$ or $d_{i,j}$, $diag $ stands for one of the literals $e' $, $\neg e' $, $e $, $\neg e $ or $\top$  (i.e.~the logical constant true), $border $ stands for one of the literals $\mathit{left} $, $\neg \mathit{left} $, $bottom $, $\neg bottom $ or $\top$, and  $t$ stands for one of the transitive predicate letters $b$, $r$ or $g$. 
	%
	The precise combinations of the literals and predicate letters in these conjuncts can be read from Fig.~\ref{fig:embeddingLeft} (cf.~Table~\ref{table:witnesses} for a full list). 
	%

%\subsection{Table defining conjuncts in group (3) of the proof of Theorem~\ref{th:three}}
%\nb{L to be decided where to put this}
\begin{table}[tbh]
	\begin{center}
		\begin{minipage}{12cm}
			\begin{minipage}{0.45\textwidth}
				\begin{center}
					
					$	\begin{array}{c|c|c|c|c}
					colour \quad & diag &  border	&  t & colour'\\
					\hline
					
					d_{00}	&	e		&   \text{\it left}		& 	b	& 	c_{01}\\
					d_{00}	&	e		&   \neg \mathit{left}	& 	g	& 	c_{50}\\
					d_{14}	&	e		&   		& 	b	& 	c_{31}\\
					d_{22}	&	e		&  			& 	r	& 	c_{12}\\
					
					\hline
					
					%do gory	
					
					d_{00}	&	\neg e	& 	 		& 	r	& 	d_{01}\\
					d_{01}	&			&   		& 	r	& 	d_{21}\\
					d_{21}	&			&   		& 	r	& 	d_{22}\\
					d_{22}	&	\neg e	&   		& 	b	& 	d_{23}\\
					
					d_{23}	&			&   		& 	b	& 	d_{13}\\
					d_{13}	&			&   		& 	b	& 	d_{14}\\
					d_{14}	&	\neg e	&   		& 	g	& 	d_{15}\\
					
					d_{15}	&			&   		& 	g	& 	d_{05}\\
					d_{05}	&			&   		& 	g	& 	d_{00}\\
					\hline
					
					% 	w doł 
					d_{11}	&	\		&   		& 	b	& 	d_{10}\\
					d_{10}	&			&   \neg bottom	& 	b	& 	d_{20}\\
					
					d_{20}	&			&  \neg bottom & 	b	& 	d_{25}\\
					
					d_{25}	&			&   		& 	r	& 	d_{24}\\
					d_{24}	&			&   		& 	r	& 	d_{04}\\
					
					d_{04}	&			&   		& 	r	& 	d_{03}\\
					
					d_{03}	&			&   		& 	g	& 	d_{02}\\
					d_{02}	&			&   		& 	g	& 	d_{12}\\
					d_{12}	&			&   		& 	g	& 	d_{11}\\
					
					\hline
					d_{20}	&			&   bottom	& 	r	& 	d_{00}\\
					d_{10}	&			&    bottom	& 	r	& 	d_{20}\\
					
					
				\end{array}$
				\end{center}
				\end{minipage}
				\hspace{0.5cm}	
				%% PRAWA POLOWA TABLICY
				\begin{minipage}{0.45\textwidth}
				\begin{center}
				
				
				$	\begin{array}{c|c|c|c|c}
				colour \quad & diag &  border	&  t & colour'\\
				\hline
				&			&  			& 		& 	\\
				c_{01}	&	 e'		&   		& 	b	& 	d_{11}\\
				c_{20}	&	e'		&   		& 	g	& 	d_{03}\\
				c_{42}	&	e'		&   		& 	r	& 	d_{25}\\
				\hline
				
				% 	w doł 
				c_{01}	&	\neg e'	&   		& 	b	& 	c_{11}\\
				c_{11}	&			&   		& 	b	& 	c_{10}\\
				c_{10}	&			&   		& 	b	& 	c_{20}\\
				
				c_{20}	&	\neg e'	&   		& 	g	& 	c_{30}\\
				c_{30}	&			&   		& 	g	& 	c_{32}\\
				c_{32}	&			&   		& 	g	& 	c_{42}\\
				
				c_{42}	&	\neg e'	&   		& 	r	& 	c_{52}\\
				c_{52}	&			&   		& 	r	& 	c_{51}\\
				c_{51}	&			&   		& 	r	& 	c_{01}\\
				\hline
				
				
				%do gory	
				c_{12}	&			&   		& 	g	& 	c_{02}\\
				c_{02}	&			&   \neg \mathit{left}	& 	g	& 	c_{00}\\
				c_{00}	&			&   \neg \mathit{left}	& 	g	& 	c_{50}\\
				
				c_{50}	&			&   		& 	b	& 	c_{40}\\
				c_{40}	&			&   		& 	b	& 	c_{41}\\
				c_{41}	&			&   		& 	b	& 	c_{31}\\
				
				c_{31}	&			&   		& 	r	& 	c_{21}\\
				c_{21}	&			&   		& 	r	& 	c_{22}\\
				c_{22}	&			&   		& 	r	& 	c_{12}\\
				\hline
				
				c_{02}	&			& \mathit{left} 		& 	b	& 	c_{00}\\
				c_{00}	&			& \mathit{left} 		& 	b	& 	c_{01}				
			\end{array}$
			\end{center}
			\end{minipage}
			\end{minipage}
			\end{center}
			
			\caption{Table defining conjuncts in group (3) of the proof of Theorem~\ref{th:three}. Various combinations of the literals in conjuncts of the form \eqref{tiling:rgb:witnesses}; empty entries in columns $diag$ or $border$ mean $\top$. }
			\label{table:witnesses}
		\end{table}
		

	
%	In Figure~\ref{fig:embeddingLeft} we do not draw edges resulting from transitivity of the predicates $b$, $g$ and $r$. However, 
To connect all pairs of elements that are neighbours in the standard grid we require a fourth property, which
we give in schematic form as follows:
	%	
	\begin{enumerate}
		%\item transitive paths do not connect distinct elements of the same colour: DELETE
		%	\begin{eqnarray}
		%	\bigwedge_{0\leq i,j\leq 3} \forall x (c_{ij} \rightarrow \forall y ((b \vee r )\wedge c_{ij}  \rightarrow x=y))\label{Clique}
		%	%	\bigwedge_{0\leq i,j\leq 3} \forall x (c_{ij} \rightarrow \forall y (b \wedge c_{ij}  \rightarrow x=y))
		%	\end{eqnarray}
		
		\item[(4)]\label{IfBlack}
		{\em Certain} pairs of elements connected by \textit{one} transitive relation are also connected by \textit{another}, as indicated in Fig.~\ref{fig:embeddingRight}. % and as shown in the right-hand picture of Figure~\ref{fig:embedding}; 
\end{enumerate}		
Here are some examples of the conjuncts enforcing this property:
\begin{align}
		%
		\forall  (c_{01}  &\rightarrow \forall  (b \wedge (c_{11}  \vee d_{11} ) \rightarrow g \wedge \neg r )),\tag{4a}\label{tiling:4a}\\
		\forall  (d_{11}  &\rightarrow \forall  (b \wedge d_{10} \rightarrow r \wedge \neg g)),\tag{4b}\label{tiling:4b} \\
		\forall  (d_{11}  &\rightarrow \forall  (r \wedge (c_{12} \vee d_{12} )\rightarrow g \wedge \neg b )),\tag{4c}\label{tiling:4c}\\
		% \wedge \nonumber\\
		\forall  (c_{21}  &\rightarrow \forall  (r \wedge (c_{22} \vee d_{22} )\rightarrow g \wedge \neg b)), \tag{4d}\label{tiling:4d}\\
		\forall  (d_{22}  &\rightarrow \forall  (r \wedge d_{12} \rightarrow b \wedge \neg g)).\tag{4e}\label{tiling:4e}
		%
		\end{align}
		%
These conjuncts are organised in such a way that in the intended model elements from two adjacent columns or two adjacent rows 	are connected by at most two distinct transitive relations: rows $3i$  and $3i+1$ are not connected by any green edge, rows $3i+1$ and $3i+2$---by any black edge, rows $3i+2$ and $3i$---by any red edge; similarly, columns $3i$  and $3i+1$ are not connected by any red edge, columns $3i+1$ and $3i+2$---by any green edge, and columns $3i+2$ and $3i$---by any black edge. 


%Finally, to ensure that the elements connect in the expected way we add the 
The role of these conjuncts can be explained referring to Fig.~\ref{fig:embeddingRight}.
For example, employing \eqref{tiling:4b} for the element $(1,1)$ in the intended model $\fG$, we get $\fG\models r((1,1),(1,0))$; hence by transitivity of $r$, also $\fG\models r((1,1),(1,2))$. This, applying \eqref{tiling:4c}, implies $\fG\models g((1,1),(1,2))$. By \eqref{tiling:4a}, we get $\fG \models g((0,1),(1,1))$ and, by transitivity of $g$, $\fG\models g((0,1),(0,2))$. The process is illustrated in Fig.~\ref{fig:embeddingRight}; when carried on along the zig-zag path, it constructs a grid-like structure. 

These conjuncts depend on having available the predicates marking the borders and the diagonals. Specifically, we require the following
property\footnote{Addition in subscripts of the $c_{i,j}$'s is
	always understood modulo 6 in the first position, and modulo 3 in the second position, i.e. $c_{i+a,j+b}$ denotes $c_{(i+a)\,\mathsf{mod}\: 6,(j+b)\,\mathsf{mod}\: 3}$.
	Similarly, addition in subscripts of the $d_{i,j}$'s is understood modulo 3 in the first position, and modulo 6 in the second position.}
:\nb{L beginning of changes} 
	%
	\begin{enumerate}
		%	\item[(2)] there is an initial element: $\exists x (d_{00}  \wedge e  \wedge l \wedge f )$.\label{rgb:initial}
		%		
		%	\item[(3)] the predicates $c_{i,j}$ together with $d_{i,j}$ enforce a partition of the universe.
		%	
		\item[(5)] the predicates $\mathit{left}$, $bottom$, $e$ and $e'$ are distributed to mark the left-most column, the first row, the diagonal and
		the `super-diagonal'  
		of the grid, as indicated above. To secure this property, we add  to $\phi_{grid}$ several conjuncts, for instance:
	\end{enumerate}
	\begin{align}
	%
\bigwedge_{0\leq i\leq 2,\; 0\leq j\leq 5}  \forall (d_{ij}	\wedge \pm e & \rightarrow \forall  ((b \vee g  \vee r )\wedge d_{i+1,j+1}  \rightarrow \pm e)) \tag{5a}\label{tiling:e}\\
%	
\bigwedge_{0\leq j \leq 5} \forall  \big(c_{0j} \wedge \pm \mathit{left} & \rightarrow \forall  ((b \vee g \vee r )\wedge c_{0,j+1}  \rightarrow \pm \mathit{left} ) \big)
\tag{5b}\label{tiling:left} \\
% \\
\bigwedge_{0\leq i \leq 2} \forall  \big(d_{i0} \wedge \pm \mathit{bottom} & \rightarrow \forall  ((b \vee g \vee r )\wedge d_{i+1,0}  \rightarrow \pm \mathit{bottom} ) \big)
\tag{5c}\label{tiling:bot} 
\end{align}
where $\pm e $ denotes uniformly $e $ or $\neg e $, etc. 

Additional  conjuncts are added for the super-diagonal and also for the connections with and between $e'$ and $e$. For instance,  for every $i$ ($0\leq i\leq 2$) and $j$ ($0\leq j\leq 5$) we add
%
		\begin{align}
	%\bigwedge_{0\leq i\leq 2,\; 0\leq j\leq 5}
	\forall ((d_{ij} \wedge e  & \rightarrow \forall  ((b \vee g  \vee r )\wedge \bigvee_{(k,l)\not\in \{(i+1,j+1),(i-1,j-1)\}} d_{k,l} \rightarrow \neg e))	\tag{5d}\label{tiling:enot}\\
	\forall  ((d_{ij} \wedge e  &\rightarrow \forall  ((b \vee g  \vee r )\wedge (c_{i-1,j}\vee c_{i+2,j}) ))  \rightarrow e'))\tag{5e}\label{tiling:eprim}.
%	\bigwedge_{0\leq i\leq 2,\; 0\leq j\leq 5}
%\end{split}
\end{align}

	
The conjuncts ensuring properties (4) and (5) work in tandem.
For instance, applying~\eqref{tiling:e} to (1,1) we get $e$ is true at $(2,2)$; then, following the zig-zag path and applying more conjuncts from the group (4), we get that $g((2,2),(3,3))$ holds, so the node $(3,3)$ will be marked by $e$; this will propagate along the main diagonal. 

Finally, we require that
	\begin{enumerate}
	\item[(6)] the intersection of all three transitive relations is empty:\nb{L looks redundant}
	$$  \forall  \forall \neg (b \wedge g \wedge r).$$  
	\item[(7)] Certain pairs of elements are not connected by certain transitive relations, for instance: 
	\begin{align}
&\forall  (d_{22} \rightarrow  \forall( c_{12} \rightarrow \neg g)) \tag{7a}\label{forbidden:7a} \\
%&\forall  (d_{12} \rightarrow  \forall( d_{22} \wedge e \rightarrow \neg r)) \tag{7b}\label{forbidden:7b} \\
&\forall  (e' \wedge c_{31} \rightarrow  \forall( d_{03} \rightarrow \neg g)) \tag{7c}\label{forbidden:7c} 
%&\forall  (d_{04} \rightarrow  \forall( d_{03} \wedge e \rightarrow \neg r)) \tag{7d}\label{forbidden:7d} \\
%&\forall  (d_{25} \wedge e  \rightarrow \forall( d_{14} \wedge e \rightarrow \neg g)) \tag{7e}\label{forbidden:7e} 
%
%
\end{align}

	\item[(8)] Certain pairs of elements are not connected by any transitive relation: 
	\begin{align}
&\forall  (d_{i-1,j} \rightarrow  \forall( d_{i,j} \wedge e \rightarrow \neg (b \vee g \vee r)) \tag{8a}\label{forbidden8a}\\
&\forall  (d_{i,j} \rightarrow \forall( d_{i-1,j-1} \rightarrow \neg (b \vee g \vee r)). \tag{8b}\label{forbidden8b}\\
&\forall  (d_{i,j+1} \rightarrow  \forall( d_{i,j} \wedge e \rightarrow \neg (b \vee g \vee r)) \tag{8c}\label{forbidden8c}
%&\forall  (d_{12} \wedge  \forall( d_{22} \wedge e \rightarrow \neg r)) \tag{8a}\label{forbiddenSb} \\
%&\forall  (e' \wedge c_{31} \wedge  \forall( d_{03} \rightarrow \neg g)) \tag{7a}\label{forbiddenSc} \\
%&\forall  (d_{04} \wedge  \forall( d_{03} \wedge e \rightarrow \neg r)) \tag{7a}\label{forbiddenSd} 
%
\end{align}

	
\end{enumerate}

	{\em Claim.} The sentence $\phi_{grid}$ is satisfiable, but not finitely satisfiable. \\
%	
\textit{Proof:}
The structure $\fG$ depicted in Fig.~%\ref{fig:grid-three-transitive}.(a)
\ref{fig:grid-three-transitive:Left}
 is a model of $\phi_{grid}$.  
 
  Now let $\fA\models \phi_{grid}$. 
 Let $next:\N\times\N \mapsto \N\times \N$ be the successor function defined on $\N\times\N$ as depicted by the zig-zag path in the left-hand picture of Fig.~\ref{fig:embedding} starting at $(0,0)$. 
% Denote $s_0=(0,0)$, $s_n=next(s_{n-1})$ and $S_n=\{s_0, \ldots, s_n\}$. 
% 
Let $a_0\in A$ be an element such that $\fA \models d_{00}(a)\wedge e(a) \wedge \mathit{left}(a)\wedge \mathit{bottom}(a)$ that exists by condition~(1). Denote $a_0=(0,0)$. 
 Suppose $a_{n}=(k,l)$ and $a_{n+1}$ is the witness of $a_{n}$ for the appropriate conjunct from the group~(3), i.e.~where the unary literals in the universal part agree with the unary literals satisfied by $a_{n}$ in $\fA$. 
 
  Let $n\geq 0$. Denote  $A_n=\{a_0,\ldots,a_n\}$ and $\fA_n=\fA \upharpoonright A_n$. 
  
  We show by induction that for every $n\geq 0$: $a_{n+1}\not\in A_n$.  The claim obviously holds for $n=0$. 
  %
  In the inductive step we assume that  
 for every $p\leq n$ and  $a_p=(k,l)\in A_n$ we have: \\
(a) if $p<n$ then $a_{p+1}=next(a_p)$;\\
(b) $\fA_n \models e(k,l)$ iff $k=l$; \\
(c) $\fA_n \models \mathit{left}(k,l)$ iff $k=0$; $\fA_n \models \mathit{bottom}(k,l)$ iff $l=0$;\\
(d) $\fA_n \models d_{ij}(k,l)$ iff $k\geq l$ and $k\mod 3=i$ and $l \mod 6=j$;\\
(e) $\fA_n \models c_{ij}(k,l)$ iff $k<l$ and $k\mod 6=i$ and $l \mod 3=j$;\\
(f) for each $p'\leq n$, for each $t\in \{b,r,g\}$, if $\fG \models t(a_p,a_{p'})$ then $\fA_n \models t(a_p,a_{p'})$. 

Condition (f) implies that each black, green or red path in $\fG\upharpoonright A_n$ is also a path in $\fA_n$ of the same pattern. 
%the transitive paths of each element $a_p\in A_n$ have the same patterns as in $\fG \upharpoonright A_n$ 
%(i.e. $\fA_n$ is similar to $\fG\upharpoonright A_n$).\\

Suppose  that 
   $a_{n}$ is the first element such that $a_{n+1}\in A_n$.
 %Denoting  $\fA_n=\fA \upharpoonright A_n$  
 %has a witness  for the appropriate conjunct from the group~(3) in $\fA_n=\fA \upharpoonright \{a_0,\ldots,a_n\}$. 
 %and $\fG\upharpoonright S_n$ satisfies all universal conjuncts of $\phi_grid$. 
 We show that this implies that some universal conjunct of $\phi_{grid}$ is not true in $\fA_n$. 
 
  In the proof one considers several cases depending on the 1-type realized by $a_n$. 
 The formula $\phi_{grid}$ ensures that $a_0, \ldots, a_{18}$ are all distinct, hence our claim holds for all $n< 18$. 
 %Note also that the conjuncts from the group~(3) ensure that any eight consecutive elements of the sequence $a_0,\ldots, a_n$ are always distinct, as they realize distinct 1-types. 
 
 Consider $a_{18}=(4,2)$ and any witness $w\in A$ such that $\fA\models g(a_{18},w)\wedge d_{11}(w)$. Since $\fA_{18}\models d_{11}(a_2)$, suppose, $w=a_{2}=(1,1)$.  
 Then, by transitivity of $g$, $\fA_{18} \models g((2,1),(1,1))$. But $a_7=(2,1)$ has colour $d_{21}$ and $\fA\models e(a_2)$ by (b); contradiction with \eqref{forbidden8a}. 
Hence, $a_{19}\not \in A_{18}$; denote  $a_{19}=next(4,2)=(4,1)$.  

 Consider $a_{19}$ and any witness $w\in A$ such that $\fA\models b(a_{19},w)\wedge d_{10}$. Since $\fA\models d_{10}(a_3)$, suppose, $w=a_{3}=(1,0)$.  
 Then, by a conjunct from group (4): $\fA\models r(a_{19},w)$. 
By transitivity of $r$, $\fA_{19} \models r((4,2),(2,2))$. But $(4,2)$ has colour $d_{12}$,  $(2,2)$ has colour $d_{22}$ and satisfies $e$; contradiction with \eqref{forbidden8a}. 
 Hence, $a_{20}\not \in A_{19}$. Denote $a_{20}=(4,0)$. 
 
 Consider $a_{20}$ and any witness $w\in A$ such that $\fA\models r(a_{20},w)\wedge d_{20}$. Since $\fA\models d_{10}(a_4)$, suppose, $w=a_{4}=(2,0)$.  
  By transitivity of $r$, $\fA_{20} \models r((4,2),(2,2))$. A contradiction as above. 
 Hence, $a_{21}\not\in A_{20}$. Denote $a_{21}=(5,0)$.  
 
 The same argument applies to the next red witnesses required, and we denote $a_{22}=(6,0)$, $a_{23}=(6,1)$, $a_{24}=(5,1)$ and $a_{25}=(5,2)$. 
 
 Consider $a_{25}$ and any witness $w\in A$ such that $\fA\models b(a_{20},w)\wedge d_{23}$. Since no element $a_k$ ($k<25$) has colour $d_{23}$, $w\not\in A_{25}$ and we denote $a_{26}=(5,3)$. Similarly, we define new elements $a_{27}=(4,3)$, $a_{28}=(4,4)$,  $a_{29}=(3,4)$, $a_{30}=(2,4)$ and $a_{31}=(2,5)$.  

 Consider $a_{31}$ and any witness $w\in A$ such that $\fA\models r(a_{31},w)\wedge c_{12}$. Since $\fA\models c_{12}(a_9)$, suppose, $w=a_{9}=(1,2)$.  
Then, by a conjunct from group (4): $\fA\models b(a_{31},w)$. 
By transitivity of $b$, $\fA \models b((2,5),(2,3))$. 
Then, by a conjunct from group (4): $\fA\models g((2,5),(2,3))$. By transitivity of $g$:  $\fA\models g((4,4),(3,3))$; forbidden by \eqref{forbidden8b}. 
Hence, $a_{32}\not\in A_{31}$ and we define $a_{32}=(1,5)$. 

 Consider $a_{32}$ and any witness $w\in A$ such that $\fA\models g(a_{32},w)\wedge c_{22}$. If $w=(0,2)$ then, by a conjunct from group (4): $\fA\models b(a_{31},w)$. By transitivity of $b$, $\fA \models b((2,5),(2,3))$ and we get a contradiction, as above. Hence, $a_{33}$ is new and $a_{33}=(0,5)$. 
 
 Now, the above argument repeats for the next black witnesses required and we obtain $a_{34}=(0,6)$, $a_{35}=(0,7)$, $a_{36}=(1,7)$, $a_{37}=(1,6)$. 
 
 Consider $a_{38}=(2,6)$. The path of witnesses traverses now through elements with new distinct colours, i.e.~$c_{30}, c_{32}, c_{42}, d_{25}, d_{24}, d_{04}$, hence all corresponding elements are obviously new. 
 
 Consider $a_{45}=(6,4)$ of colour $d_{04}$ and any witness $w$ of $a_{45}$ in $\fA$ for the appropriate conjunct of the form \eqref{tiling:rgb:witnesses}: 
 \begin{align}
 \forall (d_{04} \rightarrow \exists ( r \wedge d_{03})).\tag{*}
 \end{align}
 Since $w$ is required to have colour $d_{03}$, so far we have only one choice: $w=a_{16}=(3,3)$. 
 But $\fA_{45} \models e(3,3)$. 
 % such that $\fA\models r(a_{45},w)\wedge d_{03}$. Since $a_{16}$ has colour $d_{03}$, suppose, $w=a_{16}=\rho(3,3)$. 
  Since $\fA_{45} \models \neg e(a_{45})$ we get a contradiction with \eqref{forbidden8c} for $i=0$, $j=3$: $\forall (d_{04}\rightarrow \forall (d_{03}\wedge e\rightarrow \neg r))$.
% Then, by a conjunct from group (4): $\fA\models b(a_{16},w)$. 
% By transitivity of $r$, $\fA \models r(\rho(4,4),\rho(3,3))$; forbidden by \eqref{forbidden8b}. 
 Hence, $a_{46} \not\in A_{45}$ and we denote $a_{46}=(6,3)$. 
 
 Now, we generalize the case of $a_{45}$.  In the following argument, for any $X\in \fA_n$ by the {\em black (green, red) pattern  of $X$} we call the unique maximal black (green, red) transitive path in $\fA_n$ visiting $X$; the letters A-F are used to denote the shape of these patterns as shown in Figure~\ref{fig:patterns}.
  
 Let $a_n=X$ has colour $d_{04}$ in $\fA$. Suppose there is  a witness $Y\in A_{n}$ of $a_n$ for the above conjunct (*), i.e. 
 %
 $$\fA_n\models d_{04}(X)\wedge r(X,Y)\wedge d_{03}(Y).$$  
 %
 Denote $X=(i,j)$, $Y=(k,l)$. By (d), both $X$ and $Y$ are located on or below the diagonal in $\fA_n$, i.e.~$i\geq j$ and $k\geq l$. (cf.~the pink region on Figure~\ref{fig:grid-three-transitive:Left}). 
 Moreover, $i \mod 3=0$, $j\mod 6 =0$, $k \mod 3=0$ and $l\mod 6 =3$. Hence, $i=k+3s$ and $j=l+1+6s'$, for some integers $s,s'$ not both equal 0. 

  We have three cases. %In each of them we show that $Y$ in $\fG$ leads to a contradiction. 
% Moreover,  applying the conjuncts from the group (4) we get $\fG\models b((i,j),(k,l))$. 
% 
 % Then, by a conjunct from group (4): $\fA\models b(a_{16},w)$. 
% \begin{enumerate}
 
 %	\item[(i)] 
 	
\textbf{(i)} 	 $k=l$. 
 	  By (b), $\fA_n\models e(Y) \wedge \neg e(X)$. Contradiction with \eqref{forbidden8c} (as before for  $a_{45}$).


% \item[(ii)] 
 \textbf{(ii)} 
 $l<k$ and $3s\leq 6s'$;  e.g.~$X=(15,10)$ and $Y=(9,3)$ (cf.~Figure~\ref{fig:tiling-case-iv}).\\
In this case we have $s'>0$; hence  $j>l+6$. 
By induction, $X$ is the pre-last element of its red pattern $A$ starting at $X'=X+[-1,-1]$. 
By transitivity of $r$, $X'$ is connected to $Y$ by a red edge in $\fA_n$. Applying (4) these elements are also connected by a green edge: $\fA\models g(X',Y)$. 

Now, looking at the green patterns we have:  $X'$ is the fourth element on its green pattern $A$, and $Y$---the fifth one, also on pattern $A$. Applying transitivity of $g$, $X''$---the first element of the green pattern of $X'$ is connected to $Y'$---the last element of the green pattern of $Y$, i.e.~$\fA \models g(X'',Y')$, where $X''=X'+[1,-2]$ and $Y'=Y+[1,-2]$. 
Again, applying (4), these elements are connected by a black edge. 

Assume for a moment  $l=3$. Then $Y'=(k+1,1)$, so it is the third element of a black pattern $E$ and %$(i-1+3z+1,j-1-6z-2)$ 
$X''$ is the fourth element of its black pattern $A$. Hence, by transitivity of $b$, $X'''$---the third element of the black  pattern  of $X''$, is connected by $b$ to $Y''$---the fourth elements of the black pattern of $Y'$. Since $Y''=(k+1,0)$ we have $\fA\models \textit{bottom}(Y'')$, and by \eqref{tiling:bot}, $X'''$ also should satisfy $\mathit{bottom}$ but   $X'''=(i,j-4)$ and $j-4 \neq 0$; a contradiction. 

\input{figures-needed-case-(iv)}

%
%If $l>3$ then the black pattern of  $Y'$ has shape $A$ and $Y'$ is the fifth element on it.
% %Applying transitivity of $g$, the first element of the green pattern of $X'$ is connected to the last element of the green pattern of $Y$, i.e.~$\fG \models g(X'+[1,-2],Y+[1,-2])$.
%%Again, applying (4), these elements are connected by a black edge. Now we look at their black patterns: the elements $X'+[1,-2]$ and $Y+[1,-2]$ appear at the same positions in their black patterns $A$, as $X'$ and $Y$ before in their green patterns. 
%%
%Hence, by transitivity of $b$: %$\fG \models g((i-1+2,j-1-4),(k+2,l-4))$. \\
%$\fA \models b((X'+[2,-4],Y+[2,-4])$. 
%Now the conjuncts of the group  (4) imply a red edge between these elements;  and similarly as above, by transitivity of $r$:
%%$\fG \models r((i-1+3,j-1-6),(k+3,l-6))$. \\
%$\fA \models r(X'+[3,-6],Y+[3,-6])$. 
%
%Hence, the red edge between  $X'$ and $Y$ induces a red edge between the elements  shifted by the vector $[3,-6]$. The process repeats until we get a red edge between  elements $X'+z[3,-6]$ and $Y+z[3,-6]$ such that $l-6z=3$. Then we get a contradiction as above when $l$ was equal to 3.  
%
% %(go down to the bottom row)
%%As before, Similarly, $Y$ is the last element of its red pattern $A$. 
%%  Moreover,  applying the conjuncts from the group (4) we get $\fG\models b((i,j),(k,l))$. 
% 
 
 
 %\item[(iii)] 
 
 \textbf{(iii)} $l<k$ and $3s> 6s'$;  e.g.~$X=(15,4)$ and $Y=(9,3)$ (cf.~Figure~\ref{fig:tiling-case-v}).\\
  In this case we have $i>j+2$. By the conjuncts of the group (4) the red edge between $X$ and $Y$ implies also a black edge, i.e.~we have 
  $$\fA_n\models d_{04}(X)\wedge g(X,Y)\wedge d_{03}(Y).$$  

Suppose first, $k=l+3$. Then, $Y$ is the second element on its black pattern $B$ (not intersecting the diagonal). By transitivity of $b$, $X$ is connected by a black edge to $Y'=Y+[1,1]$. % $\fG \models b((i,j),(k+1,l+1))$. 
Applying a conjunct from the group (4), this black edge induces a green one:
$\fA \models g(X,Y')$. Now, $X$ is the fourth element of its green pattern $B$ and  $Y'$---the fourth element of its green pattern $C$ starting on the diagonal. So, transitivity of $g$ implies $X'=X+[-1,2]$ and $Y''=Y'+[-1,2]$ are connected by a green edge. %$\fG \models g((i-1,j+2),(k,l+3))$. 
Since $k=l+3$, $Y''=(l+3,l+3)$, hence  $\fA \models d_{00}(Y'') \wedge e(Y'')$. On the other hand, 
$\fG \models d_{20}(X')$; contradiction by \eqref{forbidden8a}. 
 
 Consider now $k>l+3$. Taking $Y'$ as above we have  $\fA \models g(X,Y')$.  
  We look at the green patterns: $X$ is the fourth element of its green pattern $B$ as before, and
 $Y'$---the fifth one on pattern $B$. Applying transitivity of $g$, $X'=X+[-1,2]$ %---the first element of the green pattern of $X$ 
 is connected  by a green edge to $Y''=Y'+[-1,2]$---the last element of the green pattern of $Y'$. 
 %, i.e.~$\fG \models g(X'+[1,-2],Y+[1,-2])$.
 Again, applying (4), these elements are connected by a red edge. 
 Now, we iterate the process until we get $X''=X+z[-1,2]$ and $Y'''=Y'+z[-1,2]$ such that $k-z=l+2z$. 
 Then we have %$Y'''$ is on the diagonal 
  $\fA\models r(X'',Y''')$, $\fA \models d_{22}(Y''')\wedge e(Y''')$ and $\fA \models d_{12}(X'')$. Applying \eqref{forbidden8a} we get a contradiction. 
 
 \input{figures-needed-case-(v)}
 
 
%  
% (i). $i=j+2$ and $k>l+3<j$; e.g. $X=(12,10)$, $Y=(12,3)$ (cf.~Figure~\ref{fig:tiling-case-i}). \\
%By induction, $X$ is the third element of its green pattern $C$ starting on the diagonal and $Y$ a second element on its black pattern $B$ (not starting on the diagonal). By transitivity of $b$, $X$ is connected by a black edge to $Y'=Y+[1,1]$---the last element of the black pattern of $Y$. 
%Applying the conjunct from the group (4) these elements are also connected by a green edge:  
%$\fG \models g(X,Y')$. 
%Now, by transitivity of $g$, $X'=X+[-1,1]$---the first element of the green pattern of $X$---is connected by a green edge to $Y''=Y'+[-1,2]$---the last element of the green pattern of $Y'$. By inductive hypothesis, since $X'$ is on the diagonal, we have $\fG \models d_{25}(X')\wedge e(X')$. On the other hand, $\fG \models d_{00}(Y'') \wedge \neg e(Y'')$. Taking \eqref{tiling:e} for $i=2$, $j=5$ we have 
%$\fG \models \forall (d_{25}\wedge e \rightarrow \forall (g\wedge d_{00} \rightarrow  e))$; a 
%contradiction. 
%
%\input{figures-needed-case-(i)}
%
%% Then, by transitivity of $b$ we have $\fA\models b(\rho(a_n),\rho(k,l+1)))$ which implies by (4), $\fA \models g((a_n,\rho(k+1,l+1)))$. By transitivity of $g$, we get $\fA\models g(\rho(j+1,j+1),\rho(k-1,l+3))$. By inductive hypothesis,  $\fA \models e(\rho(j+1,j+1))\wedge d_{25}(\rho(j+1,j+1))$ and $\fA \models \neg e(\rho(k-1,l+3))\wedge d_{00}(\rho(k-1,l+3))$. But \eqref{tiling:e} requires $\fA \models e(\rho(k-1,l+3)$, a contradiction.  
%
%(ii). $i=j+2$ and $k=l+3<j $; e.g.~$X=(12,10)$ and $Y=(6,3)$ (cf.~Figure~\ref{fig:tiling-case-ii}).\\ %(go down to the bottom row)
%As before,  $X$ is the third element of its green pattern $C$ starting on the diagonal but at the same time $X$ is the pre-last elements of its red pattern $A$ starting at $X'=X+[-1,-1]$. Similarly, $Y$ is the last element of its red pattern $A$. 
%By transitivity of $r$, $X'$ is connected to $Y$ by a red edge in $\fG$. Applying (4) these elements are also connected by a green edge: $\fG\models g(X',Y)$. 
%Now, looking at their green patterns we have:  $X'$ is the fourth element on its green pattern $A$, and $Y$---the fifth one, also on pattern $A$. Applying transitivity of $g$, the first element of the green pattern of $X'$ is connected to the last element of the green pattern of $Y$, i.e.~$\fG \models g(X'+[1,-2],Y+[1,-2])$.
% Again, applying (4), these elements are connected by a black edge. Now we look at their black patterns: the elements $X'+[1,-2]$ and $Y+[1,-2]$ appear at the same positions in their black patterns $A$, as $X'$ and $Y$ before in their green patterns. Hence, by transitivity of $b$: %$\fG \models g((i-1+2,j-1-4),(k+2,l-4))$. \\
% $\fG \models g((X'+[2,-4],Y+[2,-4])$. 
% Now the conjuncts of the group  (4) imply a red edge between these elements;  and similarly as above, by transitivity of $r$:
%%$\fG \models r((i-1+3,j-1-6),(k+3,l-6))$. \\
%$\fG \models r(X'+[3,-6],Y+[3,-6])$. 
%
%Hence, the red edge between  $X'$ and $Y$ induces a red edge between the pair shifted by the vector $[3,-6]$. The process repeats until we get a red edge between the elements $X'+z[3,-6]$ and $Y+z[3,-6]$ such that $l-6z=3$ (i.e.~we come close to the bottom row). 
%%$(i-1+3z,j-1-6z)$ and $(k+3z,l-6z)$
%Then, applying once more (4), we get that these elements are also connected by a green edge. % $\fG \models  g((i-1+3z,j-1-6z),(k+3z,l-6z))$, 
%Applying transitivity of $g$ and denoting $X''=X'+z[3,-6]+[1,-2]$ and $Y'=Y+z[3,-6]+[1,-2]$ we have:
%%$\fG \models  g((i-1+3z,j-1-6z),(k+3z,l-6z))$
%$\fG \models  g(X'',Y')$. 
%%$\fG \models  g(X'',Y')$. 
%Note that $Y'=(k+3z+1,1)$, so it is the third element of a black pattern $E$ and %$(i-1+3z+1,j-1-6z-2)$ 
%$X''$ is the fourth element of its black pattern $A$. Hence, by transitivity of $b$, $X'''$---the third element of the pattern $A$ of $X''$, is connected by $b$ to $Y''$---the fourth elements of the black pattern $E$ of $Y'$. Since $Y''$ is on the bottom row, by \eqref{tiling:bot}, $X'''$ also should be; but $X'''=X+[0+3z,j-6z]$ and $j-6z>0$; a contradiction. 
%
%\input{figures-needed-case-(ii)}
% 
%(iii). $i>j+2$ and $k=l+3$. 
%
%By induction, $Y$ is the second element on its black pattern $B$ (not intersecting the diagonal). By transitivity of $b$, $X$ is connected by a black edge to $Y'=Y+[1,1]$. % $\fG \models b((i,j),(k+1,l+1))$. 
%Applying a conjunct from the group (4):  
%$\fG \models g(X,Y')$. Now, $X$ is also the fourth element of its green pattern $B$ and  $Y'$---the fourth element of its green pattern $C$ starting on the diagonal. So, transitivity of $g$ implies $X'=X+[-1,2]$ and $Y''=Y'+[-1,2]$ are connected by a green edge. %$\fG \models g((i-1,j+2),(k,l+3))$. 
%Since $k=l+3$, $Y''$ is on the diagonal and $\fG \models d_{00}(Y'') \wedge e(Y'')$. On the other hand, 
%$\fG \models d_{20}(X')$; contradiction by \eqref{forbidden8a} (for $i,j=0$). 
%
%%We start as in the previous subcase, and obtain $\fA \models g(\rho(i,j),\rho(k+1,l+1))$. By transitivity of $g$ we get  that $g(\rho(i-1,j+2),\rho(k+1,l+3))$ holds. This implies, by appropriate conjunct of the group (4), $\fA \models r(\rho(i-1,j+2),\rho(k+1,l+3))$. By transitivity of $r$ we obtain $\fA \models r(\rho(i-2,j+4),\rho(k,l+5))$. Iterating the reasoning steps, we eventually obtain a forbidden connection with an element on the main diagonal. 
%
%\input{figures-needed-case-(iii)}
% 
%(iv). $i>j+2$, $k>l+3<j$ and $3s=6s'$; e.g.~$X=(15,10)$ and $Y=(9,3)$.\\ %(go towards the bottom row)
%By induction, $X$ is the pre-last element of its red pattern $A$. Hence, by transitivity of $r$, $X'$---the first element of the red pattern of $X$---is connected by a red edge to $Y$. Now, we look at the green patterns of $X'$ and $Y$: $X'$ is the fourth element of the green pattern $A$, and $Y$---the fifth one. So, we can continue the argument exactly as in case (ii). 
%
%\input{figures-needed-case-(iv)}
% 
%(v). $i>j+2$, $k>l+2$ and $3s\neq 6s'$; e.g.~$X=(15,4)$ and $Y=(9,3)$.\\ %(go towards the diagonal)
%By induction,   $Y$ is the second element of its black pattern $B$. Hence, $X$ is connected by a black edge to $Y'=Y+[1,1]$---the last element of the black pattern of $Y$.  Applying (4): $\fG\models g(X,Y')$. 
%Now, we look at the green patterns: $X$ is the fourth element of its green pattern $B$ and
%$Y'$---the fifth one, also on pattern $B$. Applying transitivity of $g$, $X'=X+[-1,2]$---the first element of the green pattern of $X$ is connected  by a green edge to $Y''=Y'+[-1,2]$---the last element of the green pattern of $Y'$. 
%%, i.e.~$\fG \models g(X'+[1,-2],Y+[1,-2])$.
%Again, applying (4), these elements are connected by a red edge. 
%Now, we iterate the process towards the diagonal until we get $X''=X+z[-1,2]$ and $Y'''=Y'+z[-1,2]$ such that $Y'''$ is on the diagonal and $\fG\models r(X'',Y''')$. But then $\fG \models d_{22}(Y''')\wedge e(Y''')$ and $fG \models d_{12}(X'')$. Applying \eqref{forbidden8a} for $i,j=2$ we get a contradiction. 
%\input{figures-needed-case-(v)}
%

%\end{enumerate}

\medskip

This way we have shown that for every element $a_n$ of colour $d_{04}$ the witness of $a_n$ is not in $A_n$. In a similar way one can show that the same holds for $a_n$ of any colour $d_{ij}$. Essentially, the point is that we can never go back to a former element of the model that is simultaneously at the same distance to the bottom row and to the diagonal. %So, there would always be a contradiction, either caused by a forbidden connection to the diagonal or to the bottom row.  

For elements of colours $c_{ij}$ the argument is identical but one needs to refer to the corresponding patterns of elements of colours $c_{ij}$, and the contradictions are caused by induced connections  with elements on either the diagonal or the left column. We omit the details here. 
  
%The argument for elements of other colours is similar and we do not include it here. 

\nb{L end of massive changes}

%\end{proof}
 
 \medskip
  
 We are now ready to define the horizontal and vertical successors in models of of $\phi_{grid}$. In fact, instead of defining the horizontal grid successor $\htw$ as one binary relation, we define two disjoint binary relations $\rt(x,y)$ and $\lt(x,y)$ such that $\rt$ and the inverse of $\lt$ together give the expected horizontal grid successor; they are defined respecting the `direction' of the transitive edges in the models. In the intended model  $\rt((x_1,y_1),(x_2,y_2))$ holds if $x_2=x_1+1$, $y_2=y_1$ and $(x_1,y_1)$ and $(x_2,y_2)$ are connected by $b$, $g$ or $r$; and for $\lt((x_1,y_1),(x_2,y_2))$ to hold we require $x_2=x_1-1$ instead of $x_2=x_1+1$. 
	%
We present the definition of $\rt(x,y)$ in detail below.	%
	\begin{align*}
	\rt(x,y) := &  (b(x,y) \vee g(x,y) \vee r(x,y))\quad \wedge  \\
	&	(c_{01}(x) \wedge d_{11}(y)) \vee 	(c_{20}(x) \wedge d_{03}(y)) \vee (c_{42}(x)\wedge d_{25}(y))\quad \vee\\%\label{def:rightDiagonal} \\
	& \mynegsp\mynegsp\mynegsp\mynegsp\mynegsp  \mynegsp\mynegsp\mynegsp\mynegsp 	\bigvee_{(i,j)\notin \{(0,2),(1,2),(2,1),(3,1),(4,0),(5,0)\} } \mynegsp\mynegsp\mynegsp \mynegsp\mynegsp\mynegsp\mynegsp   (c_{ij}(x) \wedge c_{i+1,j}(y) )\quad \vee
	\mynegsp	 \bigvee_{(i,j)\notin \{(2,1),(1,3),(0,5)\}}\mynegsp\mynegsp\mynegsp\mynegsp   (d_{ij}(x) \wedge d_{i+1,j}(y) )
	%
	\end{align*}	
	The relation $\rt$ connects elements that are connected by  $b$, $g$ or $r$ and satisfy one of the possible combinations of colours: in the second line the combinations for crossing the diagonal are listed, in the third line the left disjunction describes combinations when both elements are located above the diagonal, and in the right disjunction---when both elements are located on and below the diagonal. The definition of  $\lt(x,y)$ complements that  of $\rt$.
	%	\begin{align*}
	%	\lt(x,y) := &  (b(x,y) \vee g(x,y) \vee r(x,y))\quad \wedge  \\
	%	&	(d_{00}(x)\wedge c_{50}(y)) \vee 	(d_{14}(x)\wedge c_{31}(y)) \vee (d_{22}(x)\wedge c_{12}(y))\quad \vee\\%\label{def:leftDiagonal} \\
	%& \mynegsp\mynegsp\mynegsp\mynegsp\mynegsp  \mynegsp\mynegsp\mynegsp\mynegsp 	\bigvee_{(i,j)\in \{(1,2),(2,2),(3,1),(4,1),(5,0),(0,0)\} }  \mynegsp\mynegsp\mynegsp \mynegsp\mynegsp\mynegsp\mynegsp   (c_{ij}(x) \wedge c_{i-1,j}(y))\quad \vee
	%\mynegsp	 \bigvee_{(i,j)\in \{(0,1),(2,3),(1,5)\}}\mynegsp\mynegsp\mynegsp\mynegsp  (d_{ij}(x) \wedge d_{i-1,j}(y) )
	%%	&	\bigvee_{(i,j)\in \{(1,2),(2,2),(3,1),(4,1),(5,0),(0,0)\} }  (c_{ij}(x) \wedge c_{i-1,j}(y) ) \vee\\
	%%	&	 \bigvee_{(i,j)\in \{(0,1),(2,3),(1,5)\}}  (d_{ij}(x) \wedge d_{i-1,j}(y) )
	%	%
	%	\end{align*}	
	Analogously, we define relations $\up$ and $\dw$ that together define the vertical grid successor. 
	
	Now we are ready to write formulas that properly assign tiles to elements of the model. We do this with a formula  $\phi_{tile}$,
	which again features several conjuncts enforcing various properties of its models. Fortunately, the properties in question 
	are much simpler this time:
	\begin{enumerate}
		\item[(9)] Each node encodes precisely one tile.\label{tiling:C1}	
		%		\begin{eqnarray}
		%		\forall x (\dot{\bigvee}_{C \in {\cal C}} C x)\label{tiling:C1}
		%		\end{eqnarray}
		\item[(10)] Adjacent tiles respect ${\cal C}_H$.
	%	\begin{align*}
		%	\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\htw(x,y) \rightarrow \bigvee_{C': (C,C') \in {\cal C}_H}  C'y))\tag{7a}\label{tiling:H1f}\\
		%	%	\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\lt(x,y) \rightarrow \bigvee_{C': (C',C) \in {\cal C}_H}  C'y))\label{tiling:H1b}\\
		%	\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\vtw(x,y) \rightarrow \bigvee_{C':(C,C') \in {\cal C}_V} C'y)).\tag{7b}\label{tiling:V1f}
		%	\end{align*}
		\item[(11)] Adjacent tiles respect ${\cal C}_V$.  
	\end{enumerate}
	%
%Property (6) is secured by the conjunct $\forall x \big(\bigvee_{C \in {\cal C}} C  \wedge \bigwedge_{C \neq D} (\neg C   \vee \neg D )\big)$.
%\begin{equation*}
%\forall x \Big(\bigvee_{C \in {\cal C}} C x \wedge \bigwedge_{C \neq D} (\neg C x \vee \neg D x)\Big) ;
%\end{equation*}
Property (10)  is secured by the conjunct	
			\begin{eqnarray*}
				%		\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\rt(x,y) \rightarrow \bigvee_{C': (C,C') \in {\cal C}_H}  C'y))\label{three:H1f}\\
				%
				\bigwedge_{C\in {\cal C}}	\forall x \big(C  \rightarrow \forall y \big((\rt(x,y) \rightarrow \bigvee_{C': (C,C') \in {\cal C}_H}  C' )
			%	\quad \wedge \quad 
			\wedge
				(\lt(x,y) \rightarrow \bigvee_{C': (C',C) \in {\cal C}_H}  C' )\big)\big); \label{three:H1f} 
				%		\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\lt(x,y) \rightarrow \bigvee_{C': (C',C) \in {\cal C}_H}  C'y))\label{three:H1b}
				%		\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\up(x,y) \rightarrow \bigvee_{C':(C,C') \in {\cal C}_V} C'y)).\label{three:V1f}\\
				%		\bigwedge_{C\in {\cal C}}	\forall x (Cx \rightarrow \forall y (\dw(x,y) \rightarrow \bigvee_{C': (C',C) \in {\cal C}_V}  C'y)),\label{three:H1b}%	
			\end{eqnarray*}
and property (11) is analogous, written using $\up$ and $\dw$. We remark that these latter formulas are not strictly fluted but can be rewritten as fluted using classical tautologies (cf.~formula (7) in Section~\ref{sec:twotrans}).
	
Finally, let $\eta_{\boldsymbol{\cal C}}$ be the conjunction of $\phi_{grid}$ and $\phi_{tile}$. The following Claim completes the reduction and the proof of our theorem.
	% figure INTENDED MODEL plus EMBEDDING
	%
%	\begin{claim} 
	
	{\em Claim.}
		$\eta_{\boldsymbol{\cal C}}$ is satisfiable  iff  $\boldsymbol{\cal C}$ tiles  $\N \times \N$.\\
	%	END CLAIM\\
%	\end{claim} 
%	\begin{proof}
		\textit{Proof:} ($\Leftarrow$) If  $\boldsymbol{\cal C}$ tiles  $\N \times \N$ then  to show that $\eta_{\boldsymbol{\cal C}}$ is satisfiable we can expand our intended model $\fG$ for $\phi_{grid}$ assigning to every element of the grid a unique $C\in {\cal C}$ given by the tiling.  
		
		($\Rightarrow$) Let $\fA\models \eta_{\boldsymbol{\cal C}}$. 
		Let $\rho$ be the embedding of the standard $\N\times\N$ grid into $\fA$ defined above. One can inductively show that $\rho$  maps neighbours in the grid to elements connected by one of the relations $\lt, \rt, \up, \dw$ as follows ($i,j\geq 0$):
		\begin{align*}
			\fA\models \rt(\rho(i,j),\rho(i+1,j))\; &\dot{\vee}\; \lt(\rho(i+1,j),\rho(i,j)), \text{ and }\\
			\fA \models  \up(\rho(i,j),\rho(i,j+1))\; &\dot{\vee}\; \dw(\rho(i,j+1),\rho(i,j)).
		\end{align*}
	%	$$\fA\models \rt(\rho(i,j),\rho(i+1,j)) \dot{\vee} \lt(\rho(i+1,j),\rho(i,j)) \wedge \up(\rho(i,j),\rho(i,j+1)) \dot{\vee} \dw(\rho(i,j+1),\rho(i,j)).$$
		(Here, $\dot{\vee}$ is exclusive disjunction.)
		So, we can define a tiling of the standard grid assigning to every node $(i,j)$ the unique tile $C$ such that $\fA \models C(\rho(i,j))$. Conditions (10) and (11) together with the above observation  ensure that this assignment satisfies the %horizontal and vertical 
		tiling conditions.
%	\end{proof} 
%	The above claim ends the proof of the reduction and hence gives undecidability of the satisfiability problem.
	% For finite satisfiability, one can proceed similarly reducing the rectangle tiling problem. To this end we introduce additional unary predicates marking the right and upper border of the intended finite rectangle and  modify the conjuncts of  $\phi_{grid}$ to require witnesses only for elements within such rectangle. Details are routine and have been omitted due to space limits. 
\end{proof}


%Now, considering various conjuncts from the groups (4) and (5), and applying transitivity, we see that in the image of the embedding defined above elements connected by the transitive relations correspond to elements close in the grid. 
%%
%However, since defining $\rho$ we moved through the grid in four directions, 
%we need to respect the four directions as we have fixed order of variables in formulas. 
%%Having shown that every model of $\phi_{grid}$ is grid-like 
%So, instead of defining the horizontal grid successor $\htw$ as one binary relation, we define two binary relations $\rt(x,y)$ and $\lt(x,y)$ such that $\rt$ and the inverse of $\lt$ together give the expected horizontal grid successor;
%Similarly, we define two binary relations $\up(x,y)$ and $\dw(x,y)$ such that $\up$ and the inverse of $\dw$ together give the expected vertical grid successor $\vtw$. 
%and similarly for \eqref{tiling:V1f}; and write an appropriate counterpart of \eqref{tiling:V1f}. 
%The above formulas can be written as fluted thanks to the fact that in the definitions of $\rt(x,y)$, $\lt(x,y)$, $\up(x,y)$ and $\dw(x,y)$ the binary literals have the form $t(x,y)$ (and not $t(y,x)$).  
%%
%%defined by various combinations of the colour and transitive relations between elements located, respectively, right, left, up or down from a given element in the intended expansion of the $\N\times\N$ grid from Figure~\ref{fig:grid-three-transitive}. 
%
We remark that the formula $\phi_{grid}$ in the proof of Theorem~\ref{th:three} is an axiom of infinity, hence we do not get simultaneously undecidability of the finite satisfiability problem. The latter we prove in the following theorem modifying the formula $\phi_{grid}$ to describe (finite) square grids.

\begin{theorem}
	The finite satisfiability problem for $\FLthreetrans$, the two-variable fluted fragment with three transitive relations, is undecidable. 
\label{th:threeFinsat}
\end{theorem} 
\begin{proof}
	%
	We reduce from the rectangle tiling problem. The idea is to modify the formula $\phi_{grid}$ from Theorem \ref{th:three} so that it will be satisfiable in finite structures embedding square grids with domain $\{0,\ldots, t\}\times \{0,\ldots,t\}$, for some $t\geq 1$.  
	More precisely, the modified formula, denoted $\phi_{sgrid}$, will be true in structures that---roughly speaking---are restrictions of the expansions of the $\N\times \N$ grid defined in the proof of Theorem~\ref{th:three} to the domain $\{0,\ldots, t\}\times \{0,\ldots,t\}$ (cf.~Figure \ref{fig:grid-three-transitive:Finsat}).
	The main difference is that the zig-zag path now stops at some point (so that it is satisfiable in finite models) and before it stops it traverses all nodes from the square domain. 
	For the idea to work, we use additional unary predicates $right$ and $top$ to mark, respectively the right column and top row of a square domain, and the modified version of the formula \eqref{tiling:rgb:witnesses} demands and produces witnesses only within the marked (finite) boundary. 
	 More precisely, the zig-zag path starts as before, along the way it produces some element marked as belonging to both the bottom row and the right column. From this element markings of the right column and the counter-diagonal will start (similarly, to the markings of the left column or main diagonal). When the path later meets an element belonging to the left border, marking of the top row starts. The first element produced by the path that belongs to both the top row and the right column is the top right element of the square domain. 
	  
	To give more details of the construction, assume the top right corner of the square is coloured $d_{00}$ (i.e.~the size of the square is $(6k+1)^2$ for some $k$).  %and all elements in the last column (last row) form the right (top) border. 
	This means that there must be some element coloured $d_{00}$ in the bottom-{\em right} corner of the square. Similarly, there is a corresponding corner element located accross the counter diagonal in the left column coloured $c_{00}$ that starts the {\em top} row (we advise to refer to Figure~\ref{fig:embedding-finite}). So, after a top-left element is created new witnesses are created only within the marked boundary until the square is filled. In the particular case depicted on Figure~\ref{fig:embedding-finite}, the top-left element no longer is required to have a witness 'above' of colour $c_{01}$ connected by the black transitive relation, but is required to have a witness of colour $c_{10}$ which corresponds to a right neighbour in the grid. Similarly, the zig-zag path does not continue further to the right from the node $(6,2)$ that is already marked to belong to the right column. Instead, a new witness is created for the node $(6,4)$ going up the right column. Finally, when the process reaches the top right node, the node $(6,6)$ in this case, two more witnesses are created, i.e.~$(5,6)$ and $(4,6)$ in this case, to complete the domain of the square. No more witnesses are required. 
	
	
		\begin{figure}[hbt]
		\begin{subfigure}[t]{0.45\textwidth}	
			\begin{center}
				\begin{minipage}{5.5cm}
					\begin{center}
						%\resizebox{11.2cm}{!}
						{
							
							
							
							\begin{tikzpicture}[scale=0.7]
							
							\clip (-0.8,-0.8) rectangle (7.3,7.3);
							
							\draw [help lines] (0,0) grid (18,18);
							\draw [gray, dotted] (0,0) -- (18,18);
							\draw [gray, dotted] (6,0) -- (0,6);
							
							
							\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							{
								\filldraw[fill=white] (\x, \y) circle (0.1); 
							}
							
							%first edge 		
							\draw[ultra thick, ->, black] (0,0) -- (0,1);
							
							% diagonal		
							%	\foreach \x in {1,7,13} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
							\foreach \x in {1} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
							\foreach \x in {2,8,14} \draw[ultra thick, ->, red] (\x,\x) -- (\x-1,\x);
							\foreach \x in {3,9,15} \draw[ultra thick, <-, green] (\x,\x) -- (\x-1,\x);
							\foreach \x in {4,10,16} \draw[ultra thick, ->, black] (\x,\x) -- (\x-1,\x);
						%	\foreach \x in {5,11,17} \draw[ultra thick, <-, red] (\x,\x) -- (\x-1,\x);
							%	\foreach \x in {6,12,18} \draw[ultra thick, ->, green] (\x,\x) -- (\x-1,\x);
							
							% below the diagonal i.e. x=y+3k, k>0
							
						%	\foreach \y in {5,11,17} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							\foreach \y in {2,8,14} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							
							\foreach \y in {4,10,16} \foreach \x in {\y} %,\y+3,\y+6,\y+9,\y+12,\y+15} 
							\draw[ultra thick, <-, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							%	\foreach \y in {7,13} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							
							\foreach \y in {1} \foreach \x in {\y,\y+3}%,\y+6,\y+9,\y+12,\y+15} 
									\draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1);
							
							\foreach \y in {3,9,15} \foreach \x in {\y} %,\y+3,\y+6,\y+9,\y+12,\y+15} 
							\draw[ultra thick, ->, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							%	\foreach \y in {6,12,18} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
							
							% above the diagonal i.e. x=y+3k, k>0
							
							\foreach \x in {3,9,15} \foreach \y in {\x+1}%,\x+4,\x+7,\x+10,\x+13,\x+16} 
							\draw[ultra thick, ->, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							%					\foreach \x in {6,12,18} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							
						%	\foreach \x in {4,10,16} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							\foreach \x in {7,13} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							\foreach \x in {1} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y);
							
							%	\foreach \x in {5,11,17} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							\foreach \x in {2,8,14} \foreach \y in {\x+1}%,\x+4,\x+7,\x+10,\x+13,\x+16} 
							\draw[ultra thick, <-, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
							
							% left edges	
							\foreach \x in {0} \foreach \y in {2}%,5,8,11,14,17} 
							\draw[ultra thick, ->, black] (\x,\y) -- (\x,\y+2);
						
							\foreach \x in {0} \foreach \y in {5}%,8,11,14,17} 
							\draw[ultra thick, ->, black] (\x,\y) -- (\x,\y+1);
						
							
							%bottom edges
							\foreach \y in {0} \foreach \x in {1,4}%,7,10,13,16} 
							\draw[ultra thick, ->, red] (\x,\y) -- (\x+2,\y);
							
							\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
							\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
							
							\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							{
								\filldraw[fill=white] (\x, \y) circle (0.1); 
							}
							
							
							\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							{
								\filldraw[fill=blue] (\x, -\x+6) circle (0.1); 
							}
							\foreach \x in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
							{
						%		\filldraw[fill=yellow] (\x, \x+1) circle (0.1); 
							}
							
							
							%			
							\end{tikzpicture}
						}
					\end{center}
				\end{minipage}
			\end{center}
			\caption{Marking of the counter-diagonal (blue) after the node $(6,0)$ is marked as the bottom-right corner.
				%Arrows indicate nodes where the zig-zag path crosses the diagonal or where its definition switches from one transitive relation to another.
			}
			\label{fig:embeddingLeft:finite}
		\end{subfigure}
		\hspace{0.05\textwidth}
		\begin{subfigure}[t]{0.45\textwidth}	
			\begin{center}
				\begin{minipage}{5.5cm}
					\begin{center}
						%	\resizebox{11.2cm}{!}
						{
						\begin{tikzpicture}[scale=0.7]
					
					\clip (-0.8,-0.8) rectangle (7.3,7.3);
				
					\draw [very thick, myFuchsia] (-0.3,-0.3) rectangle (6.5,6.5);
					
					\draw [help lines] (0,0) grid (18,18);
					\draw [gray, dotted] (0,0) -- (18,18);
					\draw [gray, dotted] (6,0) -- (0,6);
				
				
					
					\foreach \x in {0,1,2,3,4,5,6}%,7,8,9,10,11,12,13,14,15,16,17}
					\foreach \y in {0,1,2,3,4,5,6}%,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=white] (\x, \y) circle (0.1); 
					}
					
					%first edge 		
					\draw[ultra thick, ->, black] (0,0) -- (0,1);
					
					% diagonal		
					%	\foreach \x in {1,7,13} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
					\foreach \x in {1} \draw[ultra thick, <-, black] (\x,\x) -- (\x-1,\x);
					\foreach \x in {2,8,14} \draw[ultra thick, ->, red] (\x,\x) -- (\x-1,\x);
					\foreach \x in {3,9,15} \draw[ultra thick, <-, green] (\x,\x) -- (\x-1,\x);
					\foreach \x in {4,10,16} \draw[ultra thick, ->, black] (\x,\x) -- (\x-1,\x);
					\foreach \x in {5,11,17} \draw[ultra thick, <-, red] (\x,\x) -- (\x-1,\x);
						\foreach \x in {6}%,12,18} 
						\draw[ultra thick, ->, green] (\x,\x) -- (\x-1,\x);
					
					% below the diagonal i.e. x=y+3k, k>0
					
					\foreach \y in {5,11,17} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					\foreach \y in {2,8,14} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, red] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					
					\foreach \y in {4,10,16} \foreach \x in {\y} %,\y+3,\y+6,\y+9,\y+12,\y+15} 
					\draw[ultra thick, <-, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					%	\foreach \y in {7,13} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					
					\foreach \y in {1} \foreach \x in {\y,\y+3}%,\y+6,\y+9,\y+12,\y+15} 
					\draw[ultra thick, ->, black] (\x,\y) -- (\x,\y-1);
					
					\foreach \y in {3,9,15} \foreach \x in {\y}%,\y+3,\y+6,\y+9,\y+12,\y+15} 
					\draw[ultra thick, ->, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					%	\foreach \y in {6,12,18} \foreach \x in {\y,\y+3,\y+6,\y+9,\y+12,\y+15} \draw[ultra thick, <-, green] (\x,\y) -- (\x,\y-1) -- (\x+1,\y-1) -- (\x+1,\y-2);
					
					 \draw[ultra thick, ->, green] (6,4) -- (6,6);
					 \draw[ultra thick, ->, green] (6,3) -- (6,2);
					 \draw[ultra thick, ->, green] (6,2) -- (7,2);
					 
					 
					
					% above the diagonal i.e. x=y+3k, k>0
					
					\foreach \x in {3,9,15} \foreach \y in {\x+1}%,\x+4,\x+7,\x+10,\x+13,\x+16} 
					\draw[ultra thick, ->, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					%					\foreach \x in {6,12,18} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, red] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					
					\foreach \x in {4,10,16} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, <-, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					\foreach \x in {7,13} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					\foreach \x in {1} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, green] (\x,\y) -- (\x-1,\y);
					
					%	\foreach \x in {5,11,17} \foreach \y in {\x+1,\x+4,\x+7,\x+10,\x+13,\x+16} \draw[ultra thick, ->, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					\foreach \x in {2}%,8,14} 
					\foreach \y in {\x+1}%,\x+4,\x+7,\x+10,\x+13,\x+16} 
					\draw[ultra thick, <-, black] (\x,\y) -- (\x-1,\y) -- (\x-1,\y+1) -- (\x-2,\y+1);
					
					\draw[ultra thick, <-, black] (2,6) -- (0,6);
					\draw[ultra thick, ->, black] (5,6) -- (4,6);
					\draw[ultra thick, ->, black] (4,6) -- (4,7);
					\draw[ultra thick, ->, black] (0,5) -- (0,6);

					
					% left edges	
					\foreach \x in {0} \foreach \y in {2,5,8,11,14,17} \draw[ultra thick, ->, black] (\x,\y) -- (\x,\y+2);
					
					%bottom edges
					\foreach \y in {0} \foreach \x in {1,4}%,7,10,13,16} 
					\draw[ultra thick, ->, red] (\x,\y) -- (\x+2,\y);
					
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} \coordinate [label=center:\x] (A) at (\x, -0.5);
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  \coordinate [label=center:\y] (A) at (-0.5,\y);
					
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=white] (\x, \y) circle (0.1); 
					}
					
					
					\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=blue] (\x, -\x+6) circle (0.1); 
					}
					\foreach \x in {0} %,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
					{
						\filldraw[fill=yellow] (\x, \x+1) circle (0.1); 
					}
					
					
					%crossed out edges
					
					\foreach \x in {0,4}
					\foreach \y in {6.5}
					{
					\draw[ultra thick, -, orange] (\x-0.25,\y-0.25) -- (\x+0.25,\y+0.25);
					\draw[ultra thick, -, orange] (\x-0.25,\y+0.25) -- (\x+0.25,\y-0.25);
					}
					\foreach \x in {6.5}
				\foreach \y in {2}
				{
					\draw[ultra thick, -, orange] (\x-0.25,\y-0.25) -- (\x+0.25,\y+0.25);
					\draw[ultra thick, -, orange] (\x-0.25,\y+0.25) -- (\x+0.25,\y-0.25);
				}
				
				
								%			
					\end{tikzpicture}
					
						
					}	
					\end{center}
				\end{minipage}
			\end{center}
			\caption{After the top-left corner $(0,6)$ is met the path continues within the indicated squared region.}
			\label{fig:embeddingRight:finite}
		\end{subfigure}
		\caption{Construction of the intended model of $\phi_{sgrid}$ % with universe $\N\times \N$ 
			in the proof of Theorem~\ref{th:threeFinsat}.}
		\label{fig:embedding-finite}
	\end{figure}
	
	
It is not difficult to write conjuncts enforcing the above property, similar to conjunct of the group~\eqref{tiling:rgb:witnesses} in the proof of Theorem~\ref{th:three}. Some examples of such  conjuncts are given below:\nb{L I don't think we need a full Table again (?)}
\begin{align*}
%
\forall  (d_{02} \wedge \mathit{right}  &\rightarrow \exists  (g \wedge \bot)),\\%\tag{4a}\label{tiling:4a}\\
\forall  (d_{04}  \wedge \mathit{right}  &\rightarrow \exists  (g \wedge d_{05})),\\%\tag{4a}
\forall  (c_{00} \wedge \mathit{left}\wedge \mathit{top}  &\rightarrow \exists (b \wedge c_{10})).%\tag{4c}\label{tiling:4c}
% \wedge \nonumber\\
%	\forall x (c_{21}  &\rightarrow \forall y (r \wedge (c_{22} \vee d_{22} )\rightarrow g )), \tag{4d}\label{tiling:4d}
%	\forall x (d_{22}  &\rightarrow \forall y (r \wedge d_{12} \rightarrow b )).\tag{4e}\label{tiling:4e}
%
\end{align*}


Hence, we can argue as before that $\phi_{sgrid}$ is satisfiable and in particular every square grid can be expanded into a model of $\phi_{sgrid}$. 

The rest of the encoding of tilings is almost identical to that in Theorem~\ref{th:three} with the only difference that now we additionally require that the two distinguished tiles are located in the appropriate positions:
	\begin{enumerate}
	\item[(12)] the distinguished tiles are located in the bottom-left and the top-right elements, respectively.\label{tiling:C:origin}	
			\begin{eqnarray}
			\forall  (\mathit{left} \wedge bottom \rightarrow C_0)\; \wedge\; \forall  (top \wedge right\rightarrow C'_0).\nonumber
			\end{eqnarray}
\end{enumerate}
So we have completed the reduction from the (undecidable) rectangle tiling problem to the finite satisfiability problem for $\FLthreetrans$. 
\end{proof}


We complete this section noticing that all formulas used in the proofs of Theorems \ref{th:three} and \ref{th:threeFinsat} are either guarded or can easily be rewritten as guarded. Furthermore, in the proof it would suffice to assume that $b$, $g$ and $r$ are interpreted as equivalence relations. Hence, we can strengthen the above theorem as follows.
\begin{corollary}
	The  (finite) satisfiability problem for the intersection of the fluted fragment with the two-variable guarded fragment is undecidable in the presence of three transitive relations \textup{(}or three equivalence relations\textup{)}. \label{cor:three}
\end{corollary}

%\input{figures-needed}


%\section{Trash}

%%% figure combined with Figure with 3 transitive relations. 
%\begin{figure}[thb]
%	\begin{center}
%		\begin{minipage}{13cm}
%			\begin{minipage}{12.5cm}
%				\begin{center}
%					\begin{tikzpicture}[xscale=0.9,yscale=0.9]
%					%
%					% 					\def{\z}{0.1}
%					\clip (-0.15,-0.15) rectangle (7.3,4.3);
%					\foreach \x in {-1,1,3,5,7}
%					\foreach \y in {-1,1,3,5,7} \foreach \z in {0.1} 
%					{
%						\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
%						(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
%						\draw[color=red,thick,-, >=latex] (\x+\z, \y+\z) --
%						(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
%						
%					}	
%					
%					\foreach \x in {0,2,4,6}
%					\foreach \y in {0,2,4,6} \foreach \z in {0.1} 
%					{
%						\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) -- (\x+1-\z, \y+\z) --
%						(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+\z, \y+\z);
%						\draw[color=blue,thick,-, >=latex] (\x+\z, \y+\z) --
%						(\x+1-\z, \y+1-\z) -- (\x+\z, \y+1-\z) -- (\x+1-\z, \y+\z);
%					}	
%					
%					\foreach \x in {1,5}
%					\foreach \y in {1,5} \foreach \z in {0.15} 
%					{
%						\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
%						\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
%						\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
%						\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
%					}	
%					
%					\foreach \x in {3,7}
%					\foreach \y in {3,7} \foreach \z in {0.15} 
%					{
%						\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x+1-\z, \y);
%						\draw[color=blue,thick,->, >=latex] (\x, \y) -- (\x, \y+1-\z);
%						\draw[color=blue,thick,->, >=latex] (\x-1, \y) -- (\x-1, \y+1-\z);
%						\draw[color=blue,thick,->, >=latex] (\x, \y-1) -- (\x+1-\z, \y-1);						
%					}	
%					
%					
%					\foreach \x in {1,5}
%					\foreach \y in {3,7} \foreach \z in {0.15} 
%					{
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x, \y) ;
%						\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y);
%						\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y);
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x, \y-1);						
%					}	
%					
%					\foreach \x in {3,7}
%					\foreach \y in {1,5} \foreach \z in {0.15} 
%					{
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
%						\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
%						\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
%					}	
%					
%					\foreach \x in {1,5}
%					\foreach \y in {3,7} \foreach \z in {0.15} 
%					{
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y) -- (\x+\z, \y) ;
%						\draw[color=blue,thick,->, >=latex] (\x, \y+1-\z) -- (\x, \y+\z);
%						\draw[color=blue,thick,->, >=latex] (\x-1, \y+1-\z) -- (\x-1, \y+\z);
%						\draw[color=blue,thick,->, >=latex] (\x+1-\z, \y-1) -- (\x+\z, \y-1);						
%					}	
%					
%					
%					
%					% 						\draw[color=red,thick,->, >=latex] (\x-0.05, \y+0.1) -- (\x-0.05, \y+0.8);
%					% 						
%					% 						%	\draw[color=blue,thick,->, >=latex] (\x+0.1, \y) -- ($(\x,\y) + (0.9,0)$); 
%					% 						\draw[color=black,thick,->, >=latex] (\x+0.1, \y-0.05) -- ($(\x,\y) + (0.8,0-0.05)$); 
%					% 						\draw[color=blue,thick,->, >=latex] (\x+0.1, \y+0.05) -- ($(\x,\y) + (0.8,0+0.05)$); 
%					% 						
%					% 						%		\draw[color=blue,thick,->, >=latex] (\x+1.9, \y) -- ($(\x,\y) + (1.1,0)$); 
%					% 						\draw[color=green,thick,->, >=latex] ($(\x,\y) + (1.1,-0.05)$) -- (\x+1.8, \y-0.05); 
%					% 						\draw[color=red,thick,->, >=latex] ($(\x,\y) + (1.1,+0.05)$) -- (\x+1.8, \y+0.05); 
%					% 						
%					% 						%\draw[color=blue,thick,->, >=latex] (\x+1, \y+0.1) -- (\x+1, \y+0.9);
%					% 						\draw[color=blue,thick,->, >=latex] (\x+0.95, \y+0.1) -- (\x+0.95, \y+0.8);
%					% 						\draw[color=red,thick,dashed,->, >=latex] (\x+1.05, \y+0.1) -- (\x+1.05, \y+0.8);
%					% 						
%					%					}
%					
%					
%					% 					\foreach \x in {1,3,5}
%					% 					\foreach \y in {3,5}{
%					% 						\draw[color=green,thick,dashed,->, >=latex]  (\x-0.05, \y+0.1) -- (\x-0.05, \y+0.8);
%					% 						\draw[color=black,thick,->, >=latex]  (\x+0.05, \y+0.1) -- (\x+0.05, \y+0.8);
%					% 						
%					% 						\draw[color=blue,thick,->, >=latex] ($(\x,\y) + (0.9,-0.05)$) -- (\x+0.2, \y-0.05) ; 
%					% 						\draw[color=black,thick,->, >=latex] ($(\x,\y) + (0.9,0.05)$) -- (\x+0.2, \y+0.05) ; 
%					% 						
%					% 						\draw[color=red,thick,->, >=latex] ($(\x,\y) + (1.8,-0.05)$) -- (\x+1.2, \y-0.05) ; 
%					% 						\draw[color=green,thick,->, >=latex] ($(\x,\y) + (1.8,0.05)$) -- (\x+1.2, \y+0.05) ; 
%					% 						
%					% 						\draw[color=black,thick,dashed,->, >=latex]  (\x+0.95, \y+0.1) -- (\x+0.95, \y+0.8);
%					% 						\draw[color=green,thick,->, >=latex]  (\x+1.05, \y+0.1) -- (\x+1.05, \y+0.8);
%					% 						
%					% 					}
%					
%					
%					% 					\foreach \x in {1,2,3,4,5,6}
%					% 					\foreach \y in {2}
%					% 					{
%					% 					\filldraw[fill=white] (\x, \y) circle (0.2); 
%					% 					\pgfmathtruncatemacro{\abc}{mod(\y-1,2)} 
%					% 					\pgfmathtruncatemacro{\bcd}{mod(\x-1,2)} 
%					% 					\coordinate [label=center:$b_{\bcd \abc}$] (A) at (\x,\y);
%					% 				}
%					
%					\foreach \x in {0,1,2,3,4,5,6,7}
%					\foreach \y in {0,1,2,3,4,5,6,7}
%					{
%						\filldraw[fill=white] (\x, \y) circle (0.2); 
%						\pgfmathtruncatemacro{\abc}{mod(\y,4)} 
%						\pgfmathtruncatemacro{\bcd}{mod(\x,4)} 
%						\coordinate [label=center:$_{\bcd\abc}$] (A) at (\x,\y);
%					}
%					
%					
%					%	\foreach \x in {1,2,3,4,5,6} \pgfmathtruncatemacro{\abc}{\x-1} \coordinate [label=center:$_{\abc}$] (A) at (\x, 1.5);
%					%	\foreach \y in {1,2,3,4,5} \pgfmathtruncatemacro{\abc}{\y-1} \coordinate [label=center:$_{\abc}$] (A) at (0.5,\y+1);
%					
%					\draw[ ->, dotted, very thick] (7.5,0) -- (8,0);
%					\draw[ ->, dotted, very thick] (0,7.5) -- (0,8);
%					\draw[ ->, dotted, very thick] (7.5,7.5) -- (8,8);
%					
%					% 					\coordinate [label=center:$b$] (A) at (1.5,1.8);
%					% 					\coordinate [label=center:$\color{cyan}c$] (A) at (1.5,2.2);
%					% 					\coordinate [label=center:$\color{green}g$] (A) at (2.5,1.8);
%					% 					\coordinate [label=center:$\color{red}r$] (A) at (2.5,2.2);
%					% 					
%					\end{tikzpicture}\end{center}
%			\end{minipage}
%			
%		\end{minipage}		
%	\end{center}
%	
%	\caption{Intended expansion of the $\N\times\N$ grid with transitive relations {\color{blue}$b$}   and  {\color{red}$r$}. Edges without arrows depict connections in both direction. Nodes are marked by the indices of  the $c_{ij}$s they satisfy.  % (left picture)
%		% and with three transitive relations $r_1, r_2, r_3$ (right picture).}\label{fig:und-equivalences}
%		\label{fig:grid-two-transitive}}
%\end{figure}





==> rectangular-paths.tex <==
%PATH PATTERNS for cases (i)---(v)	
%	

\begin{figure}[hbt]
	\begin{center}
		
		\resizebox{12.2cm}{!}{
			\begin{tikzpicture}%[scale=0.3]
			
			\clip (-0.8,-0.8) rectangle (13.3,11.3);
	
	%%%% COLOURED REGIONS.
	\path [fill=myYellow] (-0.1,0.1) to (14.0,14.1) to (-0.1,14.1) to (-0.1,0.1);
%	\path [fill=myMelon] (0,0.5) to  (8.5,9.0) to (9.0,9.0) to (9.0,0) to (0,0) to (0,0.5);
	
			
	% ZIG-ZAG PATH
		
	\draw[->,ultra thick, myGray, line width=5mm, rounded corners]%, scale=0.2] 
	(0,0) -- (0,1) 
	-- (1,1) 
	-- (1,0) 
	-- (2,0) 
	-- (2,2)
	-- (0,2) 
	-- (0,3) 
	-- (3,3) 
	-- (3,0)
	-- (4,0) 
	-- (4,4) 
	-- (0,4)
	-- (0,5) 
	-- (5,5) 
	-- (5,0)
	-- (6,0) 
	-- (6,6) 
	-- (0,6)
	-- (0,7) 
	-- (7,7) 
	-- (7,0)
	-- (8,0) 
	-- (8,8) 
	-- (0,8)
	-- (0,9) 
	-- (9,9) 
	-- (9,0)
	-- (10,0)	;	
	
	% end of ZIG-ZAG. 
	
	
	\draw [help lines] (0,0) grid (18,18);
	%\draw [black, dotted] (0,0) -- (18,18);
	\draw [orange, dotted] (0,0) -- (18,18);
	
			\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} 
	\coordinate [label=center:\x] (A) at (\x, -0.5);
	\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}  
	\coordinate [label=center:\y] (A) at (-0.5,\y);
	
		\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
	\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17}
	{
		\filldraw[fill=white] (\x, \y) circle (0.1); 
	}
	
	
	% pattern D appears around the diagonal
\foreach \x in {1,7,13} \foreach \y in {\x}%,\x+3,\x+6,\x+9,\x+12,\x+15} 
\foreach \s in {0.1}
{	\filldraw[fill=black] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s)  -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}


	% pattern D appears around the diagonal
\foreach \x in {3,9,15} \foreach \y in {\x}%,\x+3,\x+6,\x+9,\x+12,\x+15} 
\foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s)  -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}


	% pattern D appears around the diagonal
\foreach \x in {5,11} \foreach \y in {\x}%,\x+3,\x+6,\x+9,\x+12,\x+15} 
\foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-1+\s) -- (\x+1-\s,\y-1+\s)  -- (\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}



	% pattern B appears around the bottom row
\foreach \y in {2,8,14} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=black] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s)  -- (\x+1-\s,\y-\s);
	\draw [->, dashed, ultra thick, black] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
}

	% pattern E short around the bottom row
\foreach \y in {0} \foreach  \x in {\y,\y+2,\y+4,\y+6,\y+8,\y+10,\y+12,\y+14,\y+16}  \foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y+\s) -- (\x+\s,\y+1-\s) -- (\x+1-\s,\y+1-\s)  -- (\x+1-\s,\y+\s);
	\draw [->, dashed, ultra thick, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
}



	% pattern U appears around the bottom row
\foreach \y in {4,10,16} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s)  -- (\x+1-\s,\y-\s);
	\draw [->, dashed, ultra thick, green] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
}

	% pattern U appears around the bottom row
\foreach \y in {6,12,18} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y) -- (\x+\s,\y-2+\s) -- (\x+1-\s,\y-2+\s)  -- (\x+1-\s,\y-\s);
	\draw [->, dashed, ultra thick, red] (\x+\s,\y-\s) -- (\x+1-\s-\s,\y-\s);
}



	% pattern U reversed appears around the bottom row
\foreach \y in {1,7,13} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]   (\x+\s,\y) -- (\x+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, red]	(\x+\s,\y+1-\s) --	(\x+\s,\y+2-\s);
	\draw [->, rounded corners, ultra thick, red]	(\x+\s,\y+2-\s) -- (\x+1-\s,\y+2-\s); 
	\draw [->, rounded corners, ultra thick, red]	(\x+1-\s,\y+2-\s) -- (\x+1-\s,\y+1+\s);
	\draw [->, rounded corners, ultra thick, red]	(\x+1-\s,\y+1+\s) -- (\x+1-\s,\y+\s);
	\draw [->, dashed, ultra thick, red] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
}


	% pattern U reversed appears around the bottom row
\foreach \y in {3,9,15} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=black] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, black]   (\x+\s,\y) -- (\x+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, black]	(\x+\s,\y+1-\s) --	(\x+\s,\y+2-\s);
	\draw [->, rounded corners, ultra thick, black]	(\x+\s,\y+2-\s) -- (\x+1-\s,\y+2-\s); 
	\draw [->, rounded corners, ultra thick, black]	(\x+1-\s,\y+2-\s) -- (\x+1-\s,\y+1+\s);
	\draw [->, rounded corners, ultra thick, black]	(\x+1-\s,\y+1+\s) -- (\x+1-\s,\y+\s);
	\draw [->, dashed, ultra thick, black] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
}


	% pattern U reversed appears around the bottom row
\foreach \y in {5,11,17} \foreach  \x in {\y+1,\y+3,\y+5,\y+7,\y+9,\y+11,\y+13,\y+15,\y+17}  \foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]   (\x+\s,\y) -- (\x+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, green]	(\x+\s,\y+1-\s) --	(\x+\s,\y+2-\s);
	\draw [->, rounded corners, ultra thick, green]	(\x+\s,\y+2-\s) -- (\x+1-\s,\y+2-\s); 
	\draw [->, rounded corners, ultra thick, green]	(\x+1-\s,\y+2-\s) -- (\x+1-\s,\y+1+\s);
	\draw [->, rounded corners, ultra thick, green]	(\x+1-\s,\y+1+\s) -- (\x+1-\s,\y+\s);
	\draw [->, dashed, ultra thick, green] (\x+\s,\y+\s) -- (\x+1-\s-\s,\y+\s);
}




	% pattern C appears around the left column
\foreach \x in {2,8,14} \foreach \y in {\x,\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]  (\x-\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s)  -- (\x-\s,\y+1-\s);
	\draw [->, dashed, ultra thick, green] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
}

	% pattern C appears around the left column
\foreach \x in {4,10,16} \foreach \y in {\x,\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]  (\x-\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s)  -- (\x-\s,\y+1-\s);
	\draw [->, dashed, ultra thick, red] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
}

	% pattern C appears around the left column
\foreach \x in {6,12,18} \foreach \y in {\x,\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=black] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, black]  (\x-\s,\y+\s) -- (\x-2+\s,\y+\s) -- (\x-2+\s,\y+1-\s)  -- (\x-\s,\y+1-\s);
	\draw [->, dashed, ultra thick, black] (\x-\s,\y+\s) -- (\x-\s,\y+1-\s-\s);
}


	% pattern C reversed appears around the left column
\foreach \x in {1,7,13} \foreach \y in {\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=black] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, black]  (\x+\s,\y+\s) -- (\x+1,\y+\s); 
	\draw [->, rounded corners, ultra thick, black]  (\x+1-\s,\y+\s) -- (\x+2-\s,\y+\s);
	\draw [->, rounded corners, ultra thick, black]  (\x+2-\s,\y+\s) -- (\x+2-\s,\y+1-\s); 
	\draw [->, rounded corners, ultra thick, black] (\x+2-\s,\y+1-\s) -- (\x+1+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, black] 	(\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, black] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}


	% pattern C reversed appears around the left column
\foreach \x in {3,9,15} \foreach \y in {\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=green] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, green]  (\x+\s,\y+\s) -- (\x+1,\y+\s); 
	\draw [->, rounded corners, ultra thick, green]  (\x+1-\s,\y+\s) -- (\x+2-\s,\y+\s);
	\draw [->, rounded corners, ultra thick, green]  (\x+2-\s,\y+\s) -- (\x+2-\s,\y+1-\s); 
	\draw [->, rounded corners, ultra thick, green] (\x+2-\s,\y+1-\s) -- (\x+1+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, green] 	(\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, green] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}

	% pattern C reversed appears around the left column
\foreach \x in {5,11,17} \foreach \y in {\x+2,\x+4,\x+6,\x+8,\x+10,\x+12,\x+14,\x+16} \foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y+\s) -- (\x+1,\y+\s); 
	\draw [->, rounded corners, ultra thick, red]  (\x+1-\s,\y+\s) -- (\x+2-\s,\y+\s);
	\draw [->, rounded corners, ultra thick, red]  (\x+2-\s,\y+\s) -- (\x+2-\s,\y+1-\s); 
	\draw [->, rounded corners, ultra thick, red] (\x+2-\s,\y+1-\s) -- (\x+1+\s,\y+1-\s);
	\draw [->, rounded corners, ultra thick, red] 	(\x+1-\s,\y+1-\s) -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, red] (\x+\s,\y+\s) -- (\x+\s,\y+1-\s-\s);
}






	% pattern F short around the left column
\foreach \x in {0} \foreach  \y in {\x+1,\x+3,\x+5,\x+7,\x+9,\x+11,\x+13,\x+15,\x+17}  \foreach \s in {0.1}
{	\filldraw[fill=red] (\x, \y) circle (0.1);
	\draw [->, rounded corners, ultra thick, red]  (\x+\s,\y+\s) -- (\x+1-\s,\y+\s) -- (\x+1-\s,\y+1-\s)  -- (\x+\s,\y+1-\s);
	\draw [->, dashed, ultra thick, red] (\x,\y+\s) -- (\x,\y+1-\s);
}



		
			
		\end{tikzpicture}
		}
		\vspace{0cm}		
	\end{center}
	
	\caption{Intended expansion of the  $\N \times \N$ grid and the boustrophedon order (thick gray path).}
	%\label{fig:zig-zag-with-yellow}
	\label{fig:zig-zag}
\end{figure}


==> safety.tex <==
\section{Introduction}
\label{sec:intro}
The \textit{fluted fragment}, here denoted $\FL$, is a fragment of first-order logic in which, roughly speaking, the order of quantification of variables coincides with the order in which those variables appear as arguments of predicates. The allusion is presumably architectural: we are invited to think of arguments of predicates as being `lined up' in columns. The following formulas are sentences of $\FL$
\begin{align}
& \mbox{
	\begin{minipage}{10cm}
	\begin{tabbing}
	No student admires every professor\\
	$\forall x_1 (\mbox{student}(x_1) \rightarrow \neg \forall x_2 (\mbox{prof}(x_2) \rightarrow \mbox{admires}(x_1, x_2)))$
	\end{tabbing}
	\end{minipage}
}
\label{eq:eg1}\\
& \mbox{
	\begin{minipage}{8.5cm}
	\begin{tabbing}
	No lecturer introduces any professor to every student\\
	$\forall x_1 ($\=$\mbox{lecturer}(x_1) \rightarrow$
	$\neg \exists x_2 ($\=$\mbox{prof}(x_2)
	\wedge \forall x_3 (\mbox{student}(x_3) \rightarrow \mbox{intro}(x_1,x_2,x_3))))$,
	\end{tabbing}
	\end{minipage}
}
\label{eq:eg2}
\end{align}
with the `lining up' of variables illustrated in Fig.~\ref{fig:lining}. By contrast, none of the formulas
%$$ \forall x_1 . r(x_1, x_1) \;
% \forall x_1 \forall x_2 (r(x_1, x_2) \rightarrow r(x_2,x_1))\;
% \forall x_1 \forall x_2 \forall x_3 (r(x_1,x_2) \wedge r(x_2,x_3) \rightarrow r(x_1,x_3)),
%$$
%
\begin{align*}
& \forall x_1 . r(x_1, x_1)\\
& \forall x_1 \forall x_2 (r(x_1, x_2) \rightarrow r(x_2,x_1))\\
& \forall x_1 \forall x_2 \forall x_3 (r(x_1,x_2) \wedge r(x_2,x_3) \rightarrow r(x_1,x_3)),
\end{align*}
expressing, respectively, the reflexivity, symmetry and transitivity of the relation $r$, is fluted, as the atoms involved cannot be arranged so that their argument sequences `line up' in the fashion of Fig.~\ref{fig:lining}. 
%The same applies to its equivalent variant
%$\forall x_1 \forall x_2 (r(x_1,x_2) \rightarrow \forall x_3 (r(x_2,x_3) \rightarrow r(x_1,x_3))$.
\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.5]
\draw[dotted] (3.35,7.5) -- (3.25,2.5);
\draw[dotted] (4.25,7.5) -- (4.25,2.5);
\draw (3.325,7) node {$\forall x_1$};
\draw (2.2,6) node {$(\mbox{student}(x_1)$};
\draw (3.6,5) node {$\rightarrow \neg \forall x_2$};
\draw (3.7,4) node {$(\mbox{prof}(x_2)$};
\draw (2.5,3) node {$ \rightarrow \mbox{admires}(x_1, x_2)))$};
\end{tikzpicture}
\hspace{2.5cm}
\begin{tikzpicture}[scale=0.5]
\draw[dotted] (3.35,7.5) -- (3.25,0.5);
\draw[dotted] (4.25,7.5) -- (4.25,0.5);
\draw[dotted] (5.25,7.5) -- (5.25,0.5);
\draw (3.3,7) node {$\forall x_1$};
\draw (2.2,6) node {$(\mbox{lecturer}(x_1)$};
\draw (3.5,5) node {$ \rightarrow \neg \exists x_2$};
\draw (3.7,4) node {$(\mbox{prof}(x_2)$};
\draw (4.9,3) node {$ \wedge \forall x_3$};
\draw (4.2,2) node {$(\mbox{student}(x_3)$};
\draw (3.6,1) node {$\rightarrow \mbox{intro}(x_1,x_2,x_3))))$};
\end{tikzpicture}
\end{center}
\caption{The `lining up' of variables in the fluted formulas~\eqref{eq:eg1} and~\eqref{eq:eg2}; all quantification is executed on the right-most available column.}
\label{fig:lining}
\end{figure}
%

The history of this fragment is somewhat tortuous.
The basic idea of {\em fluted logic} can be traced to a paper given by W.V.~Quine to the 1968 {\em International Congress of Philosophy}~\cite{purdyTrans:quine69}, in which the author defined the {\em homogeneous $m$-adic formulas}. Quine later relaxed this fragment, in the context of a discussion of predicate-functor logic, to what he called `fluted' quantificational schemata~\cite{purdyTrans:quine76b}, 
claiming that the satisfiability problem for the relaxed fragment is decidable.
The viability of the proof strategy sketched by Quine was explicitly called into question by Noah \cite{purdyTrans:noah80}, and the subject then taken up by 
W.C.~Purdy~\cite{purdyTrans:purdy96a}, who gave his own definition of `fluted formulas', proving decidability.
It is questionable whether Purdy's reconstruction is faithful to Quine's intentions: the matter is clouded by differences in the definitions of predicate functors between between~\cite{purdyTrans:noah80}
and~\cite{purdyTrans:quine76b}, both of which Purdy cites. In fact, Quine's original definition of 
`fluted' quantificational schemata appears to coincide with a logic introduced---apparently independently---by A.~Herzig~\cite{purdyTrans:herzig90}.
Rightly or wrongly, however, the name `fluted fragment' 
has now attached itself to Purdy's definition in~\cite{purdyTrans:purdy96a}; and we shall continue to use it in that way in the present article. See Sec.~\ref{sec:prelim} for a formal definition. 

To complicate matters further, Purdy claimed in~\cite{purdyTrans:purdy02} that  
$\FL$ (i.e.~the fluted fragment, in our sense, and his) has the exponential-sized model property: if a fluted formula $\phi$ is satisfiable, then it is satisfiable over a domain of size bounded by an exponential function of the number of symbols in $\phi$. Purdy concluded that the satisfiability problem for $\FL$ is \NExpTime-complete. These latter claims are false. It was shown in~\cite{purdyTrans:P-HST16} that, although
$\FL$ has the finite model property, there
is no elementary bound on the sizes of the models required, and the satisfiability problem for $\FL$ is non-elementary.
More precisely, define $\FL^m$ to be the subfragment of
$\FL$ in which at most $m$ variables (free or bound) appear. Then the satisfiability problem 
for $\FL^m$ is $\lfloor m/2 \rfloor$-\NExpTime-hard for all $m \geq 2$ and in
$(m-2)$-\NExpTime{} for all $m \geq 3$~\cite{P-HST-FLrev}.
It follows that the satisfiability problem 
for $\FL$ is \Tower-complete, in the framework of~\cite{purdyTrans:schmitz16}.
These results fix  the exact complexity 
of satisfiability of $\FL^m$ for small values of $m$.
Indeed, the satisfiability problem for $\FOt$, 
the two-variable fragment of first-order logic, is known to be \NExpTime-complete~\cite{purdyTrans:gkv97}, whence the corresponding problem for 
$\FL^2$ is certainly in \NExpTime. Moreover, 
for $0 \leq m \leq 1$, $\FL^m$ coincides with the $m$-variable fragment of first-order logic,
whence its satisfiability problem is \NPTime-complete. Thus,
taking $0$-\NExpTime{} to mean \NPTime, we see that the satisfiability problem 
for $\FL^m$ is $\lfloor m/2 \rfloor$-\NExpTime-complete, at least for $m\leq 4$.

The focus of the present paper is what happens when we add to the fluted fragment the 
ability to stipulate that certain designated binary relations are \textit{transitive}, or are
{\em equivalence relations}. The motivation comes from analogous results obtained for other
decidable fragments of first-order logic.  Consider basic propositional modal logic K.
Under the standard translation into first-order logic (yielded by Kripke semantics), we can regard K
as a fragment of first-order logic---indeed as a fragment of $\FLt$.
From basic modal logic K, we obtain the logic K4 under the supposition that the accessibility relation
on possible worlds is transitive, and the logic S5 under the supposition that it is an equivalence relation: it is well-known that the satisfiability problems for K and K4 are \PSpace-complete, whereas that for
S5 is \NPTime-complete~\cite{purdyTrans:ladner77}. (For analogous results on {\em graded} modal logic, see~\cite{purdyTrans:kph09}.)
Closely related are also description logics (cf.~\cite{purdyTrans:2003handbook}) with {\em role hierarchies} and {\em transitive roles}. In particular, the description logic  $\mathcal{SH}$, which has the finite model property, is an $\ExpTime$-complete fragment of $\FL$ with transitivity. 
Similar investigations have been carried out in respect of \FOt{}, which has the finite model property and
whose satisfiability problem, as just mentioned, is \NExpTime-complete. The finite model property is lost when one transitive relation or two equivalence relations are allowed. 
%
For equivalence, everything is known: the (finite) satisfiability problem for \FOt{} in the presence of a single equivalence relation 
remains \NExpTime-complete, but this increases to \TwoNExpTime-complete in the presence of two equivalence relations~\cite{purdyTrans:kmp-ht,purdyTrans:KO12}, and becomes undecidable with three. For transitivity, we
have an incomplete picture:
the {\em finite} satisfiability problem for $\FOt$ in the presence with a single transitive relation in decidable in \ThreeNExpTime~\cite{purdyTrans:ph18}, while the decidability of the satisfiability problem remains open (cf.~\cite{ST-FO2T}); the corresponding problems with two transitive relations %(even one transitive relation and one equivalence relation) 
are both undecidable~\cite{purdyTrans:KT09}. 

Adding equivalence relations to the fluted fragment poses no new problems. Existing results on
of $\FOt$ with two equivalence relations can be used to show that the satisfiability and finite
satisfiability problems for $\FL$ (not just $\FLt$) with \textit{two} equivalence relations are decidable. Furthermore,
the proof that the corresponding problems for
$\FOt$ in the presence of \textit{three} equivalence relations are undecidable can easily be seen to apply also to $\FLt$. 
On the other hand, the situation with transitivity is much less clear. In particular, it is known that adding {\em inverses}  to the description logic $\mathcal{SH}$ (feature not expressible in $\FL$) does not spoil the finite model property \cite{DucL10}.\nb{L new reference}  

Some indication that flutedness interacts in interesting ways with transitivity is given by known complexity results on various extensions of
guarded two-variable fragment with transitive relations. 
The {\em guarded fragment}, denoted \GF{}, is that fragment
of first-order logic in which all quantification
is of either of the forms 
$\forall \bar{v}(\alpha \rightarrow \psi)$ or $\exists \bar{v}(\alpha \wedge \psi)$,
where $\alpha$ is an atomic formula (a so-called {\em guard}) 
featuring all free variables of $\psi$. The
{\em guarded two-variable fragment}, denoted \GFt, is the intersection of
\GF{} and \FOt. It is straightforward to show that the addition
of two transitive relations to \GFt{} yields a logic whose satisfiability 
problem is undecidable. However, as long as the distinguished 
transitive relations appear only in guards, we can extend the whole
of \GF{} with any number of transitive relations, yielding the so-called 
{\em guarded fragment with transitive guards}, whose satisfiability 
problem is in \TwoExpTime~\cite{purdyTrans:st04}. Intriguingly, in the
two-variable case, we obtain a reduction in complexity if we
require transitive relations in guards to point {\em forward}---i.e.~allowing only $\forall v(t(u,v) \rightarrow \psi)$
rather than $\forall v(t(v,u) \rightarrow \psi)$, and similarly
for existential quantification. These restrictions resemble flutedness where one is not allowed to point {\em backward} neither in transitive atoms nor in other subformulas. 
 Thus, the extension of
\GFt{} with (any number of) transitive guards has a \TwoExpTime-complete
satisfiability problem; however, the corresponding problem under 
the  restriction to one-way transitive guards is \ExpSpace-complete~\cite{purdyTrans:kieronski06}. Since the above-mentioned extensions of \GFt{} also do not enjoy the finite model property, the satisfiability and the finite satisfiability problems do not coincide. 
Decidability and complexity bounds for the finite satisfiability problems are shown in \cite{purdyTrans:KT09,purdyTrans:KT18}. 

We show in the sequel that 
$\FL$ in the presence of a single transitive relation has the finite model property and it remains decidable, despite of loosing the finite model property, when equality is added. 
On the other hand, the satisfiability and the finite satisfiability problems for 
$\FL$ in the presence of three transitive relations are undecidable even for the intersection of $\FL$ with $\GFt$. (Indeed, the same holds even when one of these transitive relations is constrained to be the identity.)
The status of the decidability of $\FL$ with just two transitive relations remains open. Table~\ref{tab:overview} gives an overview of these results in comparison with known results on $\FOt$. \nb{L new Table}

\begin{center}
	\begin{table}
		
		\begin{center}
			{
				{%\setlength{\extrarowheight}{5pt}
					\begin{tabular}{|c|c|c|}
						\hline
						%			&\\
						{\bf Special symbols} & \multicolumn{2}{c|}{%\large{\color{white}I} 
							{\bf Decidability and Complexity}}\\
												& $\FLt$ & $\FOt$ \\
						%			&\\
						\hline\hline
						no transitive r.  &  \NExpTime-hard \cite{purdyTrans:ls01} &FMP \\
							& 	&  \NExpTime{}-complete \cite{purdyTrans:gkv97}\\
						%	\hline 
						%		0 transitive r. with = & {\bf no FMP, in \TwoNExpTime{}} \cite{???}\\
						
						\hline
						1 transitive r.   & FMP & \\
										&	 in \TwoNExpTime{} \cite{P-HT19} &  \Sat{}: ? \\
						\hline
						1 transitive r. & \Sat: in \TwoNExpTime &\\
						with =		&  {\bf  Theorem~\ref{theo:FLotransmEqUpper}}	& \FinSat: in \ThreeNExpTime \cite{PH18}\\
				%		\hline
				%		2 equivalence r. & decidable\\
						\hline
						2 transitive r.  &  \Sat{}: ? & undecidable  \\
										& \FinSat{}: ? & \cite{Kie05,Kaz06}\\
						\hline
						2 transitive r.  & undecidable &  \\
							with =				&  {\bf Theorem~\ref{th:two}} & \color{gray}{undecidable}\\
						\hline
						1 trans.\& 1 equiv. & undecidable &  \\
						with =					& {\bf  Corollary~\ref{cor:two}} &  \color{gray}{undecidable}\\
						\hline
						3 transitive r. &  undecidable & \\
										& \Sat: {\bf Theorem~\ref{th:three}} & \\
										& \FinSat{}: {\bf Theorem~\ref{th:threeFinsat}} & \color{gray}{undecidable}\\
						\hline
						3 equivalence r. & undecidable & \\
										& {\bf Corollary~\ref{cor:three}} & \color{gray}{undecidable} \\
						\hline
						
						%						1 linear order $(*)$& \NExpTime-complete \cite{Otto01}\\
						%						\hline			
						%						2 linear orders $(*)$  & Sat: ? \FinSat{} in \TwoNExpTime{}   \cite{ZeumeH2016} \\
						%						\hline			
						%						3 linear orders & undecidable \cite{Kie2011}\\
						%						\hline			
						%						
					\end{tabular} 
			}}
			%\caption{Overview}
			
			\caption{Overview of $\FLt$ and $\FOt$ over restricted classes of structures. Undecidability of extensions of \FOt{} depicted by gray have been known earlier but now can be inherited from remaining results of the Table.} %The upper bounds in the results marked with $(*)$ are actually obtained for full \FOt{}.} 
				\label{tab:overview}% The corresponding lower bounds, if present, hold for \GFt{}.}
		\end{center}
	\end{table}
\end{center}





%This can also be contrasted with the situation in {\em description logics} where any sublogic of $\mathcal{SI}$ and any sublogic of $\mathcal{SHOQ}$ (the letter $\mathcal S$ in the logic names stands for transitivity) enjoys the finite model property independently from the number of transitive relations (cf.~e.g.~\cite{purdyTrans:dlh} for details).
%However, it follows from our results that, if the restriction of this logic to formulas with just two variables (and no other
%non-unary predicates other than the two distinguished transitive relations) is as general as we need: it the
%satisfiability for this sub-fragment is decidable, so is the whole fragment. 
 
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 
 \section{Conclusions}
 In this paper, we considered the ($m$-variable) fluted fragment in the presence of different numbers of transitive relations. $\FLotrans$ enjoys the finite model property; we showed that it remains decidable when adding equality (despite of loosing the finite model property). We also showed that decidability is lost already for the two-variable fragments of $\FL$: when a second transitive relation is added to $\FLotranstEq$, or equality is not present but instead the logic allows for three transitive relations. 
 %
 % This contrasts with known results for other decidable fragments, in particular, $\FOt$, where the satisfiability and finite satisfiability problems are undecidable
 %in the presence of two transitive relations, and where the \textit{finite} satisfiability problem is decidable in the presence of one transitive relation.
 It is open whether the (finite) satisfiability problem for $\FL$ in the presence of \textit{two} transitive relations, $\ft_1$ and $\ft_2$, is decidable.
 We point out that Lemma~\ref{lma:FLotransmEqToFLotransmEq} in Section~\ref{sec:onetrans} could be generalized to normal form formulas from $\FLtwotransmpo$. Hence,  the (finite) satisfiability problem for  $\FL$ in the presence of two transitive relations is decidable if and only if the corresponding problem for $\FLt$
 with two transitive relations is decidable. Unfortunately neither the method of Sec.~\ref{sec:onetrans} (to show
 decidability) nor that of Sec.~\ref{sec:undecidable} (to show
 undecidability) appears to apply here. The barrier in the former case is that pairs of elements can be related by both $\ft_1$ and $\ft_2$ via divergent $\ft_1$- and $\ft_2$-chains, so that simple certificates of the kind employed for $\FLotranstMinus$ do not guarantee the existence of models. The barrier in the latter case is that the grid construction has to build models featuring transitive paths of {\em bounded} length, and this seems not to be achievable with just two transitive relations. 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\appendix

%\section{Put this somewhere}
%
%\begin{proof}[Proof of Lemma~\ref{lma:eliminate}]
%	Assume $\phi$ to be as in~\eqref{eq:cnf}, write $T = \{1, \dots, t\}$. For
%	all $i$ ($1 \leq i \leq s$) and all $J \subseteq T$, let $p_{i,J}$ and $q_J$ be new
%	predicates of arity $k-1$. Let $\phi'$ be the conjunction of the sentences
%	\begin{align}
%	&
%	\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_1 \cdots x_{k}
%	((\alpha_i \wedge \bigwedge_{j \in J} \beta_j )  \rightarrow p_{i,J}(x_2, \dots, x_{k}))
%	\label{eq:phiStar1}\\
%	&
%	\bigwedge_{J \subseteq T}\forall x_1 \cdots x_{k}
%	((\bigwedge_{j \in J} \beta_j) \rightarrow q_{J}(x_2, \dots, x_{k}))
%	\label{eq:phiStar2}\\
%	%\begin{split}
%	& 
%	\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_2 \cdots x_{k}
%	\left( p_{i,J}(x_2, \dots, x_{m-1})\rightarrow \exists x_{k+1} \left(\Gamma_i \cup \Omega \cup \{\delta_j \mid j \in J \}\right)^\circ \right) 
%	%\end{split} 
%	\label{eq:phiStar3}\\ 
%	&
%	\bigwedge_{J \subseteq T}\forall x_2 \cdots x_{k}
%	\left( q_{J}(x_2, \dots, x_{k})\rightarrow \forall x_{k+1} \left(\Omega \cup  \{\delta_j \mid j \in J \}\right)^\circ \right).
%	\label{eq:phiStar4}
%	\end{align}
%	We claim that, if $\phi$ is satisfiable, then so is $\phi'$. 
%	For suppose $\fA \models \phi$. We expand
%	$\fA$ to a model $\fA' \models \phi'$ by setting, for all $i$ ($1 \leq i \leq s$) and all $J \subseteq T$,
%	\begin{align*}
%	\begin{split}
%	p_{i,J}^{\fA'}  = \{ \langle a_2, & \dots, a_{k} \rangle \mid \text{ for some $a_1 \in A$: }\\ 
%	& \text{$\fA \models \alpha_i[a_1, \dots, a_{k}]$ and $\fA \models \beta_j[a_1, \dots, a_{k}]$ for all $j \in J$}  \}
%	\end{split}\\
%	\begin{split}
%	q_{J}^{\fA'}  = \{ \langle a_2, & \dots, a_{k} \rangle \mid \text{ for some $a_1 \in A$: }\\ 
%	& \text{$\fA \models \beta_j[a_1, \dots, a_{k}]$ for all $j \in J$}  \}.
%	\end{split}
%	\end{align*}
%	To see that $\fA' \models \phi'$, we simply check the truth of conjuncts~\eqref{eq:phiStar1}--\eqref{eq:phiStar4} in $\fA'$ in turn.
%	Sentences~\eqref{eq:phiStar1} and~\eqref{eq:phiStar2} are immediate. For~\eqref{eq:phiStar3}, fix $i$ and $J$, and suppose
%	$\fA' \models p_{i,J}[a_2, \dots, a_{k}]$. By the definition of $\fA'$,
%	let $a_1 \in A$ be such that $\fA \models \alpha_i[a_1, \dots, a_{m-1}]$ and 
%	$\fA \models \beta_j[a_1, \dots, a_{k}]$ for all $j \in J$. Since $\fA \models \phi$, there exists
%	$b$ such that $\fA \models \Gamma_i[a_1, \dots, a_{k},b]$, \mbox{$\fA \models \Omega[a_1, \dots, a_{k},b]$} and
%	$\fA \models \delta_j[a_1, \dots, a_{k},b]$ for all $j \in J$. Since resolution is a valid inference step,
%	$\fA' \models \left(\Gamma_i \cup \Omega \cup \{\delta_j \mid j \in J \}\right)^\circ[a_2, \dots, a_{k},b]$. This
%	establishes the truth of~\eqref{eq:phiStar3} in $\fA'$. Sentence~\eqref{eq:phiStar4} is handled similarly.
%	
%	Conversely, we claim that, if 
%	$\phi'$ is satisfiable over a domain $A$, then $\phi$  is satisfiable over a domain of size  $s \cdot |A|$.
%	For suppose $\fA \models \phi'$. Let $\fB$ be the model of $\phi'$ guaranteed by Lemma~\ref{lma:multiply}, where $z= s$. 
%	We may assume that $\fA$ and hence $\fB$ interpret no predicates of arity $m$.
%	We proceed to expand $\fB$ to a model $\fB' \models \phi$ by interpreting the predicates of arity $m$ occurring in $\phi$.      
%	Pick any tuple $\langle a_1, a_2, \dots, a_{m-1} \rangle$ from $B$, and let $J$ be the set of all $j$ ($1 \leq j \leq t$)
%	such that $\fB \models \beta_j[a_1, a_2, \dots, a_{k}]$. Suppose also that, for some $i$ ($1 \leq i \leq s$)
%	$\fA \models \alpha_i[a_1, a_2, \dots, a_{k}]$. 
%	From~\eqref{eq:phiStar1}, $\fB \models p_{i,J}[a_2, \dots, a_{k}]$; and
%	from~\eqref{eq:phiStar3},
%	we may pick $b_i \in B$ such that
%	$\fB \models \left(\Gamma_i \cup \Omega \cup \{\delta_j \mid j \in J \}\right)^\circ[a_2, \dots, a_{k},b_i]$. From the properties secured for $\fB$ by Lemma~\ref{lma:multiply}, we know that if, for fixed $a_1, \dots, a_{k}$,
%	we have $\fA \models \alpha_i[a_1, a_2, \dots, a_{k}]$ for more than one value of $i$, then
%	we may choose the corresponding elements $b_{i}$ so that they are all distinct.  
%	For each such $b_i$, then, let $\tau_i = \tp^{\fB}[a_2, \dots, a_{k},b_{i}]$. Thus, $\tau_i(x_2, \dots, x_{k+1})$ is consistent
%	with $\left(\Gamma_i \cup \Omega \cup \{\delta_j \mid j \in J \}\right)^\circ$. By Lemma~\ref{lma:resolution}, there exists a 
%	fluted $(k+1)$-type $\tau_i^+ \supseteq \tau_i(x_1, \dots, x_{k+1})$ such that $\tau_i^+$ is consistent with $\Gamma_i \cup \Omega \cup  \{\delta_j \mid j \in J \}$. Set $\tp^{\fB'}[a_1,a_2, \dots, a_{k},b_{i}] = \tau^+_i$. Since $\tau^+_i \supseteq \tau_i(x_2, \dots, x_{k+1})$,
%	only ordinary predicates of arity $k+1$ are being assigned, so that there is no clash with $\fB$. Moreover, since the $b_i$ are all distinct,
%	for a given tuple $a_1, \dots, a_{k}$, these assignments do not clash with each other. In this way, every existential conjunct of $\phi$ is witnessed in $\fB'$ for the tuple
%	$a_1,a_2, \dots, a_{k}$, and no static or universal conjunct of $\phi$ is violated for the tuples from $B$ for which the $m$-ary predicates of $\sigma$ have been defined.
%	Now let $\langle a_1, a_2, \dots, a_{k}, a_{k+1} \rangle$ be any tuple from $B$ for which the $m$-ary predicates
%	of $\sigma$ have not been defined, and let $J$ be the set of all $j$ ($1 \leq j \leq m$)
%	such that $\fB \models \beta_j[a_1, a_2, \dots, a_{k}]$. From~\eqref{eq:phiStar2},
%	$\fB \models q_J[a_2, \dots, a_{k}]$; and from~\eqref{eq:phiStar4}, 
%	$\fB \models \left(\Omega \cup  \{\delta_j \mid j \in J \} \right)^\circ[a_2, \dots, a_{k}, a_{k+1}]$. 
%	Let $\tau= \tp^\fB[a_2, \dots, a_{k},a_{k+1}]$.  Hence $\tau(x_2, \dots, x_{k+1})$ is consistent with 
%	$\left( \{\delta_j \mid j \in J \} \right)^\circ$. By Lemma~\ref{lma:resolution}, there exists a 
%	fluted $(k+1)$-type $\tau^+ \supseteq \tau(x_1, \dots, x_{k+1})$ such that $\tau^+$ is consistent 
%	with $\Omega \cup  \{\delta_j \mid j \in J \}$. Set $\tp^{\fB'}[a_1,a_2, \dots, a_{k},a_{k+1}] = \tau^+$. 
%	Since $\tau^+ \supseteq \tau(x_2, \dots, x_{k+1})$, only ordinary predicates of arity $k+1$ are being assigned, so that there is no clash with $\fB$. 
%	Evidently, no static or universal conjunct of $\phi$ is violated in this process. Thus, $\fB' \models \phi$, as required.
%	
%	We now consider separately the cases $k>1$ and $k=1$. For the former, 
%	conjuncts~\eqref{eq:phiStar1} and~\eqref{eq:phiStar2} do not involve $x_{k+1}$, while~\eqref{eq:phiStar3} 
%	and~\eqref{eq:phiStar4} do not involve $x_1$. Thus, by decrementing variable indices where necessary,
%	$\phi'$ becomes a formula of $\FLotransk$. Indeed, re-writing implications as clauses in the
%	obvious way, we have a formula in normal form: formulas
%	\eqref{eq:phiStar1} and~\eqref{eq:phiStar2} give the static conjunct; formula~\eqref{eq:phiStar3} gives the $2^t s$
%	existential conjuncts; and formula~\eqref{eq:phiStar4} gives the $2^t$ 
%	universal conjuncts. Exactly $2^t(s +1)$ predicates of arity \mbox{${(k-1)}$} have been added to the signature, and some $k$-ary 
%	predicates may have been lost.
%	For the case $k=1$, we simply observe that $\phi'$ does not involve any 
%	non-distinguished predicates of arity $k+1 = 2$, and that 
%\end{proof}
%
%\section{Proofs from Section \ref{sec:onetrans}}
%%\subsection{Proof of Lemma~\ref{lma:nf}}
%%We employ standard `re-writing' techniques, temporarily allowing 0-ary predicates. By moving negations inward in the usual way, we may assume without loss of generality that negation symbols in $\phi$ apply only to atoms. 
%%%As usual, a {\em literal} is either an atom or a negated atom. Write $\phi_0:= \phi$.
%%Suppose $\phi_0$ has a subformula $\theta= \exists x_{k+1} . \zeta$ ($0 \leq k < 2$), where $\zeta$ is quantifier-free. Let $p$ be a fresh predicate of arity $k$ (thus: 0-ary predicates can be introduced), and again let $\phi_1:= \phi_0[\theta/p(x_1, \dots, x_k)]$ and $\psi_1:= \forall x_1 \cdots \forall x_k (p(x_1, \dots, x_k) \leftrightarrow \theta)$; hence, $\models \phi_1 \wedge \psi_1 \rightarrow \phi_0$, and any model of $\phi_0$ can be expanded to a model of $\phi_1 \wedge \psi_1$. Thus, $\psi_1$ is of the form $\forall x_1 \cdots \forall x_k (p(x_1, \dots, x_k) \leftrightarrow \exists x_{k+1} . \zeta)$, where $\zeta$ is fluted and quantifier-free.
%%Suppose, alternatively, that $\phi_0$ has a subformula $\theta= \forall x_{k+1} . \zeta$. where $\zeta$ is quantifier-free. We proceed in the similarly, except that 
%%$\psi_1$ is of the form $\forall x_1 \cdots \forall x_k (p(x_1, \dots, x_k) \leftrightarrow \forall x_{k+1} . \zeta)$.
%%
%%Proceeding similarly with $\phi_1$ in place of $\phi_0$, we obtain $\phi_2$ and $\psi_2$, and so on, until we reach some point where
%%the $\FL^{m}$-sentence $\phi_s$ is a proposition letter. Defining $\psi'$ to be $\psi_1 \wedge \cdots \wedge \psi_s \wedge \phi_s$, we see that 
%%$\models \psi' \rightarrow \phi$, and any model of $\phi$ can be expanded to a model of $\psi'$. It should be clear that the size
%%of $\psi'$ is at most linear in the size of $\phi$. Each of the $\psi_i$ and indeed $\phi_s$
%%is either a proposition letter or (following variable re-naming) of one of the forms 
%%\begin{align*}
%%& \ \forall x_1  (p(x_1) \leftrightarrow \exists x_2 . \lambda) \qquad \forall x_1  (p(x_1) \leftrightarrow \forall x_2 . \lambda)
%%\qquad  P \leftrightarrow \forall x_1 . \mu\qquad P \leftrightarrow \exists x_1. \mu,
%%\end{align*} 
%%where $\lambda$ is a quantifier-free fluted formula in variables $x_1, x_2$ and $\mu$ a quantifier-free fluted formula with variable $x_1$. Furthermore, we may re-write any formula $\forall x_1  (p(x_1) \leftrightarrow \exists x_2 . \lambda)$ equivalently as a conjunction
%%$\forall x_1  (p(x_1) \rightarrow \exists x_2 . \lambda) \wedge \forall x_1  (\neg p(x_1) \rightarrow \forall x_2  \neg \lambda)$, 
%%and similarly for $\forall x_1  (p(x_1) \leftrightarrow \forall x_2 . \lambda)$.
%%
%%
%%Eliminate the 0-ary predicates by guessing their truth values and carrying out the obvious simplifications. Let $\Psi'$ be any
%%satisfiable collection
%%of formulas obtained in this way if there is one (or any of them if $\phi$ is not satisfiable).
%%Massaging $\Psi'$ into a set of formulas $\Psi$ of the desired forms is then completely routine.
%%
%%
%%\subsection{Proof of Lemma~\ref{lma:resolution}}\label{app:resolution}
%%	Enumerate the atoms $r(x_1, \dots, x_m)$ where  $r \in \Sigma$ is of maximal arity $m$, as 
%%$\rho_1, \dots, \rho_n$.
%%Define a \textit{level-$i$ extension}
%%of $\tau^-$ inductively as follows: (i) $\tau^-$ is a level-0 extension of $\tau^-$; (ii) if $\tau'$ is a level-$i$ extension of $\tau^-$ ($0 \leq i < n$), then $\tau' \wedge \rho_{i+1}$  and $\tau' \wedge \neg \rho_{i+1}$ are 
%%level-$(i+1)$ extensions of $\tau^-$. Thus, the level-$n$ extensions of $\tau^-$ are exactly 
%%the fluted $m$-types over $\Sigma \cup \set{\ft}$ entailing
%%$\tau^-$. 
%%If $\tau'$ is a level-$i$ extension of $\tau^-$ ($0 \leq i < n$), we say that $\tau'$ {\em violates} a clause $\delta$
%%if, for every literal in $\delta$, the opposite literal is in $\tau'$; we say that $\tau'$ {\em violates} a set of clauses
%%$\Delta$ if $\tau'$ violates some $\delta \in \Delta$.
%%We construct a sequence of level-$i$ extensions of $\tau^-$ ($i = 0, 1, \dots$) none of which violates $\Gamma^*$.
%%
%%By definition, $\tau^-$ is a level-0 extension of itself. 
%%Suppose now that $\tau'$ is a level-$i$ extension of $\tau^-$ ($0 \leq i < n$). We claim that, if both 
%%$\tau' \wedge \rho_{i+1}$  and $\tau' \wedge \neg \rho_{i+1}$ violate $\Gamma^*$, then so does $\tau'$. For otherwise, there must be a clause $\neg \rho_{i+1} \vee \gamma' \in \Gamma^*$ violated by $\tau' \wedge \rho_{i+1}$ and a clause $\rho_{i+1} \vee \delta' \in \Gamma^*$ violated by $\tau' \wedge \neg \rho_{i+1}$. But in that case $\tau'$ violates the fluted resolvent $\gamma' \vee \delta'$,  contradicting the
%%supposition that $\tau'$ does not violate $\Gamma^*$. This proves the claim. Now, since $\tau^-$ 
%%by hypothesis is consistent with $\Gamma^\circ$, it does not violate $\Gamma^\circ$. Therefore, since $\tau^-$ involves no $m$-literals
%%$\pm r(x_1, \dots, x_m)$ for $r \in \Sigma$, it does not violate $\Gamma^*$ either. By the above claim, then,
%%there must be at least one level-$n$ extension $\tau$ of $\tau^-$ which does not
%%violate $\Gamma^* \supseteq \Gamma$. Since $\tau$ is a fluted $m$-type, this proves the lemma.
%
%\subsection{Proof of Lemma~\ref{lma:eliminateNonTrans}}\label{app:eliminateNonTrans}\nb{L: left temporarily here}
%Let $\phi$ be the formula
%% = \forall x_1 x_{2} . \Omega \ \wedge
%%{\bigwedge_{i=1}^{s} }\forall x_1 \left(p_i(x_1) \rightarrow \exists x_2 . \Gamma_i\right) \wedge
%%{\bigwedge_{j=1}^{t}} \forall x_1 (q_j(x_1) \rightarrow \forall x_2 . \Delta_j),$\nb{removed displayed math}
%%\label{eq:cnfTwo}
%%
%\begin{equation}
%\forall x_1 x_{2} . \Omega \ \wedge
%{\bigwedge_{i=1}^{s} }\forall x_1 \left(p_i(x_1) \rightarrow \exists x_2 . \Gamma_i\right) \wedge
%{\bigwedge_{j=1}^{t}} \forall x_1 (q_j(x_1) \rightarrow \forall x_2 . \Delta_j),
%\label{eq:cnfTwo}
%\end{equation}
%where $\Omega, \Gamma_1, \dots, \Gamma_s, \Delta_1, \dots, \Delta_t$ are sets of fluted 2-clauses,
%and $p_1, \dots, p_s$, $q_1, \dots, q_t$ unary predicates. Write $T = \{1, \dots, t\}$.
%For all $i$ ($1 \leq i \leq s$) and all $J \subseteq T$, let $p_{i,J}$ and $q_J$ be new unary
%predicates.
%The intended interpretation of $p_{i,J}(x_1)$ is ``$x_1$ satisfies $p_i$, and also satisfies $q_j$ for every $j \in J$;'' and
%the intended interpretation of $q_{J}(x_1)$ is ``$x_1$ satisfies $q_j$ for every $j \in J$.''
%Let $\phi'$ be the conjunction of the sentences%\nb{It occurs to me that in THIS case, we can do a bit better and avoid an exponential blow-up in the signature. But it would involve too much re-writing at this stage. For one exponential, it's hardly worth it.}
%\begin{align}
%&
%\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_2
%(p_i(x_2) \wedge \bigwedge_{j \in J} q_j(x_2))  \rightarrow p_{i,J}(x_2))
%\label{eq:phiStar1Two}\\
%&
%\bigwedge_{J \subseteq T}\forall x_2
%((\bigwedge_{j \in J} q_j(x_2)) \rightarrow q_{J}(x_2))
%\label{eq:phiStar2Two}\\
%%\begin{split}
%& 
%\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_1
%\left( p_{i,J}(x_1)\rightarrow \exists x_2 \left(\Gamma_i \cup \Omega \cup \bigcup \{\Delta_j \mid j \in J \}\right)^\circ \right) 
%%\end{split} 
%\label{eq:phiStar3Two}\\ 
%&
%\bigwedge_{J \subseteq T}\forall x_1 
%\left(q_{J}(x_1) \rightarrow \forall x_2 \left(\Omega \cup \bigcup \{\Delta_j \mid j \in J \}\right)^\circ \right).
%\label{eq:phiStar4Two}
%\end{align}
%We claim that, if $\phi$ is satisfiable, then so is $\phi'$ (see Appendix, Section~\ref{app:eliminateNonTrans}). This proves the lemma, since $\phi'$ evidently contains no
%non-distinguished binary predicates, and hence is in $\FLotranstMinus$.
%
%For suppose $\fA \models \phi$. We expand
%$\fA$ to a model $\fA' \models \phi'$ by setting, for all $i$ ($1 \leq i \leq s$) and all $J \subseteq T$,\\
%$	p_{i,J}^{\fA'}  = \{ a \mid \text{$\fA \models p_i[a]$ and $\fA \models q_j[a]$ for all $j \in J$}  \}$ and 
%$q_{J}^{\fA'}  = \{ a \mid \text{$\fA \models q_j[a]$ for all $j \in J$}  \}$.
%
%%	\begin{align*}
%%	p_{i,J}^{\fA'} & = \{ a \mid \text{$\fA \models p_i[a]$ and $\fA \models q_j[a]$ for all $j \in J$}  \}\\
%%	q_{J}^{\fA'} & = \{ a \mid \text{$\fA \models q_j[a]$ for all $j \in J$}  \}.
%%	\end{align*}
%\medskip\noindent	To see that $\fA' \models \phi'$, we simply check the truth of conjuncts~\eqref{eq:phiStar1Two}--\eqref{eq:phiStar4Two} in $\fA'$ in turn.
%Sentences~\eqref{eq:phiStar1Two} and~\eqref{eq:phiStar2Two} are immediate. For~\eqref{eq:phiStar3Two}, fix $i$ and $J$, and suppose
%$\fA' \models p_{i,J}[a_1]$. By the definition of $\fA'$, $\fA \models p_i[a_1]$ and 
%$\fA \models q_j[a_1]$ for all $j \in J$. Since $\fA \models \phi$, there exists
%$b$ such that $\fA \models \Gamma_i[a_1, b]$, \mbox{$\fA \models \Omega[a_1, b]$} and
%$\fA \models \Delta_j[a_1, b]$ for all $j \in J$. Since resolution is a valid inference step,
%$\fA' \models \left(\Gamma_i \cup \Omega \cup \bigcup \{\Delta_j \mid j \in J \}\right)^\circ[a_1,b]$. This establishes the truth of~\eqref{eq:phiStar3Two} in $\fA'$. Sentence~\eqref{eq:phiStar4Two} is handled similarly.
%
%Conversely, we claim that, if 
%$\phi'$ is satisfiable over a domain $A$, then $\phi$  is satisfiable over a domain of size  $s \cdot |A|$.
%For suppose $\fA \models \phi'$. Let $\fB$ be the model of $\phi'$ guaranteed by Lemma~\ref{lma:multiply}, where $z= s$. 
%We may assume that $\fA$ and hence $\fB$ interpret no non-distinguished predicates of arity $2$.
%We proceed to expand $\fB$ to a model $\fB' \models \phi$ by interpreting the non-distinguished predicates of arity $2$ occurring in $\phi$.      
%Pick any element $a_1$ from $B$, and let $J$ be the set of all $j$ ($1 \leq j \leq t$)
%such that $\fB \models q_j[a_1]$. Suppose also that, for some $i$ ($1 \leq i \leq s$)
%$\fA \models p_i[a_1]$. 
%From~\eqref{eq:phiStar1Two}, $\fB \models p_{i,J}[a_1]$; and
%from~\eqref{eq:phiStar3Two},
%we may pick $b_i \in B$ such that
%$\fB \models \left(\Gamma_i \cup \Omega \cup \bigcup \{\Delta_j \mid j \in J \}\right)^\circ[a_1,b_i]$. From the properties secured for $\fB$ by Lemma~\ref{lma:multiply}, we know that if, for fixed $a$,
%we have $\fA \models \alpha_i[a_1]$ for more than one value of $i$, then
%we may choose the corresponding elements $b_{i}$ so that they are all distinct.  
%For each such $b_i$, then, let $\tau_i = \ftp^{\fB}[a_1,b_{i}]$. Thus, $\tau_i(x_1,x_2)$ is consistent
%with $\left(\Gamma_i \cup \Omega \cup \bigcup \{\Delta_j \mid j \in J \}\right)^\circ$. By Lemma~\ref{lma:resolution}, there exists a 
%fluted $2$-type $\tau_i^+ \supseteq \tau_i(x_1, x_2)$ such that $\tau_i^+$ is consistent with $\Gamma_i \cup \Omega \cup  \bigcup \{\Delta_j \mid j \in J \}$. 
%Set $\ftp^{\fB'}[a_1,b_{i}] = \tau^+_i$. Since $\tau^+_i \supseteq \tau_i$,
%only non-distinguished binary predicates are being assigned, so that there is no clash with $\fB$. Moreover, since the $b_i$ are all distinct (for a given element $a$),
%these assignments do not clash with each other. In this way, every existential conjunct of $\phi$ is witnessed in $\fB'$ for every element $a$, and no static or universal conjunct of $\phi$ is violated for the tuples from $B$ for which the binary predicates of $\Sigma$ have been defined.
%Now let $\langle a_1, a_2 \rangle$ be any ordered pair from $B$ for which the binary predicates
%of $\Sigma$ have not been defined, and let $J$ be the set of all $j$ ($1 \leq j \leq t$)
%such that $\fB \models q_j[a_1]$. From~\eqref{eq:phiStar2Two},
%$\fB \models q_J[a_1]$; and from~\eqref{eq:phiStar4Two}, 
%$\fB \models \left(\Omega \cup  \bigcup \{\Delta_j \mid j \in J \} \right)^\circ[a_1,a_2]$. 
%Let $\tau= \ftp^\fB[a_1,a_2]$.  Hence $\tau(x_1, x_2)$ is consistent with 
%$\left(\Omega \cup \bigcup \{\Delta_j \mid j \in J \} \right)^\circ$. By Lemma~\ref{lma:resolution}, there exists a 
%fluted 2-type $\tau^+ \supseteq \tau$ such that $\tau^+$ is consistent 
%with $\Omega \cup  \bigcup \{\Delta_j \mid j \in J \}$. Set $\ftp^{\fB'}[a_1,a_2] = \tau^+$. 
%Since $\tau^+ \supseteq \tau$, only non-distinguished binary predicates are being assigned, so that there is no clash with $\fB$. 
%Evidently, no static or universal conjunct of $\phi$ is violated in this process. Thus, $\fB' \models \phi$, as required.
%
%
%
%%\subsection{Proof of Lemma~\ref{lma:eliminate}}
%%	Similar
%%	to the proof of Lemma~\ref{lma:eliminateNonTrans}. Taking $\phi$ to be as in~\eqref{eq:cnf},
%%	write $T = \{1, \dots, t\}$. For
%%	all $i$ ($1 \leq i \leq s$) and all $J \subseteq T$, let $p_{i,J}$ and $q_J$ be new
%%	predicates of arity $m-2$.
%%	The intended interpretation of $p_{i,J}(x_2, \dots, x_{m-1})$ is ``for some $x_1$, 
%%	the tuple $x_1, \dots, x_{m-1}$ satisfies $\alpha_i$ and also satisfies $\beta_j$ for every $j \in J$;'' and
%%	the intended interpretation of $q_{J}(x_2, \dots, x_{m-1})$ is ``for some $x_1$, 
%%	the tuple $x_1, \dots, x_{m-1}$ satisfies $\beta_j$ for every $j \in J$.''
%%	Let $\phi'$ be the conjunction of the sentences
%%	\begin{align}
%%	&
%%	\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_1 \cdots \forall x_{m-1}
%%	((\alpha_i \wedge \bigwedge_{j \in J} \beta_j )  \rightarrow p_{i,J}(x_2, \dots, x_{m-1}))
%%	\label{eq:phiStar1}\\
%%	&
%%	\bigwedge_{J \subseteq T}\forall x_1 \cdots \forall x_{m-1}
%%	((\bigwedge_{j \in J} \beta_j) \rightarrow q_{J}(x_2, \dots, x_{m-1}))
%%	\label{eq:phiStar2}\\
%%	& 
%%	\bigwedge_{i=1}^{s} \bigwedge_{J \subseteq T} \forall x_2 \cdots \forall x_{m-1}
%%	( p_{i,J}(x_2, \dots, x_{m-1})\rightarrow \exists x_m (\Gamma_i \cup \Omega \cup \bigcup_{j \in J} \Delta_j )^\circ )
%%	\label{eq:phiStar3}\\ 
%%	&
%%	\bigwedge_{J \subseteq T}\forall x_2 \cdots \forall x_{m-1}
%%	( q_{J}(x_2, \dots, x_{m-1})\rightarrow \forall x_m (\Omega \cup  \bigcup_{j \in J} \Delta_j )^\circ ).
%%	\label{eq:phiStar4}
%%	\end{align}
%%	We claim that, if $\phi$ is satisfiable, then so is $\phi'$. Note that, since $m \geq 2$, \eqref{eq:phiStar3} and~\eqref{eq:phiStar4} do not involve $x_1$. By decrementing all variable indices in these conjuncts, therefore,
%%	we obtain a formula of $\FLotransm$ as required by the lemma. The proof of the claim proceeds almost identically to Lemma~\ref{lma:eliminateNonTrans}.
%
%
%
%
%
%	%
%		
